Flow Decomposition

The decode-forward achievable region is studied for general networks. The region is subject to a fundamental tension in which nodes individually benefit at the expense of others. The complexity of the region depends on all the ways of resolving this tension. Two sets of constraints define an outer-bound on the decode-forward region: first, the conventional mutual-information inequalities implied by the one-relay channel, and second, causality constraints that ensure nodes only forward messages they have already decoded. The framework of flow decomposition is introduced to show these constraints are also sufficient. Flow decomposition provides a way of manipulating regular decode-forward schemes without the long encoding delays and restrictions on bidirectional communication of backward decoding. The two structures that define a flow decomposition are flows and layerings. Flows specify the nodes which encode messages from each source (i.e., the routes) and the encoding delays. Layerings specify the messages decoded at a specific node in the channel. We focus on two types of flow: hierarchical flow, with tree-like routes, and all-cast flow, where each route covers all nodes. For arbitrary flows of either type and any rate-vector satisfying the mutual-information constraints at a specific node, we prove there are equivalent flows and a layering that satisfy both the mutual-information and causality constraints. In separate work, we show that only the mutual-information constraints are active in channels with hierarchical flow, which implies the achievable region has minimal complexity. In channels with all-cast flow, the achievable region is computable.

==> flowdecomp 2/clocksecurity.tex <==
% Given ${\bf f}(s,d):=N_{1}\xrightarrow{k_{1}}N_{2}\xrightarrow{k_{2}}\cdots\xrightarrow{k_{e-1}}N_{e}$, suppose $v(s)\subseteq N_{l}$ for some $1\leq l\leq e$.  Let ${\bf f}(v(s),d):=v(s)\xrightarrow{k_{l}}N_{l+1}\xrightarrow{k_{l+1}}\cdots\xrightarrow{k_{e-1}}N_{e}$.  For $i\in{\bf f}(s,v(s))$, let $k_{i,v(s)}:=k_{s,v(s)}-k_{s,i}$.  It can be shown that:
 
 \begin{lemma}
 \label{vssuffices}
The $v(s)$ in (\ref{vs}) uniquely satisfies:
\begin{align}
\label{firstIndexCoding}
\text{\sc layer}(v(s))-\text{\sc layer}(i)&\leq k_{v(s),i}\hspace{2mm}\forall i\in{\bf f}(v(s),d),\\
\label{secondIndexCoding}
\text{\sc layer}(i)-\text{\sc layer}(v(s))&> k_{i,v(s)}	\hspace{2mm}\forall i\in{\bf f}(s,v(s)),
\end{align}	
where $k_{v(s),i}:=k_{s,i}-k_{s,v(s)}$ for all $i\in{\bf f}(v(s),d)$ and  $k_{i,v(s)}:=k_{s,v(s)}-k_{s,i}$ for all $i\in{\bf f}(s,v(s))$. 
\end{lemma}
\begin{proof}
By construction $v(s)\subseteq M(s)$, which minimizes $u(s,i):=\text{\sc layer}(i)+k_{s,i}$ for all $i\in{\bf f}(s)$.  Therefore $\text{\sc layer}(v(s))+k_{s,v(s)}\leq\text{\sc layer}(i)+k_{s,i}$ which implies $\text{\sc layer}(v(s))-\text{\sc layer}(i)\leq k_{s,i}-k_{s,v(s)}$.  By definition $k_{v(s),i}:=k_{s,i}-k_{s,v(s)}$ for all $i\in{\bf f}(v(s),d)$ which yields (\ref{firstIndexCoding}).  
	
Furthermore (\ref{vs}) implies $v(s)$ is the subset of $M(s)$ closest to source  $s$ by hop count.  Therefore $\text{\sc layer}(v(s))+k_{s,v(s)}<\text{\sc layer}(i)+k_{s,i}$ if $i\in{\bf f}(s,v(s))$, which implies $\text{\sc layer}(i)-\text{\sc layer}(v(s))>k_{s,v(s)}-k_{s,i}$. By definition $k_{i,v(s)}:=k_{s,v(s)}-k_{s,i}$ for all $i\in{\bf f}(s,v(s))$ which yields (\ref{secondIndexCoding}).
\end{proof}


==> flowdecomp 2/disjoint.tex <==
\begin{lemma}
	\label{disjoint}
	For every $S\subseteq{\cal S}(d)$ and $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$, $A_{l}(S)\setminus A_{l}(U)\subseteq A^{\prime}_{l}(S)$.
\end{lemma}
\begin{proof}
We first prove some preliminary claims.

\hspace{-3.5mm}{\bf Claim \ref{disjoint}.1} \textit{Suppose $s\notin U$ and $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$ for some $j\in{\bf v}(s)$.  Then:}

\begin{align}
\label{Case3v2s}
	v^{\prime}(s)&:=\left\{j:\arg\displaystyle\min_{\substack{j\in {\bf v}(s),\\ \text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)}} k_{v(s),j}\right\}.
\end{align}

\begin{proof}
Since the premise of Claim \ref{disjoint}.1 is that there is some $j\in{\bf v}(s)$ such that $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$, it follows that $v^{\prime}(s)$ is non-empty.  To prove the claim, we invoke Lemma \ref{vssuffices} and check that (\ref{Case3v2s}) satisfies (\ref{firstIndexCodingShiftedComplete}) and (\ref{secondIndexShiftedComplete}).
%$v_{2}(j):=\arg\min_{\tilde{i}\in {\bf v}_{1}(j):\text{\sc layer}_{1}(\tilde{i})=\text{\sc layer}_{2}(\tilde{i})} k_{v_{1}(j),\tilde{i}}$
  
\hspace{-3.5mm}{\bf Claim \ref{disjoint}.1.a} \textit{For all $j\in{\bf f}(v(s),v^{\prime}(s))$ and $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$, the $v^{\prime}(s)$ defined in (\ref{Case3v2s}) satisfies (\ref{secondIndexShiftedComplete}).}
\begin{proof}
Consider the following inequalities:
\begin{align}
	\label{Case3Stage28}
	k_{v(s),j}&\geq\text{\sc layer}(v(s))-\text{\sc layer}(j),\\
	\label{Case3Stage29}
	&>\text{\sc layer}(v(s))-\text{\sc layer}(j),
\end{align} 
where (\ref{Case3Stage28}) follows from (\ref{firstIndexCodingShiftedComplete2}).  Since $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$ and $j\in{\bf f}(v(s),v^{\prime}(s))$, (\ref{Case3v2s}) implies that $j\notin{\bf v}(s)$ because otherwise $j\in{\bf v}(s)$ and $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$ and   $k_{v(s),j}<k_{v(s),v^{\prime}(s)}$ is a contradiction.  Moreover, (V5) implies that equality in (\ref{Case3Stage28}) only holds if $j\in{\bf v}(s)$ which implies (\ref{Case3Stage29}).  Now consider the following inequalities:
\begin{align}
	\label{Case3Stage210}
	k_{v(s),v^{\prime}(s)}&=\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s)),\\
	\nonumber
	&=\text{\sc layer}(v(s))-\text{\sc layer}(j)\\
	\label{Case3Stage211}
	&\hspace{18mm}+\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s)),
\end{align}
where (\ref{Case3Stage210}) follows from (V5) and because (\ref{Case3v2s}) implies $v^{\prime}(s)\in{\bf v}(s)$, and (\ref{Case3Stage211}) follows by adding and subtracting $\text{\sc layer}(j)$.  Rearranging (\ref{Case3Stage211}) gives:
\begin{align}
	\nonumber
	&\hspace{-2mm}\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s))\\
	\label{Case3Stage212}
	&\hspace{9mm}=k_{v(s),v^{\prime}(s)}-(\text{\sc layer}(v(s))-\text{\sc layer}(j)),\\
	\label{Case3Stage213}
	&\hspace{9mm}>k_{v(s),v^{\prime}(s)}-k_{v(s),j},\\
	\label{Case3Stage214}
	&\hspace{9mm}=k_{j,v^{\prime}(s)},
\end{align}
where (\ref{Case3Stage213}) follows from substituting (\ref{Case3Stage29}) in (\ref{Case3Stage212}).  Continuing this series of inequalities gives:
\begin{align}
	\label{Case3Stage215}
	k_{j,v^{\prime}(s)}&<\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s)),\\
	\label{Case3Stage216}
	&=\text{\sc layer}^{\prime}(j)-\text{\sc layer}^{\prime}(v^{\prime}(s)),
\end{align}
where (\ref{Case3Stage215}) follows from (\ref{Case3Stage214}).  The premise of Claim \ref{disjoint}.1 ensures $v^{\prime}(s)$ as defined in (\ref{Case3v2s}) is non-empty.  By construction $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$.  Therefore (\ref{Case3Stage216}) follows since $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$ is the premise of Claim \ref{disjoint}.1.a.  It follows from (\ref{Case3Stage216}) that (\ref{secondIndexShiftedComplete}) is satisfied.  
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{disjoint}.1.b} \textit{For all $j\in{\bf f}(v(s),v^{\prime}(s))$ and $\text{\sc layer}^{\prime}(j)>\text{\sc layer}(j)$, the $v^{\prime}(s)$ defined in (\ref{Case3v2s}) satisfies (\ref{secondIndexShiftedComplete}).}
\begin{proof}
Consider the following inequalities:
\begin{align}
	\label{Case3newStage21}
	\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s))&\geq k_{v(s),v^{\prime}(s)}-k_{v(s),j},\\
	\label{Case3newStage22}
	&=k_{j,v^{\prime}(s)},
\end{align}  
where (\ref{Case3newStage21}) follows from substituting (\ref{firstIndexCodingShiftedComplete2}) into (\ref{Case3Stage212}) (nothing in (\ref{Case3Stage210})-(\ref{Case3Stage212}) requires $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$).  We have the following inequalities:
\begin{align}
	\label{Case3newStage23}
	k_{j,v^{\prime}(s)}&\leq\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s)),\\
	\label{Case3newStage24}
	&<\text{\sc layer}^{\prime}(j)-\text{\sc layer}^{\prime}(v^{\prime}(s)), 
\end{align}
where (\ref{Case3newStage23}) follows from (\ref{Case3newStage22}), and (\ref{Case3newStage24}) follows because $\text{\sc layer}^{\prime}(j)>\text{\sc layer}(j)$ is the premise of Claim \ref{disjoint}.1.b and (\ref{Case3v2s}) implies $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$.  It follows from (\ref{Case3newStage24}) that (\ref{secondIndexShiftedComplete}) is satisfied.  
\end{proof}

Claim \ref{disjoint}.1.a and Claim \ref{disjoint}.1.b together show that $v^{\prime}(s)$ as defined in (\ref{Case3v2s}) satisfies (\ref{secondIndexShiftedComplete}) for all $j\in{\bf f}(v(s),v^{\prime}(s))$.  For every $j\in{\bf f}(s,v(s))$:
\begin{align}
	\label{Case3Stage217}
	\hspace{-2mm}k_{j,v^{\prime}(s)}&<\text{\sc layer}(j)-\text{\sc layer}(v(s))+k_{v(s),v^{\prime}(s)},\\
	\label{Case3Stage218}
	&=\text{\sc layer}(j)-\text{\sc layer}(v^{\prime}(s)),\\
	\label{Case3Stage219}
	&\leq\text{\sc layer}^{\prime}(j)-\text{\sc layer}^{\prime}(v^{\prime}(s)),
\end{align}
where (\ref{Case3Stage217}) follows by adding $k_{v(s),v^{\prime}(s)}$ to both sides of (\ref{secondIndexShiftedComplete2}) and simplifying $k_{j,v(s)}+k_{v(s),v^{\prime}(s)}=k_{j,v^{\prime}(s)}$, (\ref{Case3Stage218}) follows from (V5) which implies $\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))=k_{v(s),v^{\prime}(s)}$ if $v^{\prime}(s)\in{\bf v}(s)$ and (\ref{Case3v2s}) which implies $v^{\prime}(s)\in{\bf v}(s)$, and (\ref{Case3Stage219}) follows because (\ref{shift2}) implies $\text{\sc layer}^{\prime}(j)\geq\text{\sc layer}(j)$ and (\ref{Case3v2s}) implies $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$.  It follows from Claim \ref{disjoint}.1.a, Claim \ref{disjoint}.1.b, and (\ref{Case3Stage219}) that (\ref{Case3v2s}) satisfies (\ref{secondIndexShiftedComplete}).  For every $j\in{\bf f}(v^{\prime}(s),d)$:
\begin{align}
	\label{Case3Stage220}
	\hspace{-2mm}k_{v^{\prime}(s),j}&\geq\text{\sc layer}(v(s))-\text{\sc layer}(j)-k_{v(s),v^{\prime}(s)},\\
	\label{Case3Stage221}
	&=\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(j),\\
	\label{Case3Stage222}
	&\geq\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(j),
\end{align}
where (\ref{Case3Stage220}) follows by subtracting $k_{v(s),v^{\prime}(s)}$ from (\ref{firstIndexCodingShiftedComplete2}) and simplifying $k_{v(s),j}-k_{v(s),v^{\prime}(s)}=k_{v^{\prime}(s),j}$, (\ref{Case3Stage221}) follows from (V5) which implies $\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))=k_{v(s),v^{\prime}(s)}$ if $v^{\prime}(s)\in{\bf v}(s)$ and (\ref{Case3v2s}) which implies $v^{\prime}(s)\in{\bf v}(s)$, and (\ref{Case3Stage222}) follows because (\ref{shift2}) implies $\text{\sc layer}^{\prime}(j)\geq\text{\sc layer}(j)$ and (\ref{Case3v2s}) implies $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$.  It follows from (\ref{Case3Stage222}) that $v^{\prime}(s)$ as defined in (\ref{Case3v2s}) satisfies (\ref{firstIndexCodingShiftedComplete}) which completes the proof of Claim \ref{disjoint}.1.
\end{proof}

To complete the proof of Lemma \ref{disjoint}, fix $i\in A_{l}(S)\setminus A_{l}(U)$.  First, we show that the premises of Lemma \ref{disjoint} satisfy the premises of Claim \ref{disjoint}.1.  It follows from (\ref{A}) and (\ref{shift2}) that $i\in{\bf v}(s)$ for some $s\in S\setminus U$.  Moreover, (\ref{A}) and (\ref{shift2}) imply that $i\notin{\bf v}(\tilde{s})$ for all $\tilde{s}\in U$.  It follows from (\ref{shift2}) that $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ which satisfies the premise of Claim \ref{disjoint}.1, that $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$ for some $j\in{\bf v}(s)$ and $s\notin U$.  Therefore $v^{\prime}(s)$ satisfies (\ref{Case3v2s}).  Finally, we have the following equalities for any $i\in{\bf v}(s)$ and $s\in S\setminus U$:
\begin{align}
	\nonumber
	&\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)\\
	\label{Case3Stage223}
	&\hspace{10mm}=\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(i),\\
	\label{preCase3Stage224}
	&\hspace{10mm}=(\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)})-\text{\sc layer}(i),\\
	\nonumber
	&\hspace{10mm}=(\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)})\\
	\label{Case3Stage224}
	&\hspace{33mm}\hspace{4mm}-(\text{\sc layer}(v(s))-k_{v(s),i}),\\
	\label{Case3Stage225}
	&\hspace{10mm}=k_{v(s),i}-k_{v(s),v^{\prime}(s)}\\
	\label{Case3Stage226}
	&\hspace{10mm}=k_{v^{\prime}(s),i}.
\end{align}
where (\ref{Case3Stage223}) follows because $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ as shown previously and (\ref{Case3v2s}) implies $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$, (\ref{preCase3Stage224}) follows from (V5) since (\ref{Case3v2s}) implies $v^{\prime}(s)\in{\bf v}(s)$, (\ref{Case3Stage224}) follows from (V5) since  $i\in{\bf v}(s)$ by assumption, and (\ref{Case3Stage225}) follows from simplifying.  Since $i\in{\bf v}(s)$ by assumption and $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ as shown previously, it follows from (\ref{Case3v2s}) that $v^{\prime}(s)\in{\bf v}(s)$ and $k_{v(s),i}>k_{v(s),v^{\prime}(s)}$.  Therefore (\ref{Case3Stage226}) follows from (\ref{Case3Stage225}).  It follows from (\ref{Case3Stage226}) and (V5) that $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.

Since $i\in A_{l}(S)\setminus A_{l}(U)$, it follows that $\text{\sc layer}(i)=l$.  Moreover, $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$, which implies $\text{\sc layer}^{\prime}(i)=l$.  By definition in (L5), $i\in L^{\prime}_{l}$ if and only if $\text{\sc layer}^{\prime}(i)=l$.  Since $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$ and $i\in L^{\prime}_{l}$, it follows from (\ref{Aprime}) that $i\in A^{\prime}_{l}(S)$.
\end{proof}


==> flowdecomp 2/fd.tex <==
\section{Flow Decomposition}
\label{FlowDecomposition}
%Let ${\cal N}=\{1,\ldots,|{\cal N}|\}$ denote the set of all nodes in the channel.  Assume that all nodes are sources and each node is a destination for some subset of sources.  Let ${\bf y}_{\cal N}:=(y_{1},\ldots,y_{|{\cal N}|})$ and ${\bf x}_{\cal N}:=(x_{1},\ldots,x_{|{\cal N}|})$.  The input-output dynamics conform to the discrete memoryless channel:
%\begin{align}
%	\label{discretememorylesschannel}
	%\nonumber
%	(\displaystyle\prod_{i\in {\cal N}}{\cal X}_{i},\hspace{1mm}p({\bf y}_{\cal N}|{\bf x}_{\cal N}),\displaystyle\prod_{i\in{\cal N}}{\cal Y}_{i}).
%\end{align}


%\begin{align}
%	\nonumber
%	\text{Prob}({\bf s})&=\text{Prob}({\bf z}_{i_{1}},{\bf z}_{i_{2}},\ldots,{\bf z}_{i_{l}})\\
%	\nonumber
%	&=\prod^{n}_{k=1}p(z_{i_{1},k},z_{i_{2},k},\ldots,z_{i_{l},k}).	
%\end{align}
%In the decode-forward setting, messages \textit{hop} from node to node.    %\textit{Encoding delays} are by definition, the difference between the blocks in which sources and relays transmit the same messages.     
%Two fundamentally different categories of decode-forward schemes exist: one based on correlated input distributions and super-position coding \cite{GamalCover}\cite{XieMultiLevel}, the other based on independent input distributions and index coding \cite{Xie2007}.  Both generate rate regions with similar structure and have their respective advantages, but neither is universally better than the other.  This paper only examines index-coding decode-forward schemes.

The \textit{flow} ${\bf f}(s)$ describes both the sequence of nodes along which messages from source $s$ are relayed through the network and the corresponding one-hop encoding delays.  %Messages either reach all of the network (in all-cast channels) or some of the network (in multi-cast channels).  
Formally, ${\bf f}(s):=N_{1}\xrightarrow{k_{1}}N_{2}\xrightarrow{k_{2}}\cdots\xrightarrow{k_{e_{s}-1}}N_{e_{s}}$ where: 

({F1}) $N_{1}:=\{s\}$ and $s\in{\cal N}$,

({F2}) $N_{l}\subseteq{\cal N}$ and $N_{l}\cap N_{q}=\{\null\}$ for all $1\leq l\neq q\leq e_{s}$, 

 ({F3}) $k_{l}\in\mathbb{N}$ is a one-hop encoding delay for $l=1,\ldots,e_{s}$,

(F4) $i\in{\bf f}(s)$ if and only if $i\in N_{l}$ for some $l=1,\ldots,e_{s}$,

({F5}) ${\bf f}(s,i):=N_{1}\xrightarrow{k_{1}}N_{2}\xrightarrow{k_{2}}\cdots\xrightarrow{k_{l-2}}N_{l-1}$ and \\
\text{\hspace{10mm}} $k_{s,i}:=\sum^{l-1}_{q=1}k_{q}$ if $i\in N_{l}$ for some $l=1,\ldots,e_{s}$.

%By definition, node $j$ is \textit{upstream} of node $i$ in ${\bf f}(s)$ if $k_{s,j}<k_{s,i}$ and \textit{downstream} of node $i$ if $k_{s,j}>k_{s,i}$.

In each \textit{block} of $n$ channel uses, sources generate new messages, and relays forward messages from previous blocks.  Transmission occurs over $B$ blocks.  The flows ${\bf F}=\{{\bf f}(s):s\in{\cal N}\}$ form a multi-edge directed graph on ${\cal N}$ that determines  the encoded messages in each block.  For a fixed rate vector ${\bf R}=(R_{1},\ldots,R_{|{\cal N}|})$,  the codebooks are generated as follows:
\begin{itemize}
	\item For each node $i\in{\cal N}$ independently generate  $2^{n\sum_{s:i\in{\bf f}(s)}R_{s}}$ $n$-length codewords ${\bf x}_{i}(w)$ according to the distribution $p(x)$ over $x\in{\cal X}_{i}$ where $w\in\{1,\ldots,2^{n\sum_{s:i\in{\bf f}(s)}R_{s}}\}$.
\end{itemize}
The encoding proceeds as follows for each $b\in\{1,\ldots,B\}$:
\begin{itemize}
	\item In block $b$, source $s$ generates the message $m_{s}(b)\in\{1,\ldots,2^{nR_{s}}\}$
	\item In block $b$, node $i$ transmits the codeword ${\bf x}_{i}(w(b))$ where $w(b)\in\{1,\ldots,2^{n(\sum_{s:i\in{\bf f}(s)}R_{s})}\}$ is the index assigned to the message vector ${\bf w}(b):=(w_{1},\ldots,w_{|{\cal N}|})$ and:
\begin{align}
\label{dubenc}
w_{s}=\begin{cases}m_{s}(b-k_{s,i})&i\in {\bf f}(s)\\ ``1" & i\notin {\bf f}(s)\text{ or }b-k_{s,i}\leq 0\end{cases}	
\end{align}
\end{itemize}
%In block $b$, source $s$ generates the message $m(b)\in\{1,\ldots,2^{nR_{s}}\}$ and node $i\in{\cal Z}$ sends the index $w_{i}(b)\in\{1,\ldots,2^{n(\sum_{s\in{\cal  S}_{i}}R_{s})}\}$ assigned to the message vector 
%\begin{align}
%\label{doubleudb}
%\bar{w}_{d}(b):=\{\langle s,m(b-k_{s,d})\rangle: s\in{\cal S}_{d}\}	.
%\end{align}

%The codebook at node $i\in{\cal Z}$ consists of $2^{n\sum_{s\in{\cal S}_{i}}R_{s}}$ $n$-length codewords independently generated according to the distribution $p(x)$ over $x\in{\cal X}_{i}$.  The index $w\in\{1,\ldots,2^{n\sum_{s\in{\cal S}_{i}}R_{s}}\}$ maps to a unique codeword ${\bar x}_{i}(w)$.  In block $b$, node $i$ transmits the codeword ${\bar x}_{i}(w_{i}(b))$.

In each block, the relays decode source messages.  To simplify the analysis,   assume each node encodes the same set of sources that it decodes, and   define:
\begin{align}
	\label{sd}
	{\cal S}(d)&:=\{s:d\in{\bf f}(s)\}.
\end{align}  
Observe that ${\cal S}(d)$ denotes the set of sources encoded (and thus decoded) by node $d\in{\cal N}$.  

For any subset $S\subseteq{\cal N}$, let $F_{d}(S):=\{i\in{\bf f}(s,d):S\cap{\cal S}(d)\}$.  The messages decoded by node $d$ in each block correspond to ordered partitions or  \textit{layerings} of $F_{d}({\cal N})$, all the nodes upstream of (or preceding) node $d$.  A layering ${\bf L}_{d}:=(L_{0},\ldots,L_{|{\bf L}_{d}|-1})$ satisfies the following conditions: 
 
({L1})  $L_{l}\subseteq F_{d}({\cal N})$ for every $l=0,\ldots,|{\bf L}_{d}|-1$,

({L2}) $L_{l}\cap L_{q}=\{\}$ for $l\neq q$,

({L3}) $F_{d}({\cal N})=\cup^{|{\bf L}_{d}|-1}_{l=0}L_{l}$,

({L4}) $L_{|{\bf L}_{d}|-1}\neq\{\}$,

({L5}) $\text{\sc layer}(i):=l$ by definition if $i\in L_{l}$.  

Each layer corresponds to previous block of channel uses.  %A flow decomposition at node $d$ denoted by $({\bf F},{\bf L}_{d})$ is a flow set and a layering that in each block  defines, respectively, the messages encoded at all nodes and the messages decoded by node $d$.  
It is convenient to associate with $({\bf F},{\bf L}_{d})$ a \textit{virtual source} $v(s)$ and a \textit{virtual flow} ${\bf v}(s)$ for each $s\in{\cal S}(d)$, where ${\bf v}(s)$ is a subsequence of ${\bf f}(s)$.  Virtual sources and flows are the sources and flows ``seen'' by node $d$ given the layering ${\bf L}_{d}$.    Different layerings change how node $d$ decodes messages from nodes in $F_{d}({\cal N})$.

For each $s\in{\cal S}(d)$, define the function $u(s,i):=\text{\sc layer}(i)+k_{s,i}$ and the node subset $M(s):=\{\arg\min_{i\in{\bf f}(s,d)}u(s,i)\}$.  The virtual source $v(s)$ corresponding to $s$ is defined as:
\begin{align}
\label{vs}
v(s)&:=\{\arg\min_{i\in M(s)}k_{s,i}\}.  	
\end{align}
Suppose $d\in N_{e_{s,d}+1}$ for some $1\leq e_{s,d}\leq e_{s}$ and, per (F5), ${\bf f}(s,d):=N_{1}\xrightarrow{k_{1}}N_{2}\xrightarrow{k_{2}}\cdots\xrightarrow{k_{e_{s,d}-1}}N_{e_{s,d}}$.  By construction $v(s)\subseteq N_{l}$ for some $l=1,\ldots,e_{s,d}$.  The virtual flow ${\bf v}(s):= N^{\prime}_{1}\xrightarrow{k^{\prime}_{1}} N^{\prime}_{2}\xrightarrow{k^{\prime}_{2}}\cdots N^{\prime}_{p}$ is the subsequence of ${\bf f}(s,d)$ that satisfies the following conditions: 

({V1}) $N^{\prime}_{1}:=\{v(s)\}$,

({V2}) $N^{\prime}_{l}\subseteq N_{z_{l}}$ where $1\leq l\leq p$ and $z_{1}, z_{2},\ldots, z_{p}$ is a 

\hspace{7.5mm}subsequence of $1, 2,\ldots, e_{s,d}$, 

({V3}) $k^{\prime}_{l}=\sum^{z_{l+1}-1}_{q=z_{l}}k_{q}$,

({V4})  $i\in{\bf v}(s)$ implies $i\in N^{\prime}_{l}$ for some $1\leq l\leq p$, 

({V5}) $\text{\sc layer}(v(s))-\text{\sc layer}(i)=k_{v(s),i}$ for all  $i\in{\bf v}(s)$ 

\hspace{8mm}where $k_{v(s),i}:=k_{s,i}-k_{s,v(s)}$ as per (F5).

There is a convenient way of checking whether or not a particular node is in fact the virtual source of a given flow.

\input{"clocksecurity.tex"}

%and  
%\begin{align}
%\label{virtualflow}
%\nonumber
%\text{\sc layer}(v(s))-\text{\sc layer}(i)=k_{v(s),i},
%\end{align}

%\hspace{8mm}where $k_{v(s),i}:=k_{s,i}-k_{s,v(s)}$ as per (F5).

In block $b$, node $d$ decodes the message vector ${\bf m}(b):=(m_{1},\ldots,m_{|{\cal N}|})$ where
\begin{align}
\label{emdb}
m_{s}:=\begin{cases}
m_{s}(b-k_{s,v(s)}-\text{\sc layer}(v(s)))& s\in{\cal S}(d)\\
``1" & s\notin {\cal S}(d),\end{cases}
\end{align}
and $m_{s}:= ``1"$ if $b-k_{s,v(s)}-\text{\sc layer}(v(s))\leq0$.  Define: 
\begin{align}
\label{id}
I(d)&:=\{i:{\cal S}(i)\subseteq{\cal S}(d)\}.	
\end{align}
Observe that (\ref{id}) denotes the set of relays that only encode sources decoded by node $d$.  For every $S\subseteq{\cal N}$ and $0\leq l\leq|{\bf L}_{d}|-1$, let: 
\begin{align}
\label{A}
A_{l}(S)&:=\{i\in{\bf v}(s):s\in S\cap{\cal S}(d)\}\cap L_{l},\\
\label{Atilde}
	\tilde{A}_{l}(S)&:=(\cup_{i\in I(d)}F_{i}({\cal N}))\setminus(\cup^{|{\bf L}_{d}|-1}_{q=l+1}L_{q}\cup A_{l}(S)).
\end{align}

To decode ${\bf m}(b)$, node $d$ finds the message vector ${\bf\hat{m}}(b):=(\hat{m}_{1},\ldots,\hat{m}_{|{\cal N}|})$ that satisfies the following typicality checks for $0\leq l\leq |{\bf L}_{d}|-1$:
\begin{align}
\nonumber
	&\hspace{-3.2mm}(\{{\bf x}_{i}(\hat{w}(b-l)):i\in A_{l}({\cal N})\}, \{{\bf X}_{i}(b-l):i\in\tilde{A}_{l}({\cal N})\},\hspace{4.5mm}\\
\label{tippie}
	&\hspace{21mm}{\bf Y}_{d}(b-l))\in T^{(n)}_{\epsilon}(X_{A_{l}({\cal N})\cup\tilde{A}_{l}({\cal N})},Y_{d})
\end{align}
where ${\bf X}_{i}(b-l)$ is the sequence sent by node $i$ in block $b-l$ and ${\bf Y}_{d}(b-l)$ is the sequence received by node $d$ in block $b-l$.  For all $i\in A_{l}({\cal N})$ and ${\bf x}_{i}(\hat{w}(b-l))$, $\hat{w}(b-l)$ is the index that maps to ${\bf\hat{w}}(b-l):=(\hat{w}_{1},\ldots,\hat{w}_{|{\cal N}|})$ where:
\begin{align}
\label{dubdb}
\hat{w}_{s}:=\begin{cases}
\hat{m}_{s}& i\in{\bf v}(s)\\
m_{s}(b-l-k_{s,i})&i\notin{\bf v}(s)\text{ and }i\in{\bf f}(s)\\ 
``1" & i\notin {\bf f}(s).\end{cases}	
\end{align}

The index $\hat{m}_{s}$ is the message to be decoded in block $b$, that is, $m_{s}(b-k_{s,v(s)}-\text{\sc layer}(v(s)))$ as given in (\ref{emdb}).  The message actually encoded in $w(b-l)$ is $m_{s}(b-l-k_{s,i})$ as given in (\ref{dubenc}).  These messages must be the same in order for the scheme to work.  If $i\notin{\bf v}(s)$ but $i\in{\bf f}(s)$ then $m_{s}(b-l-k_{s,i})$ must be already known to node $d$ (decoded in some previous block).  If $i\notin{\bf f}(s)$ then node $i$ encodes ``1'' in place of messages from source $s$ as per (\ref{dubenc}).  Observe that (\ref{A}) and (\ref{Atilde}) imply:
\begin{align}
\label{AN}
A_{l}({\cal N})&=\{i\in{\bf v}(s):s\in {\cal S}(d)\}\cap L_{l},\\
\label{AtildeN}
	\tilde{A}_{l}({\cal N})&=(\cup_{i\in I(d)}F_{i}({\cal N}))\setminus(\cup^{|{\bf L}_{d}|-1}_{q=l+1}L_{q}\cup A_{l}({\cal N})).
\end{align}

There are five conditions that must be satisfied in order for the typicality checks to be feasible.  The first follows from causality and the rest are  index-coding primitives.  

An encoding/decoding scheme is causal if in block $b$, each relay only encodes source messages it decoded in previous blocks.  The messages encoded and decoded by node $d$ in block $b$ are defined by (\ref{dubenc}) and (\ref{emdb}) respectively.

(C1) For every $s\in{\cal S}(d)$:
\begin{align}
\label{causal}
	b-k_{s,d}<b-k_{s,v(s)}-\text{\sc layer}(v(s)).
\end{align}
It is convenient to simplify (\ref{causal}):
\begin{align}
\label{causal2}
	\text{\sc layer}(v(s))<k_{v(s),d},
\end{align}
which yields the causality constraints in (\ref{outline2}).  The next condition pertains to the flow itself, and states that node $d$ must decode or know all sources encoded in node $i$ to decode any one source encoded in node $i$.   

(C2) For every $s\in{\cal S}(d)$ and $i\in {\bf f}(s,d)$:
\begin{align}
\label{C1}
{\cal S}(i)\subseteq {\cal S}(d).
\end{align}
 
Two flow types of interest that satisfy (C2) are all-cast channels, in which all nodes decode all sources, and multi-cast channels with hierarchical (or tree structured) flow, in which messages proceed from the branches to the root.  

The remaining conditions ensure that (\ref{dubenc})-(\ref{AtildeN}) are consistent.  Comparing (\ref{dubenc}), (\ref{emdb}), (\ref{tippie}) and (\ref{dubdb}), the messages decoded by node $d$ in block 
$b$ must match the corresponding messages encoded by node $i$ in block $b-l$.

(C3) Suppose $i\in{\bf f}(s)$ and $i\in A_{l}({\cal N})$ for some $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$.  If $i\in{\bf v}(s)$ then:
\begin{align}
\label{C2}
	b-l-k_{s,i} = b-k_{s,v(s)}-\text{\sc layer}(v(s)).
\end{align}

Again comparing (\ref{dubenc}), (\ref{emdb}), (\ref{tippie}) and (\ref{dubdb}), any messages not decoded by node $d$ in block $b$ but encoded by node $i$ in block $b-l$, must already be known by node $d$ in some previous block.

(C4) Suppose $i\in{\bf f}(s)$ and $i\in L_{l}$ for some $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$.  If $i\notin{\bf v}(s)$ then:
\begin{align}
\label{C3}
	b-l-k_{s,i} < b-k_{s,v(s)}-\text{\sc layer}(v(s)).
\end{align}

Finally, comparing (\ref{dubenc}), (\ref{emdb}) and (\ref{tippie}), the sequences in $\{{\bf X}_{i}(b-l):i\in\tilde{A}_{l}({\cal N})\}$, which are side information in (\ref{tippie}), must only encode messages known to node $d$.

(C5) Suppose $i\in{\bf f}(s)$ and $i\in\tilde{A}_{l}({\cal N})$ for some $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$.  Then:
\begin{align}
	b-l-k_{s,i} < b-k_{s,v(s)}-\text{\sc layer}(v(s)).
\end{align}

%The previous typicality checks are valid if it can verified for all $0\leq l\leq |\bar{L}_{d}|-1$ and $i\in F_{d}({\cal S})$ that $\bar{m}_{d}(b)$ splits $\bar{w}_{i}(b-l)$ into a set of messages that node $d$ decodes in block $b$ and a set of messages that node $d$ knows from its side information.  Let $A_{l}:=\{i:\bar{w}_{i}(b-l)\cap\bar{m}_{d}(b)\neq\{\}, \bar{w}_{i}(b-l)\subseteq\cup^{b}_{q=1}\bar{m}_{d}(q)\}$ and $\tilde{A}_{l}:=\{i:\bar{w}_{i}(b-l)\subseteq\cup^{b-1}_{q=1}\bar{m}_{d}(q)\}$.  Equivalently, $\tilde{A}_{l}:=\{i:\bar{w}_{i}(b-l)\subseteq\cup^{b}_{q=1}\bar{m}_{d}(q)\}\setminus A_{l}$.  If $L_{d,l}\subseteq A_{l}\cup\tilde{A}_{l}$ for every $0\leq l\leq |\bar{L}_{d}|-1$, then $\bar{m}_{d}(b)$ is a \textit{splitting vector}.

\begin{figure*}[t]
        \center{\includegraphics[width=\textwidth]
        {./Figures/hierarchicalallcast}}
        \caption{(i) Hierarchical flows ${\bf F}=\{{\bf f}(1),{\bf f}(3),{\bf f}(4),{\bf f}(5),{\bf f}(7),{\bf f}(9),{\bf f}(10),{\bf f}(16),{\bf f}(18),{\bf f}(19), {\bf f}(21)\}$ where ${\bf f}(1)=1\xrightarrow{1}2\xrightarrow{3}12\xrightarrow{2}23\xrightarrow{9}26\xrightarrow{12}30$, ${\bf f}(3)=3\xrightarrow{5}13\xrightarrow{1}26\xrightarrow{2}30$, ${\bf f}(4)=4\xrightarrow{8}14\xrightarrow{1}21\xrightarrow{6}26\xrightarrow{9}30$, ${\bf f}(5)=5\xrightarrow{37}\{6,15\}\xrightarrow{17}16\xrightarrow{6}25\xrightarrow{18}28\xrightarrow{1}30$, ${\bf f}(7)=7\xrightarrow{2}17\xrightarrow{27}24\xrightarrow{1}28\xrightarrow{2}30$, ${\bf f}(9)=9\xrightarrow{19}8\xrightarrow{7}18\xrightarrow{3}27\xrightarrow{2}29\xrightarrow{5}30$, ${\bf f}(10)=10\xrightarrow{8}11\xrightarrow{13}19\xrightarrow{2}20\xrightarrow{1}22\xrightarrow{11}29\xrightarrow{2}30$, ${\bf f}(16)=16\xrightarrow{2}25\xrightarrow{1}28\xrightarrow{7}30$, ${\bf f}(18)=18\xrightarrow{2}27\xrightarrow{4}29\xrightarrow{1}30$, ${\bf f}(19)=19\xrightarrow{1}20\xrightarrow{5}22\xrightarrow{3}29\xrightarrow{1}30$, and ${\bf f}(21)=21\xrightarrow{5}26\xrightarrow{2}30$. (ii) All-cast flows ${\bf F}=\{{\bf f}(3),{\bf f}(5),{\bf f}(14),{\bf f}(18)\}$ where ${\bf f}(3)=9\xrightarrow{9}11\xrightarrow{5}10\xrightarrow{14}6\xrightarrow{19}4\xrightarrow{11}5\xrightarrow{13}7\xrightarrow{4}8\xrightarrow{18}9\xrightarrow{6}19\xrightarrow{1}18\xrightarrow{23}17\xrightarrow{14}16\xrightarrow{5}15\xrightarrow{12}14\xrightarrow{32}13\xrightarrow{57}12\xrightarrow{99}1\xrightarrow{71}2$, ${\bf f}(5)=5\xrightarrow{6}6\xrightarrow{1}11\xrightarrow{9}10\xrightarrow{19}7\xrightarrow{7}8\xrightarrow{17}9\xrightarrow{13}18\xrightarrow{6}19\xrightarrow{47}16\xrightarrow{7}15\xrightarrow{9}14\xrightarrow{13}13\xrightarrow{10}1\xrightarrow{2}2\xrightarrow{64}3\xrightarrow{8}\{4,12\}$, ${\bf f}(14)=14\xrightarrow{3}13\xrightarrow{17}15\xrightarrow{9}16\xrightarrow{13}12\xrightarrow{5}11\xrightarrow{15}6\xrightarrow{29}10\xrightarrow{21}19\xrightarrow{42}17\xrightarrow{1}18\xrightarrow{36}9\xrightarrow{31}8\xrightarrow{29}7\xrightarrow{18}5\xrightarrow{9}4\xrightarrow{16}3\xrightarrow{7}2\xrightarrow{22}1$, ${\bf f}(18)=18\xrightarrow{3}\{9,17\}\xrightarrow{1}19\xrightarrow{7}10\xrightarrow{13}8\xrightarrow{9}7\xrightarrow{8}5\xrightarrow{11}6\xrightarrow{19}11\xrightarrow{4}4\xrightarrow{17}3\xrightarrow{27}2\xrightarrow{23}1\xrightarrow{15}13\xrightarrow{39}14\xrightarrow{17}15\xrightarrow{3}16$.}
        \label{hierarchicalallcast}
 \end{figure*}

\input{"splitting.tex"}

  For any rate vector ${\bf R}:=(R_{1},\ldots,R_{|{\cal N}|})$ and some subset $S\subseteq{\cal S}(d)$, let $R_{S}=\sum_{s\in S} R_{s}$.  Lemma \ref{splitting} implies the encoding/decoding scheme defined by (\ref{dubenc})-(\ref{AtildeN}) is well-defined contingent on (C1) and (C2).  For the product distribution $\{\Pi^{|{\cal N}|}_{i=1}p(x_{i}):x_{i}\in{\cal X}_{i},i=1,\ldots,|{\cal N}|\}$, it follows from (\ref{tippie}) that the probability node $d$ decodes some subset of sources $S\subseteq{\cal S}(d)$ incorrectly, goes to zero if the following constraint is satisfied:

\begin{align}
\label{flowdecomp}
R_{S}<\displaystyle\sum^{|{\bf L}_{d}|-1}_{l=0}I(X_{A_{l}(S)};Y_{d}|X_{\tilde{A}_{l}(S)}).
\end{align}

Let ${\cal R}({\bf F},{\bf L}_{d})$ denote the region of rate vectors that satisfy (\ref{flowdecomp}) for every $S\subseteq{\cal S}(d)$.

%\input{flows}

\section{Main Result}
\label{mainresult}
For any subset $S\subseteq{\cal N}$, recall that $F_{d}(S):=\{i\in{\bf f}(s,d):s\in S\cap{\cal S}(d)\}$ and let $\tilde{F}_{d}(S):=(\cup_{i\in I(d)}F_{i}({\cal N}))\setminus F_{d}(S)$.  For the product distribution $\{\Pi^{|{\cal N}|}_{i=1}p(x_{i}):x_{i}\in{\cal X}_{i},i=1,\ldots,|{\cal N}|\}$, let ${\cal R}_{d}({\bf F})$ denote the set of rate vectors that satisfy the following constraint for all subsets $S\subseteq{\cal S}(d)$:
\begin{align}
\label{biggiewiggie}
	R_{S}<I(X_{F_{d}(S)};Y_{d}|X_{\tilde{F}_{d}(S)}).
\end{align}   
Since $F_{d}(S)$ includes all the nodes upstream of node $d$, that encode the sources $S$, and $\tilde{F}_{d}(S)$ includes all the nodes downstream of node $d$ as well as the remaining nodes in $F_{d}({\cal N})$, it follows that (\ref{biggiewiggie}) is is an upper-bound on the decode-forward achievable sum rate at node $d$.
%, not only for the class of regular decode-forward schemes defined by (\ref{dubenc})-(\ref{AtildeN}), but for all decode-forward schemes in general, including those based on backward-decoding.  An important caveat is that (\ref{biggiewiggie}), as an outer-bound, applies to all input distributions $p(x_{1},\ldots,x_{|{\cal N}|})$ not just the product input distribution used in (\ref{dubenc})-(\ref{AtildeN}).

Two flows ${\bf F}$ and ${\bf F}^{\prime}$ are \textit{equivalent}, by definition, if for every $s\in{\cal N}$, ${\bf f}(s)\in{\bf F}$ and ${\bf f}^{\prime}(s)\in{\bf F}^{\prime}$ differ only in their encoding delays, $\{k_{i}:1\leq i\leq e_{s}\}$ and $\{k^{\prime}_{i}: 1\leq i\leq e_{s}\}$ respectively, but not the node sequences, so that  $N_{i}=N^{\prime}_{i}$ for all $1\leq i\leq e_{s}$ where ${\bf f}(s):=N_{1}\xrightarrow{k_{1}}N_{2}\xrightarrow{k_{2}}\cdots\xrightarrow{k_{e_{s}-1}}N_{e_{s}}$ and ${\bf f}^{\prime}(s):=N^{\prime}_{1}\xrightarrow{k^{\prime}_{1}}N^{\prime}_{2}\xrightarrow{k^{\prime}_{2}}\cdots\xrightarrow{k^{\prime}_{e_{s}-1}}N^{\prime}_{e_{s}}$.  Since (\ref{biggiewiggie}) depends only the nodes in the flows and not the encoding delays, it follows that ${\cal R}_{d}({\bf F})={\cal R}_{d}({\bf F}^{\prime})$ for all $d\in{\cal N}$ and channel statistics $p({\bf y}_{{\cal N}}|{\bf x}_{{\cal N}})$ if ${\bf F}$ and ${\bf F}^{\prime}$ are equivalent.
\begin{theorem}
\label{theoremone}
Fix some $d\in{\cal N}$.  For any ${\bf F}$ satisfying (C2) and ${\bf R}\in{\cal R}_{d}({\bf F})$, there exists an equivalent ${\bf F}^{\prime}$ and ${\bf L}_{d}$ satisfying (C1) and (C2) such that 
${\bf R}\in{\cal R}({\bf F}^{\prime},{\bf L}_{d})$.
\end{theorem}
\begin{proof}
	See Section \ref{prooftheoremone}.
\end{proof}
%Theorem \ref{theoremone} partially confirms the hypothesis that regular-coding schemes collectively achieve the same region as backward-decoding in the decode-forward setting.
  %The independent input distributions in (\ref{flowdecomp}) and (\ref{biggiewiggie}) are a feature of index-coding.  A fundamentally different scheme called super-position coding creates correlated input distributions and is compatible with regular-coding \cite{Sankar}.  
  %Correlated input distributions introduce auxiliary conditional random variables into the mutual information in (\ref{biggiewiggie}) (see \cite{Sankar} and \cite{XieKumar}), and are unambiguously advantageous in broadcast channels unconstrained by (C2).

If ${\bf R}\in\cap^{|{\cal N}|}_{d=1}{\cal R}_{d}({\bf F})$, Theorem \ref{theoremone} does \textit{not} imply that ${\bf R}\in{\cal R}({\bf F}^{\prime},{\bf L}_{d})$ for each $1\leq d\leq |{\cal N}|$ and some ${\bf L}_{d}$ \textit{simultaneously}.  That result only occurs if the flow is hierarchical.  %All-cast channels are more complicated and require algorithmic methods to verify (C1) simultaneously for all $d\in{\cal N}$. 

%For the purpose of this argument, we can relax the assumption that node $d$ is silent.  Given ${\bf F}$, the outer-bound (\ref{biggiewiggie}) has complexity $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$; any achievable rate ${\bf R}$ in the class must simultaneously satisfy $2^{|{\cal S}|}$ different $S$-induced cut-set constraints defined by (\ref{biggiewiggie}) at each node $d\in{\cal N}$. 

%The outer-bound is actually achievable for arbitrary encoding delays, provided non-causal decoding is allowed (as implied by Theorem \ref{theoremone}).  This ``achievable region'' (or pseudo inner-bound) still has $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$ time complexity.  The proof of Theorem \ref{theoremone} fixes some ${\bf R}\in{\cal R}({\bf F})$ and constructs a sequence of flow decompositions $\{({\bf F},{\bf L}_{k}):k\in\mathbb{N}\}$ that converges in $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$ time to some $({\bf F},{\bf L}_{k*})$ where ${\bf R}\in{\cal R}({\bf F},{\bf L}_{k^{*}})$.  
%collectively achieve the regional cut-set extension of the one-relay decode-forward rate; given any arbitrary set of ``weighted'' flows, node $d$ can support any desired rate-vector in ${\cal R}({\bf F})$ by decoding the message vector ${\bf m}(b)$ corresponding to some flow decomposition $({\bf F}, {\bf L})$ at node $d$.  Regular encoding/decoding avoids the exponential delays \cite{Sankar} and artificial restrictions on bidirectional flow \cite{XieKumar} imposed by backward decoding.  
%With causality fully enforced, the actual achievable region splits into two extremal cases: multi-cast channels with hierarchical flow and all-cast channels with arbitrary flow.  Related work shows the former case (unlike the latter) does not alter the complexity of the achievable region.

%Decode-forward and compress-forward schemes share a deeper symmetry (compare the statements and proofs of Theorems \ref{theoremone} and \cite{compdecomp}:(Theorem 1)) inherent in the submodular structure of their boundary constraints.  %This duality also has implications for combinatorial optimization.  Given any rate-vector ${\bf R}\in{\cal R}({\bf F})$ the proof constructs a ``shifted'' sequence of layered partitions that converges to ${\bf R}$ after at most a linear number of shifts in $|F({\cal S})|$, where the space of layered partitions is factorial in $|F({\cal S})|$.  The proof exploits the submodular structure in mutual information inequalities.

%Flow decomposition solves a more general information-theoretic variation of the index coding problem.  The conventional formulation \cite{indexcoding} assumes a sender and a set of receivers with assigned side information, and attempts to characterize the minimum rate of the sender's common message that noiselessly delivers the appropriate missing information to each of the receivers,  for all side information assignments.  

%The more general variation of this problem introduces encoding delays and the discrete memoryless channel.  Given a set of senders  ${\cal S}$ and a single receiver node $d$ (as opposed to a single sender and a set of receivers), a flow set ${\bf F}$ which assigns messages to each sender, and a desired rate-vector ${\bf R}\in{\cal R}({\bf F})$, Theorem \ref{theoremone} determines the ``side information assignment'' $\{\cup^{b-1}_{q=0}{\bf m}(q)\}$ of previously decoded messages implied by $({\bf F},{\bf L})$, that enables node $d$ to extract the missing information at the desired rates through the noisy channel.  The general variation yields closed-form solutions, even though the conventional formulation does not.  
  


==> flowdecomp 2/grandefinale.tex <==
\begin{lemma}
	\label{grandefinale}
	${\bf R}\in{\cal R}({\bf F},{\bf L}_{d,n^{*}})$ for some $n^{*}\in\mathbb{N}$.
\end{lemma}

\begin{proof}
	The proof is by contradiction.  We prove some initial claims, but first introduce a classical definition of the limit inferior of any sequence of sets $\{S_{n}:n\in\mathbb{N}\}$.
\begin{align}
	\label{liminf}
	\liminf_{n} S_{n}&:=\cup^{\infty}_{n=1}\cap^{\infty}_{q=n}S_{q}.
\end{align} 
	
\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.1} \textit{$\liminf\limits_{n} U_{n}\neq\{\}$.}
\begin{proof}
The proof is by contradiction.  Suppose $\liminf_{n}U_{n}=\{\}$ and Lemma \ref{grandefinale} is false.  If Lemma \ref{grandefinale} is false then $Z_{n}\neq{\cal S}(d)$ for all $n\in\mathbb{N}$.  For every $s\in{\cal S}(d)$, it follows from (\ref{liminf}) and the hypothesis $\liminf_{n}U_{n}=\{\}$ that some $n_{s}$ exists such that $s\notin U_{n_{s}}$.  Therefore (\ref{inductionupdate}) implies that $s\in Z_{n_{s}+1}$.  Moreover, (\ref{inductionupdate}) also implies $Z_{n}\subseteq Z_{n+1}$ for all $n\in\mathbb{N}$.  It follows that $Z_{n}={\cal S}(d)$, for all $n\geq\max_{s\in{\cal S}(d)}n_{s}$, which contradicts the hypothesis that $Z_{n}\neq{\cal S}(d)$ for all $n\in\mathbb{N}$.
\end{proof}

%\input{"grandefinaleclaim2.tex"}


\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.2} \textit{If $i\in{\bf v}_{n}(s)$ for some $s\in U_{n}$ then $i\in{\bf v}_{n+1}(s)$.}

\begin{proof}
There are two cases to consider.  If $v_{n+1}(s)=v_{n}(s)$ then Claim \ref{join}.1 implies $i\in{\bf v}_{n+1}(s)$.  Otherwise, if $v_{n+1}(s)\neq v_{n}(s)$ then Claim \ref{join}.2 implies $i\in{\bf v}_{n+1}(s)$.
%We have the following sequence of inequalities:
%\begin{align}
%	\nonumber
%	&\hspace{-3mm}\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
%	\label{grandfinale18}
%	&\hspace{7mm}=\text{\sc layer}_{n+1}(v_{n}(s))-\text{\sc layer}_{n+1}(i),\\
%	\label{grandfinale19}
%	&\hspace{7mm}=(\text{\sc layer}_{n}(v_{n}(s))+1)-(\text{\sc layer}_{n}(i)+1),\\
	%\label{grandfinale20}
%	\nonumber
%	&\hspace{7mm}=\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i),\\
%	\label{grandfinale21}
%	&\hspace{7mm}=k_{v_{n}(s),i},\\
%	\label{grandfinale22}
%	&\hspace{7mm}=k_{v_{n+1}(s),i},
%\end{align}
%where (\ref{grandfinale18}) follows from the premise of Case 1 that $v_{n+1}(s)=v_{n}(s)$, (\ref{grandfinale19}) follows from (\ref{shift4}) and because $s\in U_{n}$ and $i\in{\bf v}_{n}(s)$, (\ref{grandfinale21}) follows from (V5) and the premise of Claim \ref{grandefinale}.2 that $i\in{\bf v}_{n}(s)$, and (\ref{grandfinale22}) follows from the premise of Case 1 that $v_{n+1}(s)=v_{n}(s)$.  Both (\ref{grandfinale22}) and (V5) imply that $i\in{\bf v}_{n+1}(s)$.
%\hspace{-3.5mm}{\bf Case 2:} $v_{n+1}(s)\neq v_{n}(s)$.
%We have the following sequence of inequalities:
%\begin{align}
%	\nonumber
%	&\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
%	\nonumber
%	&\hspace{5mm}=\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(v_{n}(s))\\
%	\label{grandfinale23}
%	&\hspace{19mm}+\text{\sc layer}_{n+1}(v_{n}(s))-\text{\sc layer}_{n+1}(i),\\
%	\nonumber
%	&\hspace{5mm}=k_{v_{n+1}(s),v_{n}(s)}+\text{\sc layer}_{n+1}(v_{n}(s))\\
%	\label{grandfinale24}
%	&\hspace{49mm}-\text{\sc layer}_{n+1}(i),\\
%	\nonumber
%	&\hspace{5mm}=k_{v_{n+1}(s),v_{n}(s)}+(\text{\sc layer}_{n}(v_{n}(s))+1)\\
%	\label{grandfinale25}
%	&\hspace{44mm}-(\text{\sc layer}_{n}(i)+1),\\
	%\label{grandfinale28}
%	\nonumber
%	&\hspace{5mm}=k_{v_{n+1}(s),v_{n}(s)}+(\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)),\\
%	\label{grandfinale26}
%	&\hspace{5mm}=k_{v_{n+1}(s),v_{n}(s)}+k_{v_{n}(s),i},\\
%	\label{grandfinale27}
%	&\hspace{5mm}=k_{v_{n+1}(s),i},
%\end{align}
%where (\ref{grandfinale23}) follows by adding and subtracting $\text{\sc layer}_{n+1}(v_{n}(s))$, (\ref{grandfinale24}) follows from (V5) and because Claim \ref{grandefinale}.3.b implies $v_{n}(s)\in{\bf v}_{n+1}(s)$, (\ref{grandfinale25}) follows from (\ref{shift4}) and because $s\in U_{n}$ and $i\in{\bf v}_{n}(s)$, and (\ref{grandfinale26}) follows from (V5) and the premise of Claim \ref{grandefinale}.2 that $i\in{\bf v}_{n}(s)$.  Both (V5) and (\ref{grandfinale27}) imply that $i\in{\bf v}_{n+1}(s)$ which finishes the proof of Claim \ref{grandefinale}.2 for Case 2.
\end{proof}
We introduce the following definitions: 
\begin{align}
\label{U}
U^{*}&:=\liminf\limits_{n} U_{n},\\
V^{*}_{n}&:=\{i\in{\bf v}_{n}(s):s\in U_{n}\setminus U^{*}\}.
\label{vstar}
\end{align}

\hspace{-3mm}{\bf Claim.\ref{grandefinale}.3} $\liminf\limits_{n}(U_{n}\setminus U^{*})=\{\}$.
\begin{proof}
The proof is by contradiction.  Suppose $\liminf_{n}(U_{n}\setminus U^{*})\neq\{\}$.  For some $s\in{\cal S}(d)$ and $n_{s}\in\mathbb{N}$, it follows that $s\in U_{n}\setminus U^{*}$ for all $n\geq n_{s}$.  Therefore $s\in\cap_{q\geq n_{s}} U_{q}$.  It follows from (\ref{liminf}) and (\ref{U}) that $s\in U^{*}$ which is a contradiction.
\end{proof}

%let $U^{*}:=\liminf\limits_{n} U_{n}$ and $V^{*}_{n}:=\{i\in{\bf v}_{n}(s):s\in U_{n}\setminus U^{*}\}$.
%\begin{align}
%\label{U}
%U^{*}&:=\liminf_{n} U_{n}
%\end{align}
%Define the sequence of sets $\{U^{*}_{n}:n\in\mathbb{N}\}$ as follows:
%\begin{align}
%	\label{ustar}
%	U^{*}_{n}:=U_{n}\setminus U^{*}.
%\end{align}
%By construction, there is no $s\in{\cal S}(d)$ such that $s\in U^{*}_{n}$ for all $n\geq n_{s}$ and some $n_{s}\in\mathbb{N}$ (if such an $s$ exists then $U\cup\{s\}\subseteq U_{n}$ for all $n\geq\max\{n_{U},n_{s}\}$ which contradicts the definition of $U$ as the largest such subset).  
%Define the sequence of sets $\{V^{*}_{n}:n\in\mathbb{N}\}$ as follows: 
%\begin{align}
%\label{vstar}
%V^{*}_{n}&:=\{i\in{\bf v}_{n}(s):s\in U^{*}_{n}\}.	
%\end{align}

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.4} \textit{$\liminf\limits_{n}V^{*}_{n}=\{\}$}.

\begin{proof}
We first prove some preliminary claims.

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.4.a} \textit{If $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$ and $i\in{\bf v}_{n}(s)$ for some $s\notin U_{n}$ then $i\notin{\bf v}_{n+1}(s)$}.

\begin{proof}
Fix $i\in{\bf v}_{n}(s)$ for some $s\notin U_{n}$.  Since $({\bf F},{\bf L}_{d,n+1})=\text{\sc shift}(({\bf F},{\bf L}_{d,n}),U_{n})$ and $s\notin U_{n}$, Claim \ref{remain}.1 implies that $\text{\sc layer}_{n+1}(j)=\text{\sc layer}_{n}(j)$ for some $j\in{\bf v}_{n}(s)$.  Therefore, Claim \ref{disjoint}.1 implies:
	\begin{align}
	\label{vnplus1}
		v_{n+1}(s)=\displaystyle\min_{\substack{j\in{\bf v}_{n}(s),\\ \text{\sc layer}_{n+1}(j)=\text{\sc layer}_{n}(j)}}k_{v_{n}(s),j}.
	\end{align}
	We have the following sequence of equalities:
	\begin{align}
		\nonumber
		&\hspace{-3mm}\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
		\label{grandfinale32}
		&\hspace{8mm}=\text{\sc layer}_{n+1}(v_{n+1}(s))-(\text{\sc layer}_{n}(i)+1),\\
		\label{grandfinale37}
		&\hspace{8mm}=\text{\sc layer}_{n}(v_{n+1}(s))-(\text{\sc layer}_{n}(i)+1),\\		
		\nonumber
		&\hspace{8mm}=(\text{\sc layer}_{n}(v_{n}(s))-k_{v_{n}(s),v_{n+1}(s)})\\
		\label{grandfinale33}
		&\hspace{42mm}-(\text{\sc layer}_{n}(i)+1),\\
		\nonumber
		&\hspace{8mm}=\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)\\
		\label{grandfinale34}
		&\hspace{42mm}-k_{v_{n}(s),v_{n+1}(s)}-1,\\
		\label{grandfinale35}
		&\hspace{8mm}=k_{v_{n}(s),i}-k_{v_{n}(s),v_{n+1}(s)}-1,\\
		\label{grandfinale36}
		&\hspace{8mm}=k_{v_{n+1}(s),i}-1,
	\end{align}
	where (\ref{grandfinale32}) follows from the premise of Claim \ref{grandefinale}.4.a that $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$, (\ref{grandfinale37}) follows because (\ref{vnplus1}) implies $\text{\sc layer}_{n+1}(v_{n+1}(s))=\text{\sc layer}_{n}(v_{n+1}(s))$, (\ref{grandfinale33}) follows because (V5) implies $\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(v_{n+1}(s))=k_{v_{n}(s),v_{n+1}(s)}$ if $v_{n+1}(s)\in{\bf v}_{n}(s)$ and (\ref{vnplus1}) implies $v_{n+1}(s)\in{\bf v}_{n}(s)$, (\ref{grandfinale34}) follows by rearranging terms, and (\ref{grandfinale35}) follows from the premise of Claim \ref{grandefinale}.4.a that $i\in{\bf v}_{n}(s)$. 

To justify (\ref{grandfinale36}), it suffices to show that $i\in{\bf f}(v_{n+1}(s),d)$.  If $i\in{\bf f}(s,v_{n}(s))$ then $i\notin{\bf v}_{n}(s)$ which contradicts the premise of Claim \ref{grandefinale}.4.a that $i\in{\bf v}_{n}(s)$.  Moreover, if $i\in{\bf f}(v_{n}(s),v_{n+1}(s))$ then $i\notin{\bf v}_{n+1}(s)$ which proves Claim \ref{grandefinale}.4.a.  Therefore it suffices to assume $i\in{\bf f}(v_{n+1}(s),d)$.  It follows from (\ref{grandfinale36}) that $\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\neq k_{v_{n+1}(s),i}$ which, together with (V5), implies $i\notin{\bf v}_{n+1}(s)$.
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.4.b} \textit{If $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$ and $i\notin{\bf v}_{n}(s)$ for some $s\in U_{n}$ then $i\notin{\bf v}_{n+1}(s)$}.
	\begin{proof}
	There are two cases to consider.

	\hspace{-3.5mm}{\bf Case 1:} $v_{n+1}(s)=v_{n}(s)$.
	
	We have the following sequence of inequalities:
	\begin{align}
		\nonumber
		&\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
		\label{grandfinale38}
		&\hspace{7mm}=\text{\sc layer}_{n+1}(v_{n}(s))-\text{\sc layer}_{n+1}(i),\\
		\label{grandfinale39}
		&\hspace{7mm}=(\text{\sc layer}_{n}(v_{n}(s))+1)-\text{\sc layer}_{n+1}(i),\\
		\label{postgrandfinale39}
		&\hspace{7mm}=(\text{\sc layer}_{n}(v_{n}(s))+1)-(\text{\sc layer}_{n}(i)+1),\\
		\nonumber
		&\hspace{7mm}=\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i),\\
		\label{grandfinale41}
		&\hspace{7mm}\neq k_{v_{n}(s),i},\\
		\label{grandfinale42}
		&\hspace{7mm}=k_{v_{n+1}(s),i},
	\end{align}
	where (\ref{grandfinale38}) follows from the premise of Case 1 that $v_{n+1}(s)=v_{n}(s)$, (\ref{grandfinale39}) follows from (\ref{shift4}) and because $s\in U_{n}$, (\ref{postgrandfinale39}) follows from the premise of Claim \ref{grandefinale}.4.b that $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$, (\ref{grandfinale41}) follows because $i\notin{\bf v}_{n}(s)$ and (V5) implies $\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)=k_{v_{n}(s),i}$ if $i\in{\bf v}_{n}(s)$, and (\ref{grandfinale42}) follows because $v_{n+1}(s)=v_{n}(s)$ by case assumption.  It follows from (\ref{grandfinale42}) and (V5) that $i\notin{\bf v}_{n+1}(s)$.
	
	\hspace{-3.5mm}{\bf Case 2:} $v_{n+1}(s)\neq v_{n}(s)$.
	The premise of Claim \ref{grandefinale}.4.b that $s\in U_{n}$ and the premise of Case 2 that $v_{n+1}(s)\neq v_{n}(s)$, together with Claim \ref{join}.2.c imply:
	\begin{align}
	\nonumber
	&k_{v_{n+1}(s),v_{n}(s)}\\
	\label{kvnplus}
	&\hspace{7mm}=\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(v_{n}(s)).
	\end{align} 
We have the following inequalities:
	\begin{align}
		\nonumber
		&\hspace{-3mm}\text{\sc layer}_{n+1}(v_{n+1}(s))-\text	{\sc layer}_{n+1}(i)\\
		\nonumber
		&=\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(v_{n}(s))\\
		\label{grandfinale43}
		&\hspace{17mm}+\text{\sc layer}_{n+1}(v_{n}(s))-\text{\sc layer}_{n+1}(i),\\
		\nonumber
		&=k_{v_{n+1}(s),v_{n}(s)}+\text{\sc layer}_{n+1}(v_{n}(s))\\
		\label{grandfinale44}
		&\hspace{47mm}-\text{\sc layer}_{n+1}(i),\\
		\nonumber
		&=k_{v_{n+1}(s),v_{n}(s)}+(\text{\sc layer}_{n}(v_{n}(s))+1)\\
		\label{grandfinale45}
		&\hspace{47mm}-\text{\sc layer}_{n+1}(i),\\
		\nonumber
		&=k_{v_{n+1}(s),v_{n}(s)}+(\text{\sc layer}_{n}(v_{n}(s))+1)\\
		\label{postgrandfinale45}
		&\hspace{42mm}-(\text{\sc layer}_{n}(i)+1),\\
		\nonumber
		&=k_{v_{n+1}(s),v_{n}(s)}\\
		\nonumber
		&\hspace{21mm}+(\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)),\\
		\label{grandfinale47}
		&\neq k_{v_{n+1}(s),v_{n}(s)}+k_{v_{n}(s),i},\\
		\label{grandfinale48}
		&=k_{v_{n+1}(s),i},
	\end{align}
	where (\ref{grandfinale43}) follows by subtracting and adding $\text{\sc layer}_{n+1}(v_{n}(s))$ to the left side, (\ref{grandfinale44}) follows from (\ref{kvnplus}), (\ref{grandfinale45}) follows from (\ref{shift4}) and because $s\in U_{n}$, (\ref{postgrandfinale45}) follows from the premise of Claim \ref{grandefinale}.4.b that $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$, and (\ref{grandfinale47}) follows from (V5) and the premise of Claim \ref{grandefinale}.4.b that $i\notin{\bf v}_{n}(s)$.  It follows from (\ref{grandfinale48}) and (V5) that $i\notin{\bf v}_{n+1}(s)$.
	\end{proof}
	
	\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.4.c} \textit{If $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$ and $i\notin{\bf v}_{n}(s)$ for some $s\notin U_{n}$ then $i\notin{\bf v}_{n+1}(s)$}.
	
	\begin{proof}
	Since $s\notin U_{n}$, it follows from Claim \ref{disjoint}.1 and Claim \ref{remain}.1 that $v_{n+1}(s)$ is defined by (\ref{vnplus1}).  Without loss of generality, assume $i\in{\bf f}(v_{n+1}(s),d)$ since the claim is trivial otherwise.  We have the following sequence of equalities:
	\begin{align}
		\nonumber
		&\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
		\label{grandfinale49}
		&=\text{\sc layer}_{n}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i),\\
		\label{grandfinale50}
		&=\text{\sc layer}_{n}(v_{n}(s))-k_{v_{n}(s),v_{n+1}(s)}-\text{\sc layer}_{n+1}(i),\\
		\nonumber
		&=\text{\sc layer}_{n}(v_{n}(s))-k_{v_{n}(s),v_{n+1}(s)}\\
		\label{grandfinale51}
		&\hspace{45mm}-(\text{\sc layer}_{n}(i)+1),\\
		\nonumber
		&=\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)\\
		\nonumber
		&\hspace{45mm}-k_{v_{n}(s),v_{n+1}(s)}-1,\\
		\label{grandfinale53}
		&\leq k_{v_{n}(s),i}-k_{v_{n}(s),v_{n+1}(s)}-1,\\
		\label{grandfinale54}
		&=k_{v_{n+1}(s),i}-1,\\
		\label{grandfinale55}
		&<k_{v_{n+1}(s),i},
	\end{align}
	where (\ref{grandfinale49}) follows because (\ref{vnplus1}) implies $\text{\sc layer}_{n+1}(v_{n+1}(s))=\text{\sc layer}_{n}(v_{n+1}(s))$, (\ref{grandfinale50}) follows from (\ref{kvnplus}), (\ref{grandfinale51}) follows from the premise of Claim \ref{grandefinale}.3.c that $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$, and (\ref{grandfinale53}) follows because (\ref{pregrandfinale3}) implies $\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)\leq k_{v_{n}(s),i}$ if $i\in{\bf f}(v_{n}(s),d)$.  Since (\ref{vnplus1}) implies $v_{n+1}(s)\in{\bf v}_{n}(s)$ and $i\in{\bf f}(v_{n+1}(s),d)$ by assumption, it follows that $i\in{\bf f}(v_{n}(s),d)$.  Furthermore (\ref{grandfinale54}) follows because $v_{n+1}(s)\in{\bf f}(v_{n}(s),i)$.  It follows from (V5) and (\ref{grandfinale55}) that $i\notin{\bf v}_{n+1}(s)$.
	\end{proof}
	
	\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.4.d} \textit{Suppose $s\notin U_{n_{s}}$ for some $n_{s}\in\mathbb{N}$.  If $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$ for all $n\geq n_{s}$ then $i\notin{\bf v}_{n}(s)$ for all $n\geq n_{s}+1$.}
	
	\begin{proof}
	The proof is by induction.  First we prove the initial condition that $i\notin{\bf v}_{n_{s}+1}(s)$ if $\text{\sc layer}_{n_{s}+1}(i)=\text{\sc layer}_{n_{s}}(i)+1$ for some $s\notin U_{n_{s}}$.  There are two cases to consider for the initial condition.

First suppose $i\notin{\bf v}_{n_{s}}(s)$.  Since $s\notin U_{n_{s}}$, and $i\notin{\bf v}_{n_{s}}(s)$, it follows from Claim \ref{grandefinale}.4.c that $i\notin{\bf v}_{n_{s}+1}(s)$.  Next suppose $i\in{\bf v}_{n_{s}}(s)$.  Since $s\notin U_{n_{s}}$ and $i\in{\bf v}_{n_{s}}(s)$, it follows from Claim \ref{grandefinale}.4.a that $i\notin{\bf v}_{n_{s}+1}(s)$.

Now assume the inductive hypothesis that $i\notin{\bf v}_{n}(s)$ for some fixed $n\geq n_{s}+1$.  If $s\in U_{n}$ then Claim \ref{grandefinale}.4.b implies $i\notin{\bf v}_{n+1}(s)$.  If $s\notin U_{n}$ then Claim \ref{grandefinale}.4.c implies $i\notin{\bf v}_{n+1}(s)$.  It follows that $i\notin{\bf v}_{n}(s)$ for all $n\geq n_{s}+1$.
	\end{proof}
	
	
	We can now complete the proof of Claim \ref{grandefinale}.4.  The proof is by contradiction.  Suppose $\liminf\limits_{n}V^{*}_{n}\neq\{\}$.  For some $i\in F_{d}({\cal N})$ and $n_{i}\in\mathbb{N}$, it follows that $i\in V^{*}_{n}$ for all $n\geq n_{i}$.  Therefore (\ref{vstar}) implies $i\in v_{n}(s)$ for some $s\in U_{n}\setminus U^{*}$ and all $n\geq n_{i}$.  It follows from (\ref{shift4}) that: 
	\begin{align}
	\label{layernplus1}
	\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1\hspace{1mm}\text{for all}\hspace{1mm}n\geq n_{i}.	
	\end{align}
Fix $s\in U_{n_{i_{s}}}\setminus U^{*}$ such that $i\in{\bf v}_{n_{i_{s}}}(s)$ for some $n_{i_{s}}\geq n_{i}$.  Since $\liminf_{n} U_{n}\setminus U^{*}=\{\}$ from Claim \ref{grandefinale}.3, it follows that $s\notin U_{n_{s}}\setminus U^{*}$ for some $n_{s}\geq n_{i_{s}}$.  Moreover, $s\notin U^{*}$ by construction, so $s\notin U_{n_{s}}$.  Since $n_{s}\geq n_{i}$, Claim \ref{grandefinale}.4.d and (\ref{layernplus1}) imply that $i\notin{\bf v}_{n}(s)$ for all $n\geq n_{s}+1$.  Similarly, for every $s\in U_{n}\setminus U^{*}$ such that $i\in{\bf v}_{n}(s)$ for some $n\geq n_{i}$, there exists some $n_{s}\geq n_{i}$ such that $i\notin{\bf v}_{n}(s)$ for all $n\geq n_{s}+1$.  For all other $s\notin U^{*}$, we set $n_{s}:=0$.  It follows that $i\notin{\bf v}_{n}(s)$ for any $s\in U_{n}\setminus U^{*}$ and all $n\geq \max_{s}n_{s}+1$.  Therefore $i\notin V^{*}_{n}$ for all $n\geq \max_{s}n_{s}+1$ which is a contradiction.      
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.5} $V_{n}(U^{*})=F_{d}(U^{*})$ $\forall n\geq K_{5}$ and some $K_{5}\in\mathbb{N}$.
\begin{proof}
%There exists some $n_{V}\in\mathbb{N}$ such that $V_{n}(U)=F_{d}(U)$ for all $n\geq n_{V}$
We first prove a preliminary claim.

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.5.a}\textit{ $\lim_{n\rightarrow\infty}{\bf v}_{n}(s)$ exists for every $s\in U^{*}$.} 

\begin{proof}
To prove Claim \ref{grandefinale}.5.a, we show for every $s\in U^{*}$, there exists some $n_{s}\in\mathbb{N}$ such that ${\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$.

Suppose $i\in{\bf v}_{n_{i}}(s)$ for some $n_{i}\in\mathbb{N}$ and $s\in U^{*}$.  It follows from (\ref{U}), that $s\in U_{n}$ for all $n\geq n_{i}$.  Therefore Claim \ref{grandefinale}.2 implies $i\in{\bf v}_{n}(s)$ for all $n\geq n_{i}$.  Hence, $V_{n}(\{s\})\subseteq V_{n+1}(\{s\})\subseteq F_{d}(\{s\})$ for all $n\in\mathbb{N}$.  Since $\{V_{n}(\{s\}):n\in\mathbb{N}\}$ is a monotonically increasing sequence of finite sets, ordered by inclusion with bounded size, there exists some $V(\{s\})\subseteq F_{d}(\{s\})$ and $n_{s}\in\mathbb{N}$ such that: 
\begin{align}
	\label{vdn}
	V_{n}(\{s\})=V(\{s\})\hspace{1mm}\text{for all}\hspace{1mm}n\geq n_{s}.
\end{align}
By construction in (V1)-(V5), both ${\bf v}_{n+1}(s)$ and ${\bf v}_{n}(s)$ are subsequences of ${\bf f}(s,d)$.  Since (\ref{vdn}) implies $V_{n}(\{s\})=V_{n+1}(\{s\})=V(\{s\})$, it follows that ${\bf v}_{n+1}(s)$ and ${\bf v}_{n}(s)$ have the same nodes.  Therefore ${\bf v}_{n+1}(s)={\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$. 
%Next, we show that $v_{n+1}(s)=v_{n}(s)$ for all $n\geq n_{s}$.  Since (\ref{vdn}) implies $V_{n}(\{s\})=V_{n+1}(\{s\})=V(\{s\})$ for all $n\geq n_{s}$, it suffices to verify that $v_{n+1}(s)=v_{n}(s)$ satisfies (V5) for every $i\in {\bf v}_{n+1}(s)$ and $n\geq n_{s}$.  For every such $i\in {\bf v}_{n+1}(s)$ and $n\geq n_{s}$,  we have the following inequalities:
%\begin{align}
%	\nonumber
%	&\text{\sc layer}_{n+1}(v_{n+1}(s))-\text{\sc layer}_{n+1}(i)\\
%	\label{grandfinale56}
%	&\hspace{5mm}=\text{\sc layer}_{n+1}(v_{n}(s))-\text{\sc layer}_{n+1}(i),\\
%	\label{grandfinale57}
%	&\hspace{5mm}=(\text{\sc layer}_{n}(v_{n}(s))+1)-(\text{\sc layer}_{n}(i)+1),\\
%	\label{grandfinale58}
%	&\hspace{5mm}=\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i),\\
%	\label{grandfinale59}
%	&\hspace{5mm}=k_{v_{n}(s),i},\\
%	\label{grandfinale60}
%	&\hspace{5mm}=k_{v_{n+1}(s),i},
%\end{align}
%where (\ref{grandfinale56}) follows from the hypothesis that $v_{n+1}(s)=v_{n}(s)$, (\ref{grandfinale57}) follows from (\ref{shift4}) and because $i\in{\bf v}_{n}(s)$ for some $s\in U^{*}\subseteq U_{n}$, and (\ref{grandfinale59}) follows from (V5) and because (\ref{vdn}) implies $i\in{\bf v}_{n}(s)$ if $n\geq n_{s}$.  Since (\ref{grandfinale60}) is true for every $i\in{\bf v}_{n+1}(s)$, it follows from (V5) that $v_{n+1}(s)=v_{n}(s)$.  Moreover, (\ref{grandfinale59}) and (\ref{grandfinale60}) show that ${\bf v}_{n+1}(s)$ and ${\bf v}_{n}(s)$ have the same encoding delays.  Since ${\bf v}_{n+1}(s)$ and ${\bf v}_{n}(s)$ have the same virtual sources, the same nodes, and the same encoding delays, it follows that ${\bf v}_{n+1}(s)={\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$.  To finish the proof, set $n_{V}:=\max_{s\in U}n_{s}$ with $n_{s}$ defined in (\ref{vdn}).
\end{proof}

%\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.5.b} \textit{$\lim_{n\rightarrow\infty}V_{n}(U^{*})$ exists.}

%\textit{There exists some $V(U)\subseteq F_{d}(U)$ such that $V_{n}(U)=V(U)$ for all $n\geq n_{V}$ and some $n_{V}\in\mathbb{N}$.}

%\begin{proof}
%By definition, $V_{n}(U^{*}):=\{i\in{\bf v}_{n}(s):s\in U^{*}\}$.  The proof follows from Claim \ref{grandefinale}.5.a.
%To prove Claim \ref{grandefinale}.5.b, we show that $V_{n}(U^{*})=V(U^{*})$ for some  $V(U^{*})\subseteq F_{d}(U^{*})$ and all $n\geq n_{V}$, where $n_{V}\in\mathbb{N}$.
%If $i\in V_{n_{i}}(U^{*})$ for some $n_{i}\in\mathbb{N}$, then $i\in{\bf v}_{n_{i}}(s)$ for some $s\in U^{*}$.  It follows from (\ref{U}), that $s\in U_{n}$ for all $n\geq n_{i}$.  Therefore Claim \ref{grandefinale}.2 implies $i\in{\bf v}_{n}(s)$ for all $n\geq n_{i}$.  It follows that $V_{n}(U^{*})\subseteq V_{n+1}(U^{*})\subseteq F_{d}(U^{*})$ for all $n\in\mathbb{N}$, so $\{V_{n}(U^{*}):n\in\mathbb{N}\}$ is a monotonically increasing sequence of universally bounded finite sets, with inclusion acting as partial ordering. Hence, there exists some $n_{V}\in\mathbb{N}$ and $V(U^{*})\subseteq F_{d}(U^{*})$ such that:
 %\begin{align}
 %		V_{n}(U^{*})=V(U^{*})\hspace{1mm}\text{for all}\hspace{1mm}n\geq n_{V},
 %	\end{align} 
 %	which completes the proof of Claim \ref{grandefinale}.5.a.
%\end{proof}

We can now complete the proof of Claim \ref{grandefinale}.5.  The proof is by contradiction.  For every $s\in U^{*}$, Claim \ref{grandefinale}.5.a implies ${\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$ and some $n_{s}\in\mathbb{N}$.  Define $V(U^{*}):=\{i\in{\bf v}(s):s\in U^{*}\}$.  It follows that $V_{n}(U^{*})=V(U^{*})$ for all $n\geq\max_{s\in U^{*}}n_{s}$.  Therefore $\lim_{n\rightarrow\infty}V_{n}(U^{*})=V(U^{*})$.  Suppose $V(U^{*})\neq F_{d}(U)$, and pick some $i\in F_{d}(U^{*})\setminus V(U^{*})$.  Now $i\in{\bf f}(s,d)$ for some $s\in U^{*}$.  There are two cases to consider.

\hspace{-3.5mm}{\bf Case 1:} $i\in{\bf f}(v(s),d)$.

For all $n\in\mathbb{N}$:
\begin{align}
	\label{grandfinale61}
	\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)\leq k_{v_{n}(s),i},
\end{align}
where (\ref{grandfinale61}) follows from (\ref{pregrandfinale3}).  Claim \ref{grandefinale}.5.a implies ${\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$.  For all $n\geq n_{s}$, Claim \ref{grandefinale}.5.a and (\ref{grandfinale61}) imply:
\begin{align}
	\label{grandfinale62}
	\text{\sc layer}_{n}(v(s))-\text{\sc layer}_{n}(i)\leq k_{v(s),i}.
\end{align} 
For all $n\in\mathbb{N}$:
\begin{align}
	\label{grandfinale63}
	\text{\sc layer}_{n}(i)\leq\text{\sc layer}_{n+1}(i)\leq\text{\sc layer}_{n}(i)+1,
\end{align}
where (\ref{grandfinale63}) follows from (\ref{shift4}).  The definition of $U^{*}$ in (\ref{U}) implies that $U^{*}\subseteq U_{n}$ for all $n\geq K_{1}$ and some $K_{1}\in\mathbb{N}$.  For all $n\geq\max\{n_{s},K_{1}\}$:
\begin{align}
	\label{grandfinale64}
	\text{\sc layer}_{n+1}(v(s))=\text{\sc layer}_{n}(v(s))+1.
\end{align}
To justify (\ref{grandfinale64}), observe that Claim \ref{grandefinale}.5.a implies  $v_{n}(s)=v(s)$ for all $n\geq n_{s}$.  Therefore (\ref{grandfinale64}) follows from (\ref{shift4}) and because $U^{*}\subseteq U_{n}$ for all $n\geq K_{1}$.  

Define the sequence $a_{n}:=\text{\sc layer}_{n}(v(s))-\text{\sc layer}_{n}(i)$.  Both   (\ref{grandfinale63}) and (\ref{grandfinale64}) imply $a_{n}$ is monotonically non-decreasing for all $n\geq\max\{n_{s}, K_{1}\}$.  We will show $a_{n}$ is actually unbounded from above, which contradicts (\ref{grandfinale62}).  

Since $\liminf_{n}V^{*}_{n}=\{\}$ from Claim \ref{grandefinale}.4, there exists an infinite sequence $\{n_{q}:q\in\mathbb{N}\}$ where $n_{0}:=\max\{n_{s},K_{1}\}$ such that $i\notin V^{*}_{n_{q}}$.  It follows from (\ref{vstar}) that $i\notin{\bf v}_{n_{q}}(s^{\prime})$ for all $s^{\prime}\in U_{n_{q}}\setminus U^{*}$ and $q\in\mathbb{N}$.  Moreover, since $i\in F_{d}(U)\setminus V(U)$, it follows that $i\notin{\bf v}(s^{\prime})$ for all $s^{\prime}\in U^{*}$.  Hence, $i\notin{\bf v}(s^{\prime})$ for any $s^{\prime}\in U_{n_{q}}$.  It follows from (\ref{shift4}) that:
\begin{align}
	\label{grandfinale65}
	\text{\sc layer}_{n_{q}+1}(i)=\text{\sc layer}_{n_{q}}(i)\hspace{1mm}\text{for all}\hspace{1mm}q\in\mathbb{N}.
\end{align}
For every $q\in\mathbb{N}$:
\begin{align}
\label{grandfinale66}
a_{n_{q}+1}&:=\text{\sc layer}_{n_{q}+1}(v_{n_{q}+1}(s))-\text{\sc layer}_{n_{q}+1}(i),\\
\label{grandfinale67}
&=(\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))+1)-\text{\sc layer}_{n_{q}+1}(i),\\
\label{postgrandfinale67}
&=(\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))+1)-\text{\sc layer}_{n_{q}}(i),\\
\nonumber
&=\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))-\text{\sc layer}_{n_{q}}(i)+1,\\
\label{grandfinale68}
&=a_{n_{q}}+1,
\end{align}
where (\ref{grandfinale66}) follows from the definition of $a_{n}$, (\ref{grandfinale67}) follows from (\ref{grandfinale64}) and because $n_{0}:=\max\{n_{s},K_{1}\}$, (\ref{postgrandfinale67}) follows from (\ref{grandfinale65}), and (\ref{grandfinale68}) follows from the definition of $a_{n}$.  It follows from (\ref{grandfinale68}), that $a_{n}$ is unbounded from above.  Therefore $a_{n}$ is monotonically non-decreasing and unbounded from above which contradicts (\ref{grandfinale62}).  It follows that $i\in V(U^{*})$ if $i\in{\bf f}(v(s),d)$.

\hspace{-3.5mm}{\bf Case 2:} $i\in{\bf f}(s,v(s))$.

For all $n\in\mathbb{N}$:
\begin{align}
	\label{grandfinale69}
	\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(v_{n}(s))>k_{i,v_{n}(s)},
\end{align}
where (\ref{grandfinale69}) follows from (\ref{pregrandfinale4}).  Claim \ref{grandefinale}.5.a implies ${\bf v}_{n}(s)={\bf v}(s)$ for all $n\geq n_{s}$ and some $n_{s}\in\mathbb{N}$.  Therefore: 
\begin{align}
	\label{grandfinale70}
	\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(v(s))>k_{i,v(s)}.
\end{align}
where (\ref{grandfinale70}) follows from (\ref{grandfinale69}) and Claim \ref{grandefinale}.5.a. 

Define the sequence $b_{n}:=\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(v(s))$.  Both (\ref{grandfinale63}) and (\ref{grandfinale64}) imply $b_{n}$ is monotonically non-increasing for all $n\geq\max\{n_{s}, K_{1}\}$.  We will show that $b_{n}$ is actually unbounded from below which contradicts (\ref{grandfinale70}).  

As before, we construct an infinite sequence $\{n_{q}:q\in\mathbb{N}\}$ where $n_{0}:=\max\{n_{s},K_{1}\}$ such that $i\notin V^{*}_{n_{q}}$.  For every $q\in\mathbb{N}$: 
\begin{align}
	\label{grandfinale71}
	b_{n_{q}+1}&:=\text{\sc layer}_{n_{q}+1}(i)-\text{\sc layer}_{n_{q}+1}(v_{n_{q}+1}(s)),\\
	\label{grandfinale72}
	&=\text{\sc layer}_{n_{q}+1}(i)-(\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))+1),\\
	\label{postgrandfinale72}
	&=\text{\sc layer}_{n_{q}}(i)-(\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))+1),\\
	\nonumber
	&=\text{\sc layer}_{n_{q}}(i)-\text{\sc layer}_{n_{q}}(v_{n_{q}}(s))-1,\\
	\label{grandfinale74}
	&=b_{n_{q}}-1,
\end{align}
where (\ref{grandfinale71}) follows from the definition of $b_{n}$, (\ref{grandfinale72}) follows from (\ref{grandfinale64}) and the fact that $n_{0}:=\max\{n_{s},n_{U}\}$,  (\ref{postgrandfinale72}) follows from (\ref{grandfinale65}), and (\ref{grandfinale74}) follows from the definition of $b_{n}$.  It follows from (\ref{grandfinale74}), that $b_{n}$ is unbounded from below.  Therefore $b_{n}$ is monotonically non-increasing and unbounded from below, which contradicts (\ref{grandfinale70}).  It follows that $i\in V(U^{*})$ if $i\in{\bf f}(s,v(s))$. 

Case 1 and Case 2 imply $V(U^{*})=F_{d}(U^{*})$ which completes the proof of Claim \ref{grandefinale}.5. 
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.6} \textit{For some function $l(n)$, $K_{6}\in\mathbb{N}$, and all $n\geq K_{6}$:}
\begin{align}
	\label{FDU}
	F_{d}(U^{*})&\subseteq\displaystyle\cup^{|{\bf L}_{d,n}|-1}_{q=l(n)}L_{q,n},\\
	\label{FDU2}
	F_{d}({\cal N})\setminus F_{d}(U^{*})&\subseteq\cup^{l(n)}_{q=0}L_{q,n},\\
	\label{FDU3}
	V_{n}(U_{n}\setminus U^{*})&\subseteq\cup^{l(n)}_{q=0}L_{q,n}.
	%\label{FDN}
	%F_{d}({\cal N})\setminus F_{d}(U^{*})&=\lim_{n\rightarrow\infty}\displaystyle\cup^{l(n)}_{q=0}L_{q,n}.
\end{align}
\begin{proof}
%\textit{For some $n_{F}\in\mathbb{N}$ and every $n\geq n_{F}$, there exists some $l(n)$ such that:}
We introduce some preliminary notation.  For all $i,j\in F_{d}({\cal N})$ define:
\begin{align}
	\label{enij}
	e_{n}(i,j):=\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(j).
\end{align}
To prove (\ref{FDU}) and (\ref{FDU2}), it suffices to establish the following limits.  If $i,j\in F_{d}(U^{*})$ then:
\begin{align}
	\label{limenij1}
	\lim_{n\rightarrow\infty}e_{n}(i,j)&=e(i,j),
\end{align}
where $e(i,j)$ is a constant with respect to $n$.  If $i\in F_{d}(U^{*})$ and $j\in F_{d}({\cal N})\setminus F_{d}(U^{*})$ then:
\begin{align}
	\label{limenij2}
	\lim_{n\rightarrow\infty}e_{n}(i,j)&=\infty.
\end{align}
Both (\ref{limenij1}) and (\ref{limenij2}) also imply (\ref{FDU3}).  To justify (\ref{FDU3}), suppose by contradiction that $i\in F_{d}(U^{*})\cap V_{n}(U_{n}\setminus U^{*})$ and $j\in V_{n}(U_{n}\setminus U^{*})\setminus F_{d}(U^{*})$ for some $s\in U_{n}\setminus U^{*}$ and $i,j\in v_{n}(s)$.  Then,
\begin{align}
	\nonumber
	&\hspace{-6mm}\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(j)\\
	\nonumber
	&\hspace{7mm}=(\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(j)),\\
	\label{FDU4}
	&\hspace{13mm}-(\text{\sc layer}_{n}(v_{n}(s))-\text{\sc layer}_{n}(i)),\\
	\label{FDU5}
	&\hspace{7mm}=k_{v_{n}(s),j}-k_{v_{n}(s),i},\\
	\nonumber
	&\hspace{7mm}\leq k_{v_{n}(s),j},\\
	\label{FDU6}
	&\hspace{7mm}\leq k_{s,j},
\end{align}
where (\ref{FDU4}) follows by adding and subtracting $\text{\sc layer}_{n}(v_{n}(s))$, (\ref{FDU5}) follows from (V5) and the assumption that $i,j\in v_{n}(s)$, and (\ref{FDU6}) follows from the definition of $k_{v_{n}(s),j}$ in  (V5).  The bound in (\ref{FDU6}) contradicts (\ref{limenij2}).  Therefore  (\ref{limenij1}) and (\ref{limenij2}) implies (\ref{FDU})-(\ref{FDU3}).  It remains to prove (\ref{limenij1}) and (\ref{limenij2}). 

%For every $n\in\mathbb{N}$, we have the following sequence of equalities:
%\begin{align}
%	\nonumber
%	&F_{d}({\cal N})\\
%	\label{grandfinale77}
%	&\hspace{3mm}=V_{n}({\cal N}),\\
%	\nonumber
%	&\hspace{3mm}=[F_{d}({\cal N})\setminus V_{n}(U_{n})]\cup V_{n}(U_{n}),\\
%	\nonumber
%	&\hspace{3mm}=[F_{d}({\cal N})\setminus V_{n}(U_{n})]\cup[V_{n}(U)\cup V_{n}(U_{n}\setminus U)],\\
%	\label{grandfinale80}
%	&\hspace{3mm}=[(F_{d}({\cal N})\setminus V_{n}(U_{n}))\cup V_{n}(U_{n}\setminus U)]\cup V_{n}(U),
%\end{align}
%where (\ref{grandfinale77}) follows because $({\bf F},{\bf L}_{d,0})$ is complete (by construction in Lemma \ref{completeexists}), so Lemma \ref{complete} implies that $({\bf F},{\bf L}_{d,n})$ is complete for all $n\in\mathbb{N}$.  It follows from (\ref{grandfinale80}) that $i\in F_{d}({\cal N})$ implies $i\in (F_{d}({\cal N})\setminus V_{n}(U))\cup V_{n}(U_{n}\setminus U)\cup V_{n}(U)$.  
The definition of $U^{*}$ in (\ref{U}) implies that $U^{*}\subseteq U_{n}$ for all $n\geq K_{1}$ and some $K_{1}\in\mathbb{N}$.  For all $i\in V_{n}(U^{*})$ and $n\geq K_{1}$, it follows that:
\begin{align}
	\label{grandfinale81}
	\text{\sc layer}_{n+1}(i)&=\text{\sc layer}_{n}(i)+1,
\end{align}
where (\ref{grandfinale81}) follows from (\ref{shift4}) and the fact that $U^{*}\subseteq U_{n}$ for all $n\geq K_{1}$.

First, we justify (\ref{limenij1}).  Claim \ref{grandefinale}.5, implies that $V_{n}(U^{*})=F_{d}(U^{*})$ for all $n\geq K_{5}$ and some $K_{5}\in\mathbb{N}$.  Fix $i,j\in F_{d}(U^{*})$. For all $n\geq K_{5}$:
\begin{align}
	\label{grandfinale84}
	e_{n+1}(i,j)&=\text{\sc layer}_{n+1}(i)-\text{\sc layer}_{n+1}(j),\\
	\label{grandfinale85}
	&=(\text{\sc layer}_{n}(i)+1)+(\text{\sc layer}_{n}(j)+1),\\
	\nonumber
	&=\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(j),\\
	\label{grandfinale87}
	&=e_{n}(i,j)
	%\label{grandfinale88}
	%&=e_{n_{V}}(i,j),
\end{align}
where (\ref{grandfinale84}) follows from (\ref{enij}), (\ref{grandfinale85}) follows from (\ref{grandfinale81}) and because $F_{d}(U^{*})=V_{n}(U^{*})$ for $n\geq K_{5}$, and (\ref{grandfinale87}) follows from (\ref{enij}). Set $e(i,j):=e_{n}(i,j)$ for $n=K_{5}$.  Now (\ref{grandfinale87}) implies that $e_{n}(i,j)=e(i,j)$ for all $n\geq K_{5}$, which proves (\ref{limenij1}).

Now we justify (\ref{limenij2}).  Fix $i\in F_{d}(U^{*})$ and $j\notin F_{d}(U^{*})$.  Invoking Claim \ref{grandefinale}.4, we construct an infinite sequence $\{n_{q}:q\in\mathbb{N}\}$ where $n_{0}=K_{5}$ such that $j\notin V^{*}_{n_{q}}$.  First we show that $j$ satisfies:
\begin{align}
	\label{grandfinale83}
	\text{\sc layer}_{n_{q}+1}(j)=\text{\sc layer}_{n_{q}}(j)\hspace{2mm}\text{for all}\hspace{1mm}q\in\mathbb{N}.
\end{align}
Since $V_{n_{q}}(U^{*})\subseteq F_{d}(U^{*})$ for all $q\in\mathbb{N}$, it follows that $j\notin V_{n_{q}}(U^{*})$.  If $j\notin V_{n_{q}}(U^{*})$ and $j\notin V^{*}_{n_{q}}$, it follows that $j\notin {\bf v}_{n_{q}}(s)$ for any $s\in U^{*}$ and, as implied by (\ref{vstar}), any $s\in U_{n_{q}}\setminus U^{*}$.  Therefore $j\notin{\bf v}_{n_{q}}(s)$ for any $s\in U_{n_{q}}$, so (\ref{grandfinale83}) follows from (\ref{shift4}). 
%If $i\in F_{d}({\cal N})\setminus V_{n}(U_{n})$:
%\begin{align}
%	\label{grandfinale82}
%	\hspace{-1mm}\text{\sc layer}_{n+1}(i)&=\text{\sc layer}_{n}(i)\hspace{2mm}\text{for all}\hspace{1mm}n\in\mathbb{N}
%\end{align}
%where (\ref{grandfinale82}) follows from (\ref{aln}), (\ref{shift4}), 
%and the fact that $i\notin{\bf v}_{n}(s)$ for any $s\in U_{n}$, implies $i\notin A_{l,n}(U_{n})$ for any $l\in\{0,\ldots,|{\bf L}_{d,n}|-1\}$.  
%For any $i\in F_{d}({\cal N})$, Claim \ref{grandefinale}.4 implies there is a corresponding infinite sequence $\{n_{q}:q\in\mathbb{N}\}$ where $n_{0}:=n_{V}\geq n_{U}$, such that $i\notin V^{*}_{n_{q}}$.  Therefore, if $i\notin F_{d}(U)$:
%\begin{align}
%	\label{grandfinale83}
%	\text{\sc layer}_{n_{q}+1}(i)=\text{\sc layer}_{n_{q}}(i)\hspace{2mm}\text{for all}\hspace{1mm}q\in\mathbb{N},
%\end{align}
%where (\ref{grandfinale83}) follows because $i\notin F_{d}(U)$ implies $i\notin V_{n_{q}}(U)$, since $V_{n_{q}}(U)\subseteq F_{d}(U)$.  Moreover $i\notin V^{*}_{n_{q}}:=V_{n_{q}}(U_{n_{q}}\setminus U)$ so $i\notin V_{n_{q}}(U_{n_{q}})$.  If $i\notin {\bf v}_{n_{q}}(s)$ for any $s\in U_{n_{q}}$, then (\ref{aln}) implies $i\notin A_{l,n_{q}}(U_{n_{q}})$ for any $l\in\{0,\ldots,|{\bf L}_{d,n_{q}}|-1\}$ so (\ref{grandfinale83}) follows from (\ref{shift4}).  
%If $i\in F_{d}(U)$ and $j\in F_{d}({\cal N})\setminus V_{n}(U_{n})$ and $n\geq n_{V}$:
%\begin{align}
%	\label{grandfinale89}
%	e_{n+1}(i,j)&=\text{\sc layer}_{n+1}(i)-\text{\sc layer}_{n+1}(j),\\
%	\label{grandfinale90}
%	&=(\text{\sc layer}_{n}(i)+1)-\text{\sc layer}_{n+1}(j),\\
%	\label{pregrandfinale91}
%	&=(\text{\sc layer}_{n}(i)+1)-\text{\sc layer}_{n}(j),\\
%	\nonumber
%	&=\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(j)+1,\\
%	\label{grandfinale92}
%	&=e_{n}(i,j)+1,
%\end{align}
%where (\ref{grandfinale89}) follows from (\ref{enij}), (\ref{grandfinale90}) follows by substituting (\ref{grandfinale81}) into $\text{\sc layer}_{n+1}(i)$ and the fact that Claim \ref{grandefinale}.5 implies $F_{d}(U)=V_{n}(U)$ for $n\geq n_{V}$, (\ref{pregrandfinale91}) follows by substituting (\ref{grandfinale82}) into $\text{\sc layer}_{n+1}(j)$, and (\ref{grandfinale92}) follows from (\ref{enij}).  It follows from (\ref{grandfinale92}) that $\lim_{n\rightarrow\infty}e_{n}(i,j)=\infty$, so the limit (\ref{limenij2}) is satisfied.  
For all $n\geq K_{5}$:
\begin{align}
	\label{grandfinale93}
	e_{n_{q}+1}(i,j)&=\text{\sc layer}_{n_{q}+1}(i)-\text{\sc layer}_{n_{q}+1}(j),\\
	\label{grandfinale94}
	&=(\text{\sc layer}_{n_{q}}(i)+1)-\text{\sc layer}_{n_{q}+1}(j),\\
	\label{pregrandfinale95}
	&=(\text{\sc layer}_{n_{q}}(i)+1)-\text{\sc layer}_{n_{q}}(j),\\
	\nonumber
	&=\text{\sc layer}_{n_{q}}(i)-\text{\sc layer}_{n_{q}}(j)+1,\\
	\label{grandfinale96}
	&=e_{n_{q}}(i,j)+1,
\end{align}
where (\ref{grandfinale93}) follows from (\ref{enij}), (\ref{grandfinale94}) follows from (\ref{grandfinale81}) and because $F_{d}(U^{*})=V_{n}(U^{*})$ for $n\geq K_{5}$, (\ref{pregrandfinale95}) follows from (\ref{grandfinale83}), and (\ref{grandfinale96}) follows from (\ref{enij}).  More generally, for all $n\geq K_{5}$:
\begin{align}
	\label{grandfinale97}
	e_{n+1}(i,j)&=\text{\sc layer}_{n+1}(i)-\text{\sc layer}_{n+1}(j),\\
	\label{grandfinale98}
	&=(\text{\sc layer}_{n}(i)+1)-\text{\sc layer}_{n+1}(j),\\
	\label{grandfinale99}
	&\geq(\text{\sc layer}_{n}(i)+1)-(\text{\sc layer}_{n}(j)+1),\\
	\nonumber
	&=\text{\sc layer}_{n}(i)-\text{\sc layer}_{n}(j),\\
	\label{grandfinale100}
	&=e_{n}(i,j),
\end{align}
where (\ref{grandfinale97}) follows from (\ref{enij}), (\ref{grandfinale98}) follows because (\ref{grandfinale81}) applies for $n\geq K_{1}$ and because $F_{d}(U^{*})=V_{n}(U^{*})$ for $n\geq K_{5}$, (\ref{grandfinale99}) follows because (\ref{shift4}) implies $\text{\sc layer}_{n}(j)\leq\text{\sc layer}_{n+1}(j)\leq\text{\sc layer}_{n}(j)+1$, and (\ref{grandfinale100}) follows from (\ref{enij}).  Combining (\ref{grandfinale96}) and (\ref{grandfinale100}) implies $\lim_{n\rightarrow\infty}e_{n}(i,j)=\infty$ if $i\in F_{d}(U^{*})$ and $j\in F_{d}({\cal N})\setminus F_{d}(U^{*})$, which proves (\ref{limenij2}).
\end{proof}

%\hspace{-3.5mm}{\bf Claim \ref{grandefinale}.7} \textit{For the $l(n)$ defined in (\ref{FDU}):}
%\begin{align}
%	\label{vnun}
%	V_{n}(U_{n}\setminus U^{*})&=\lim_{n\rightarrow\infty}\cup^{l(n)}_{q=0}L_{q,n}.
%\end{align}
%\textit{where $l(n)$ is the function in (\ref{FDU}) and (\ref{FDN})}.
%\begin{proof}
%Fix some $i\in V_{n}(U_{n}\setminus U^{*})$.  If $i\notin F_{d}(U^{*})$ then Claim \ref{grandefinale}.6 implies $i\in\cup^{l(n)}_{q=0}L_{q,n}$ for all $n\geq n_{6}$ and some $n_{6}\in\mathbb{N}$.  Hence, we can assume $i\in F_{d}(U^{*})$.  Claim \ref{grandefinale}.5 implies that $V_{n}(U^{*})=F_{d}(U^{*})$ for all $n\geq n_{5}$ and some $n_{5}\in\mathbb{N}$.  Moreover, Claim \ref{grandefinale}.1 and the definition of $U^{*}$ imply $U^{*}\subseteq U_{n}$ for all $n\geq n_{1}$ and some $n_{1}\in\mathbb{N}$.  Therefore (\ref{shift4}) implies that $\text{\sc layer}_{n+1}(i)=\text{\sc layer}_{n}(i)+1$ for all $n\geq\max\{n_{1},n_{5}\}$.  For every $s\notin U^{*}$, Claim \ref{grandefinale}.3 implies that $s\notin U_{n_{s}}$ for some $n_{s}\geq\max\{n_{1},n_{5}\}$.  Moreover, Claim \ref{grandefinale}.4.d implies that $i\notin{\bf v}_{n}(s)$ for all $n\geq n_{s}+1$.  It follows that $i\notin{\bf v}_{n}(s)$ for any $s\notin U^{*}$ and $n\geq\max_{s\notin U^{*}}n_{s}+1$.  Hence, $i\notin V_{n}(U_{n}\setminus U^{*})$ for all $n\geq\max_{s\notin U^{*}}n_{s}+1$.  It follows that $V_{n}(U_{n}\setminus U^{*})\cap F_{d}(U^{*})=\{\}$ for all $n\geq\max_{s\notin U^{*}}n_{s}+1$.  Therefore (\ref{vnun}) follows from Claim \ref{grandefinale}.6.   
%Repeating this argument for every $s\notin U$ and setting $n_{L}:=\max_{s\notin U}n_{s}+1$ proves that $i\notin V_{n}(U_{n}\setminus U)$ for all $n\geq n_{L}$.
%\hspace{-3.5mm}{\bf Case 2:} $i\notin F_{d}(U)$
%Since $i\in F_{d}({\cal N})\setminus F_{d}(U)$, it follows from (\ref{FDN}) that $i\in\cup^{l(n)}_{q=0}L_{q,n}$.
%\end{proof}

We can now complete the proof of Lemma \ref{grandefinale}.  The proof is by contradiction.  If the Lemma is false, then Claim \ref{grandefinale}.1 implies there exists some non-empty $U^{*}$ defined by (\ref{U}) for all $n\geq K_{1}$ and some $K_{1}\in\mathbb{N}$.  For some function $l(n)$, all $q\in\{l(n)+1,\ldots,|{\bf L}_{d,n}|-1\}$, all $n\geq K_{6}$ and some $K_{6}\in\mathbb{N}$, Claim \ref{grandefinale}.5 and \ref{grandefinale}.6 imply:   
%Claim \ref{grandefinale}.5 implies $V_{n}(U^{*})=F_{d}(U^{*})$ for all $n\geq n_{5}$ and some $n_{5}\in\mathbb{N}$.  Claim \ref{grandefinale}.6 implies that $F_{d}(U^{*})=\cup^{|{\bf L}_{d,n}|-1}_{q=l(n)+1}L_{q,n}$ for all $n\geq n_{6}$ and some $n_{6}\in\mathbb{N}$.  For all $n\geq\max\{n_{5},n_{6}\}$ it follows that:
%\begin{align}
%	\label{FDU2}
%	F_{d}(U^{*})&=\cup^{|{\bf L}_{d,n}|-1}_{q=l(n)+1}A_{q,n}(U^{*}).
%\end{align}
%For all $n\geq n_{6}$, Claim \ref{grandefinale}.6 implies that:
%\begin{align}
%	\label{FDN2}
%	F_{d}({\cal N})\setminus F_{d}(U^{*})&=\cup^{l(n)}_{q=0}L_{q,n}.
%\end{align}
\begin{align}
	\label{aln2}
	A_{q,n}(U^{*})&=L_{q,n}.
\end{align}
To justify (\ref{aln2}), suppose by contradiction, there is some $i\in L_{q,n}$ and $q\in\{l(n)+1,\ldots,|{\bf L}_{d,n}|-1\}$ such that $i\notin A_{q,n}(U^{*})$ for some $n\geq K_{6}$.  It follows from (\ref{FDU}) and (\ref{FDU2}) that $i\in F_{d}(U^{*})$.  But $i\notin A_{q,n}(U^{*})$ implies $i\notin v_{n}(s)$ for all $s\in U^{*}$ which contradicts Claim \ref{grandefinale}.5.  

For all $q\in\{l(n)+1,\ldots,|{\bf L}_{d,n}|-1\}$ and $n\geq K_{6}$: 
\begin{align}
	\nonumber
	&\tilde{A}_{q,n}(U^{*})\\
	\label{newgrandefinale2}
	&=F_{I(d)}\cup(\cup^{q}_{k=0}L_{k,n})\setminus A_{q,n}(U^{*}),\\
	\nonumber
	&=F_{I(d)}\cup(\cup^{l(n)}_{k=0}L_{k,n})\\
	\label{newgrandefinale3}
	&\hspace{29mm}\cup(\cup^{q}_{k=l(n)+1}L_{k,n})\setminus A_{q,n}(U^{*}),\\
	\nonumber
	&=F_{I(d)}\cup(F_{d}({\cal N})\setminus F_{d}(U^{*}))\\
	\label{newgrandefinale4}
	&\hspace{29mm}\cup(\cup^{q}_{k=l(n)+1}L_{k,n})\setminus A_{q,n}(U^{*}),\\
	\label{newgrandefinale5}
	&=\tilde{F}_{d}(U^{*})\cup(\cup^{q}_{k=l(n)+1}L_{k,n})\setminus A_{q,n}(U^{*}),\\
	\label{newgrandefinale6}
	&=\tilde{F}_{d}(U^{*})\cup(\cup^{q-1}_{k=l(n)+1}A_{k,n}(U^{*})),
\end{align}
where (\ref{newgrandefinale2}) follows from (\ref{alntilde}), (\ref{newgrandefinale3}) follows because $q\in\{l(n)+1,\ldots,|{\bf L}_{d,n}|-1\}$ by assumption, (\ref{newgrandefinale4}) follows from (\ref{FDU2}), (\ref{newgrandefinale5}) follows from the definition of $\tilde{F}_{d}(U^{*})$, and (\ref{newgrandefinale6}) follows from (\ref{aln2}).  

For every $s\notin U^{*}$, Claim \ref{grandefinale}.3 implies $s\notin U_{n_{s}}\setminus U^{*}$ for some $n_{s}\in\mathbb{N}$.  Therefore $s\notin U_{n_{s}}$.  Lemma \ref{induction} implies $s\in Z_{n_{s}+1}$.  Define $K_{7}:=\max_{s\notin U^{*}}n_{s}+1$.  Since Lemma \ref{induction} also implies $Z_{n}\subseteq Z_{n+1}$ for all $n\in\mathbb{N}$, it follows that $({\cal S}(d)\setminus U^{*})\subseteq Z_{n}$ for all $n\geq K_{7}$.  For all $n\geq\max\{K_{6},K_{7}\}$:
\begin{align}
	\nonumber
	&R_{U_{n}\setminus U^{*}}\\
	\label{newgrandfinale12}
	&\hspace{4mm}<\sum^{|{\bf L}_{d,n}|-1}_{q=0}I(X_{A_{q,n}(U_{n}\setminus U^{*})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n}\setminus U^{*})}),\\
	\label{newgrandfinale13}
	&\hspace{4mm}=\sum^{l(n)}_{q=0}I(X_{A_{q,n}(U_{n}\setminus U^{*})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n}\setminus U^{*})}),
\end{align}
where (\ref{newgrandfinale12}) follows because $(U_{n}\setminus U^{*})\subseteq({\cal S}(d)\setminus U^{*})\subseteq Z_{n}$ and all subsets of $Z_{n}$ satisfy (\ref{flowdecomp3}) by definition, and (\ref{newgrandfinale13}) follows from (\ref{FDU3}).  For all $n\geq\max\{K_{6},K_{7}\}$:
\begin{align}
	\label{newgrandfinale7}
	R_{U_{n}}&>\sum^{|{\bf L}_{d,n}|-1}_{q=0}I(X_{A_{q,n}(U_{n})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n})}),\\
	\nonumber
	&=\sum^{l(n)}_{q=0}I(X_{A_{q,n}(U_{n})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n})})\\
	\nonumber
	&\hspace{4mm}+\sum^{|{\bf L}_{d,n}|-1}_{q=l(n)+1}I(X_{A_{q,n}(U_{n})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n})}),\\
	\nonumber
	&=\sum^{l(n)}_{q=0}I(X_{A_{q,n}(U_{n})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n})})\\
	\label{newgrandfinale9}
	&\hspace{5mm}+\sum^{|{\bf L}_{d,n}|-1}_{q=l(n)+1}I(X_{A_{q,n}(U^{*})};Y_{d}|X_{\tilde{A}_{q,n}(U^{*})}),\\
	\nonumber
	&=\sum^{l(n)}_{q=0}I(X_{A_{q,n}(U_{n})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n})})\\
	\label{newgrandfinale10}
	&\hspace{23mm}+I(X_{F_{d}(U^{*})};Y_{d}|X_{\tilde{F}_{d}(U^{*})}),\\
	\nonumber
	&=\sum^{l(n)}_{q=0}I(X_{A_{q,n}(U_{n}\setminus U^{*})};Y_{d}|X_{\tilde{A}_{q,n}(U_{n}\setminus U^{*})})\\
	\label{newgrandfinale11}
	&\hspace{23mm}+I(X_{F_{d}(U^{*})};Y_{d}|X_{\tilde{F}_{d}(U^{*})}),
\end{align}
where (\ref{newgrandfinale7}) follows from the definition of $U_{n}$, (\ref{newgrandfinale9}) follows from (\ref{aln2}), (\ref{newgrandfinale10}) follows from (\ref{FDU2}), and (\ref{newgrandfinale11}) follows from Claim \ref{grandefinale}.5, (\ref{FDU}) and (\ref{FDU3}).
%observe that (\ref{aln2}) implies $A_{q,n}(U^{*})=L_{q,n}$ for all $n\geq\{n_{5},n_{6}\}$.  Claim \ref{grandefinale}.1 and (\ref{U}) imply that $U^{*}\subseteq U_{n}$ for all $n\geq n_{1}$.  Since $A_{q,n}(U_{n})\subseteq L_{q,n}$ for all $n\in\mathbb{N}$, it follows that  $A_{q,n}(U^{*})\subseteq A_{q,n}(U_{n})\subseteq L_{q,n}$ for all $n\geq n_{1}$.  Therefore, $A_{q,n}(U_{n})=A_{q,n}(U^{*})$ for all $n\geq\max\{n_{1},n_{5},n_{6}\}$ which implies (\ref{newgrandfinale9}).  Since $n\geq\max\{n_{5},n_{6}\}$, we invoke (\ref{FDU2}) and (\ref{newgrandefinale6}) with the  Chain Rule to justify (\ref{newgrandfinale10}).  Moreover (\ref{newgrandfinale11}) follows because Claim \ref{grandefinale}.7 and (\ref{aln}) imply  $A_{q,n}(U_{n}\setminus U^{*})=L_{q,n}$ for all $n\geq n_{7}$ and every $q\in\{0,\ldots,l(n)\}$.  Since $A_{q,n}(U_{n}\setminus U^{*})\subseteq A_{q,n}(U_{n})\subseteq L_{q,n}$ for all $n\in\mathbb{N}$, it follows that $A_{q,n}(U_{n}\setminus U^{*})=A_{q,n}(U_{n})$ for all $n\geq n_{7}$ and every  $q\in\{0,\ldots,l(n)\}$.

Now $R_{U_{n}}=R_{U_{n}\setminus U^{*}}+R_{U^{*}}$.  Since $n\geq\max\{K_{6},K_{7}\}$ we can invoke (\ref{newgrandfinale13}).  Together (\ref{newgrandfinale13}) and (\ref{newgrandfinale11}) imply:
\begin{align}
	\label{actualgrandefinale}
	R_{U^{*}}&>I(X_{F_{d}(U^{*})};Y_{d}|X_{\tilde{F}_{d}(U^{*})}).
\end{align}
By selection ${\bf R}\in{\cal R}_{d}({\bf F})$ satisfies (\ref{biggiewiggie}) for all $S\subseteq{\cal S}(d)$, which contradicts (\ref{actualgrandefinale}).  It follows that the non-empty $U^{*}$ defined in (\ref{U}) does not exist.  Therefore Claim \ref{grandefinale}.1 implies ${\bf R}\in{\cal R}({\bf F},{\bf L}_{d,n})$ for some $n\in\mathbb{N}$.
\end{proof}


==> flowdecomp 2/induction.tex <==
\begin{lemma}
	\label{induction}
	$Z^{\prime}=({\cal S}(d)\setminus U)\cup Z$.
\end{lemma}
\begin{proof}
	The proof is by contradiction.  Suppose there is some $S\subseteq({\cal S}\setminus U)\cup Z$ that violates (\ref{flowdecomp2}) for $({\bf F},{\bf L}^{\prime}_{d})$.  Then:
	\begin{align}
		\label{lemmaVprep2}
		R_{S}&>\sum^{|{\bf  L}^{\prime}_{d}|-1}_{l=0}I(X_{A^{\prime}_{l}(S)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S)}).
	\end{align}
	To simplify the analysis, we first examine the case $S\cap U=\{\}$ and then consider $S\cap U\neq\{\}$.
	
	\hspace{-3.5mm}{\bf Case 1:}  $S\cap U=\{\}$.
	
	We will prove the following sequence of inequalities:
	\begin{align}
		\nonumber
		R_{U\cup S}&>\sum^{|{\bf L}_{d}|-1}_{k=0}I(X_{A_{k}(U)};Y_{d}|X_{\tilde{A}_{k}(U)})\\
		\label{lemmaU1}
		&\hspace{20mm}+\sum^{|{\bf L}^{\prime}_{d}|-1}_{l=0}I(X_{A^{\prime}_{l}(S)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S)}),\\
		\nonumber
		&\geq\sum^{|{\bf L}_{d}|-1}_{k=0}I(X_{A_{k}(U)};Y_{d}|X_{\tilde{A}_{k}(U)})\\
		\label{lemmaU2}
		&\hspace{3mm}+\sum^{|{\bf L}_{d}|-1}_{l=0}I(X_{A_{l}(S)\setminus A_{l}(U)};Y_{d}|X_{\tilde{A}_{l}(S)\setminus A_{l}(U)}),\\
		\nonumber
		&=\sum^{|{\bf L}_{d}|-1}_{k=0}(I(X_{A_{k}(U)};Y_{d}|X_{\tilde{A}_{k}(U)})\\
		\label{lemmaU3}
		&\hspace{8mm}+I(X_{A_{k}(S)\setminus A_{k}(U)};Y_{d}|X_{\tilde{A}_{k}(S)\setminus A_{k}(U)})),\\
		\label{lemmaU4}
		&=\sum^{|{\bf L}_{d}|-1}_{k=0}I(X_{A_{k}(U)\cup A_{k}(S)};Y_{d}|X_{\tilde{A}_{k}(S)\setminus A_{k}(U)}),\\
		\label{lemmaU5}
		&=\sum^{|{\bf L}_{d}|-1}_{k=0}I(X_{A_{k}(U\cup S)};Y_{d}|X_{\tilde{A}_{k}(U\cup S)}),
	\end{align}
which contradicts the assumption that $U$ is the largest subset that violates (\ref{flowdecomp}) since $S$ and $U$ are disjoint.  Define:
\begin{align}
	\label{induction3}
	F_{I(d)}&:=\cup_{j\in I(d)}F_{j}({\cal N})\setminus F_{d}({\cal N}),
\end{align}
where $I(d)$ is defined in (\ref{id}).  To justify (\ref{lemmaU1}) - (\ref{lemmaU5}), observe that $\tilde{A}^{\prime}_{l}(S)$ defined in (\ref{Atildeprime}) can be rewritten as follows for any $S\subseteq{\cal S}(d)$:
\begin{align}
	\label{induction1}
	\tilde{A}^{\prime}_{l}(S)&=F_{I(d)}\cup F_{d}({\cal N})\setminus(\cup^{|{\bf L}^{\prime}_{d}|-1}_{q=l+1}L^{\prime}_{q}\cup A^{\prime}_{l}(S)),\\
	\label{induction2}
	&=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S),
\end{align}
where (\ref{induction1}) follows from (\ref{Atildeprime}) and (\ref{induction3}), and (\ref{induction2}) follows because $\cup^{|{\bf L}^{\prime}_{d}|-1}_{q=0}L^{\prime}_{q}=F_{d}({\cal N})$.  Similarly, $\tilde{A}_{l}(S)$ defined in (\ref{Atilde}) can be rewritten as follows for any $S\subseteq{\cal S}(d)$:
\begin{align}
	\label{induction7}
	\tilde{A}_{l}(S)&=F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\setminus A_{l}(S).
\end{align}  

Now observe that (\ref{lemmaU1}) follows from (\ref{lemmaVprep2}) and the definition of $U$.  To justify (\ref{lemmaU2}) we prove the following claims:

\hspace{-3.5mm}{\bf Claim \ref{induction}.1}  \textit{If $S_{1}\subseteq{\cal N}$, $S_{3}\subseteq S_{2}\subseteq{\cal N}$ and $S_{1}\cap S_{2}=\{\}$ then:}
\begin{align}
	\nonumber
	&\hspace{-2.5mm}I(X_{S_{1}};Y_{d}|X_{S_{2}})+I(X_{S_{3}};Y_{d}|X_{S_{2}\setminus S_{3}})\\
	&\hspace{35mm}=I(X_{S_{1}\cup S_{3}};Y_{d}|X_{S_{2}\setminus S_{3}}).
\end{align}
\begin{proof}
	Apply the chain rule.
\end{proof}


\hspace{-3.5mm}{\bf Claim \ref{induction}.2}  \textit{If $S_{1}\subseteq S_{2}\subseteq S_{3}\subseteq{\cal N}$ then:} 
\begin{align}
\label{induction9}
I(X_{S_{2}};Y_{d}|X_{S_{3}\setminus S_{2}})&\geq I(X_{S_{1}};Y_{d}|X_{S_{3}\setminus S_{1}}).
\end{align}

\begin{proof}
Consider the following inequalities:
\begin{align}
	\nonumber
	&\hspace{-2.5mm}I(X_{S_{1}};Y_{d}|X_{S_{3}\setminus S_{1}})+I(X_{S_{2}\setminus S_{1}};Y_{d}|X_{S_{3}\setminus(S_{1}\cup S_{2})})\\
	\label{preinduction4}
	&\hspace{21mm}=I(X_{S_{1}\cup(S_{2}\setminus S_{1})};Y_{d}|X_{S_{3}\setminus(S_{1}\cup S_{2})}),\\
	\label{induction4}
	&\hspace{21mm}=I(X_{S_{1}\cup(S_{2}\setminus S_{1})};Y_{d}|X_{S_{3}\setminus S_{2}}),\\
	\label{induction5}
	&\hspace{21mm}=I(X_{S_{1}\cup S_{2}};Y_{d}|X_{S_{3}\setminus S_{2}}),\\
	\label{induction6},
	&\hspace{21mm}=I(X_{S_{2}};Y_{d}|X_{S_{3}\setminus S_{2}}).
\end{align}
To justify (\ref{preinduction4}), let $S^{\prime}_{1}:=S_{1}$, $S^{\prime}_{2}:=S_{3}\setminus S_{1}$, and $S^{\prime}_{3}:=S_{2}\setminus S_{1}$.  First we verify that the premises of Claim \ref{induction}.1 are satisfied.  Since $S_{1}\subseteq S_{2}\subseteq S_{3}$, it follows that $(S_{2}\setminus S_{1})\subseteq(S_{3}\setminus S_{1})$, which implies $S^{\prime}_{3}\subseteq S^{\prime}_{2}$.  Furthermore, $S_{1}\cap(S_{3}\setminus S_{1})=\{\}$ which implies $S^{\prime}_{1}\cap S^{\prime}_{2}=\{\}$.  Finally, $S^{\prime}_{2}\setminus S^{\prime}_{3}=(S_{3}\setminus S_{1})\setminus (S_{2}\setminus S_{1})=S_{3}\setminus(S_{1}\cup(S_{2}\setminus S_{1}))=S_{3}\setminus(S_{1}\cup S_{2})$.  Now we can invoke Claim \ref{induction}.1 to justify (\ref{preinduction4}).  Since $S_{1}\subseteq S_{2}$, (\ref{induction4}) follows from (\ref{preinduction4}) and the fact that $S_{1}\subseteq S_{2}$ and (\ref{induction6}) follows from (\ref{induction5}) and the same fact.  By the non-negativity of mutual-information, $I(X_{S_{2}\setminus S_{1}};Y_{d}|X_{S_{3}\setminus(S_{1}\cup S_{2})})\geq0$.  Therefore (\ref{induction6}) implies (\ref{induction9}) which completes the proof of Claim \ref{induction}.2.
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{induction}.3} \textit{For any $S\subseteq{\cal S}(d)$ and every $l\in 0,\ldots,|{\bf L}_{d}|-1$:}
\begin{align}
\nonumber
&\hspace{-2mm}I(X_{A^{\prime}_{l}(S)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S)})\\
\label{induction8}
&\hspace{19mm}\geq I(X_{A_{l}(S)\setminus A_{l}(U)};Y_{d}|X_{\tilde{A}_{l}(S)\setminus A_{l}(U)})
	\end{align}	
	
\begin{proof}
To justify (\ref{induction8}), we invoke Claim \ref{induction}.2.  First we verify that the premises of Claim \ref{induction}.2 are satisfied.  Let  $S_{1}:=A_{l}(S)\setminus A_{l}(U)$, $S_{2}:=A^{\prime}_{l}(S)$, and $S_{3}:=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})$.  Lemma \ref{disjoint} implies $S_{1}\subseteq S_{2}$.  It follows from (\ref{Aprime}) that $A^{\prime}_{l}(S)\subseteq L^{\prime}_{l}$.  Therefore $S_{2}\subseteq S_{3}$.  Moreover, (\ref{induction2}) implies $\tilde{A}^{\prime}_{l}(S):=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S)=S_{3}\setminus S_{2}$.  In addition:
\begin{align}
\label{preinduction14}
S_{3}\setminus S_{1}=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus(A_{l}(S)\setminus A_{l}(U)).	
\end{align}
For every $l=0,\ldots,|{\bf L}_{d}|-1$, (\ref{shift2}) implies:
\begin{align}
\label{induction14}
\cup^{l}_{q=0}L^{\prime}_{q}=\cup^{l}_{q=0}L_{q}\setminus A_{l}(U).	
\end{align}
Substituting (\ref{induction14}) into (\ref{preinduction14}) gives $S_{3}\setminus S_{1}=F_{I(d)}\cup(\cup^{l}_{q=0}L_{q}\setminus A_{l}(U))\setminus(A_{l}(S)\setminus A_{l}(U))=F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\setminus(A_{l}(S)\cup A_{l}(U))$.  It follows that $S_{3}\setminus S_{1}=\tilde{A}_{l}(S)\setminus A_{l}(U)$, since (\ref{induction7}) implies $\tilde{A}_{l}(S):=F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\setminus A_{l}(S)$.  Therefore (\ref{induction8}) follows from Claim \ref{induction}.2.
\end{proof}

To justify (\ref{lemmaU2}), invoke Claim \ref{induction}.3 for $l=0,\ldots,|{\bf L}_{d}|-1$ and observe that (\ref{shift2}) implies $|{\bf L}_{d}|\leq|{\bf L}^{\prime}_{d}|$.  Since mutual informations are always non-negative, (\ref{lemmaU2}) is justified.  

\hspace{-3.5mm}{\bf Claim \ref{induction}.4} \textit{For any $S\subseteq{\cal S}(d)$ and every $l\in 0,\ldots,|{\bf L}_{d}|-1$:}
\begin{align}
\nonumber
&\hspace{-4mm}I(X_{A_{k}(U)};Y_{d}|X_{\tilde{A}^{\prime}_{k}(U)})\\
\nonumber
&\hspace{13mm}+I(X_{A_{k}(S)\setminus A_{k}(U)};Y_{d}|X_{\tilde{A}_{k}(S)\setminus A_{k}(U)})\\
\label{induction8a}
&\hspace{13mm}=I(X_{A_{k}(U)\cup A_{k}(S)};Y_{d}|X_{\tilde{A}_{k}(S)\setminus A_{k}(U)})
	\end{align}
\begin{proof}
To prove (\ref{induction8a}), we invoke Claim 6.1.  First, we verify that the premises of Claim 6.1 are satisfied.  Let $S_{1}:=A_{k}(U)$, $S_{2}:=\tilde{A}_{k}(U)$, and $S_{3}:=A_{k}(S)\setminus A_{k}(U)$.  From (\ref{induction7}):
\begin{align}
	\label{induction8b}
	\tilde{A}_{k}(U)=F_{I(d)}\cup(\cup^{k}_{q=0}L_{q})\setminus A_{k}(U).
\end{align}
Since $A_{k}(S)\subseteq L_{k}$, (\ref{induction8b}) implies $S_{3}\subseteq S_{2}$.  By inspection, $S_{1}\cap S_{2}=\{\}$.  Finally,
\begin{align}
	\nonumber
	&\hspace{-3mm}S_{2}\setminus S_{3}\\
	\nonumber
	&\hspace{-3mm}=\tilde{A}_{k}(U)\setminus (A_{k}(S)\setminus A_{k}(U)),\\
	\nonumber
	&\hspace{-3mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\setminus A_{k}(U))\setminus(A_{k}(S)\setminus A_{k}(U)),\\
%	\nonumber
%	&\hspace{3mm}\hspace{-9mm}\hspace{30mm}\setminus(A_{k}(S)\setminus A_{k}(U)),\\
	\nonumber
	&\hspace{-3mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L_{q}))\setminus(A_{k}(S)\cup A_{k}(U)),\\
	\nonumber
	%&\hspace{3mm}\hspace{-9mm}\hspace{30mm}\setminus(A_{k}(S)\cup A_{k}(U)),\\
	\nonumber
	&\hspace{-3mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\setminus A_{k}(S))\setminus A_{k}(U),\\
	\label{induction8d}
	&\hspace{-3mm}=\tilde{A}_{k}(S)\setminus A_{k}(U),
\end{align}
where the equalities follow from normal set-theoretic operations and (\ref{induction8b}).  Furthermore,
	\begin{align}
		\nonumber
		S_{1}\cup S_{3}&=A_{k}(U)\cup(A_{k}(S)\setminus A_{k}(U))\\
		\label{induction8c}
		&=A_{k}(U)\cup A_{k}(S).
	\end{align}
	The premises of Claim 6.1 are satisfied in (\ref{induction8a}),  (\ref{induction8d}) and  (\ref{induction8c}). 
\end{proof}
Relabeling (\ref{lemmaU2}) gives (\ref{lemmaU3}).  To justify (\ref{lemmaU4}), invoke Claim 6.4 for $l=0,\ldots,|{\bf L}_{d}|-1$.  Now (\ref{A}) implies $i\in A_{k}(S\cup U)$ if and only if $i\in A_{k}(S)\cup A_{k}(U)$.  Therefore $A_{k}(S\cup U)=A_{k}(S)\cup A_{k}(U)$.  In addition:
\begin{align}
	\nonumber
	\tilde{A}_{k}(S)\setminus A_{k}(U)&=(F_{I(d)}\cup(\cup^{k}_{q=0}L_{q})\setminus A_{k}(S))\setminus A_{k}(U),\\
	\nonumber
	&=(F_{I(d)}\cup(\cup^{k}_{q=0}L_{q}))\setminus(A_{k}(S)\cup A_{k}(U)),\\
	\nonumber
	&=(F_{I(d)}\cup(\cup^{k}_{q=0}L_{q}))\setminus A_{k}(S\cup U),\\
	\label{induction8e}
	&=\tilde{A}_{k}(S\cup U),
\end{align} 
where the equalities follow from normal set-theoretic operations.  Applying (\ref{induction8e}) to (\ref{lemmaU4}) gives (\ref{lemmaU5}), which proves Lemma \ref{induction} for Case 1.

%Both $A^{\prime}_{l}(\cdot)$ and $\tilde{A}^{\prime}_{l}(\cdot)$ in (\ref{lemmaU1}) are defined with respect to $(F,\bar{L}^{\prime}_{d})$, whereas $A_{l}(\cdot)$ and $\tilde{A}_{l}(\cdot)$ in (\ref{lemmaU1}) and  (\ref{lemmaU2}) are defined with respect to $(F,\bar{L}_{d})$.  %To see why (\ref{lemmaU1}) leads to (\ref{lemmaU2}), recognize that $A_{l}(U)\subseteq\tilde{A}^{\prime}_{l}(S)$ since $S$ and $U$ are disjoint.  

\hspace{-3.5mm}{\bf Case 2:}  $S\cap U\neq\{\}$.  

Since $(S\setminus U)\cap U=\{\}$, Case 1 implies:
\begin{align}
\label{lemmaVprep1}
	R_{S\setminus U}&<\sum^{|{\bf L}^{\prime}_{d}|-1}_{l=0}I(X_{A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)}).
\end{align}
We will prove the following sequence of inequalities:
\begin{align}
		\nonumber
		&\hspace{-2.7mm}R_{S\cap U}\\
		\label{lemmaV1}
		&\hspace{-2.5mm}>\sum^{|{\bf L}^{\prime}_{d}|-1}_{l=0}I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)}),\\
		\label{lemmaV2}
		&\hspace{-2.5mm}\geq\sum^{|{\bf L}_{d}|-1}_{l=0}I(X_{A_{l}(S\cap U)};Y_{d}|X_{\tilde{A}_{l}(S\cap U)}).
\end{align}
Since $S\subseteq({\cal S}(d)\setminus U)\cup Z$ by hypothesis, it follows that $(S\cap U)\subseteq Z$.  Therefore (\ref{lemmaV2}) contradicts the assumption that all subsets of $Z$ satisfy (\ref{flowdecomp}) for $({\bf F},{\bf L}_{d})$.  First we show (\ref{lemmaV1}).

\hspace{-3.5mm}{\bf Claim \ref{induction}.5}   \textit{For any $S\subseteq{\cal S}(d)$:}
\begin{align}
	\nonumber
	R_{S\cap U}>\sum^{|{\bf L}^{\prime}_{d}|-1}_{l=0}I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})
\end{align}

\begin{proof}
Fix any $l\in\{0,\ldots,|{\bf L}^{\prime}_{d}|-1\}$ and consider the following sequence of equalities:
\begin{align}
\nonumber
&\hspace{-3mm}I(X_{A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)})\\
   \nonumber
	&\hspace{3mm}+I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})\\
	\label{induction10}
	&\hspace{3mm}= I(X_{A^{\prime}_{l}(S\setminus U)\cup A^{\prime}_{l}(S\cap U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)}),\\
	\label{induction11}
	&\hspace{3mm}= I(X_{A^{\prime}_{l}(S)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S)}).
\end{align}
To justify (\ref{induction10}), we invoke Claim \ref{induction}.1.  First, we verify that  the premises of Claim \ref{induction}.1 are satisfied.  Let $S_{1}:=A^{\prime}_{l}(S\setminus U)$, $S_{2}:=\tilde{A}^{\prime}_{l}(S\setminus U)$, and $S_{3}:=A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)$.  By inspection $S_{1}\cap S_{2}=\{\}$.  Observe that (\ref{Aprime}) implies $A^{\prime}_{l}(S\cap U)\subseteq L^{\prime}_{l}$ and (\ref{induction2}) implies $\tilde{A}^{\prime}_{l}(S\setminus U):=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\setminus U)$.  It follows that: 
\begin{align}
	\label{induction16}
	A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)\subseteq\tilde{A}^{\prime}_{l}(S\setminus U),
\end{align}
which implies $S_{3}\subseteq S_{2}$.  Moreover,  
\begin{align}
	\nonumber
	&\hspace{-9mm}S_{2}\setminus S_{3}\\
	\nonumber
	&\hspace{3mm}\hspace{-9mm}=\tilde{A}^{\prime}_{l}(S\setminus U)\setminus (A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U))\\
	\nonumber
	&\hspace{3mm}\hspace{-9mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\setminus U))\\
	\nonumber
	&\hspace{3mm}\hspace{-9mm}\hspace{30mm}\setminus(A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)),\\
	\nonumber
	&\hspace{3mm}\hspace{-9mm}=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus(A^{\prime}_{l}(S\setminus U)\cup A^{\prime}_{l}(S\cap U)),\\
	\nonumber
	&\hspace{3mm}\hspace{-9mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\cap U))\setminus A^{\prime}_{l}(S\setminus U),\\
	\label{induction17}
	&\hspace{3mm}\hspace{-9mm}=\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U),
\end{align}
where the equalities follow from normal set-theoretic operations and (\ref{induction2}).  Furthermore, 
\begin{align}
	\nonumber
	S_{1}\cup S_{3}&=A^{\prime}_{l}(S\setminus U)\cup(A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U))\\
	\label{induction18}
	&=A^{\prime}_{l}(S\cap U)\cup A^{\prime}_{l}(S\setminus U).
\end{align}
Since the premises of Claim \ref{induction}.1 are satisfied in (\ref{induction16}), (\ref{induction17}), and (\ref{induction18}), invoking Claim \ref{induction}.1 proves (\ref{induction10}). 
\begin{align}
\nonumber
&\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)\\
\label{induction12}
&=(F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\cap U))\setminus A^{\prime}_{l}(S\setminus U),\\
\label{induction13}
&=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus(A^{\prime}_{l}(S\cap U)\cup A^{\prime}_{l}(S\setminus U)),\\
\label{postinduction13}
&=\tilde{A}^{\prime}_{l}(S),
\end{align}
where (\ref{induction12}) follows from (\ref{induction2}) and (\ref{induction13}) follows from normal set-theoretic operations.  The definition of (\ref{Aprime}) implies that $i\in A^{\prime}_{l}(S)$ if and only if $i\in A^{\prime}_{l}(S\setminus U)\cup A^{\prime}_{l}(S\cap U)$.  Therefore $A^{\prime}_{l}(S)=A^{\prime}_{l}(S\setminus U)\cup A^{\prime}_{l}(S\cap U)$ which implies (\ref{postinduction13}). Therefore (\ref{induction11}) follows from (\ref{postinduction13}).  Since  $R_{S}=R_{S\setminus U}+R_{S\cap U}$, Claim \ref{induction}.4 follows from (\ref{lemmaVprep2}), (\ref{lemmaVprep1}), and  (\ref{induction11}).
\end{proof} 
We invoke Claim \ref{induction}.5 to justify (\ref{lemmaV1}).  To prove (\ref{lemmaV2}), we introduce more preliminary claims.
 
 \hspace{-3.5mm}{\bf Claim \ref{induction}.6}   \textit{For any $S\subseteq{\cal S}(d)$ and every $l=0,\ldots,|{\bf L}^{\prime}_{d}|-1$:}
\begin{align}
\nonumber
	&I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})\geq\\
	\label{induction19}
	&\hspace{15mm}I(X_{A_{l-1}(S\cap U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)\setminus A_{l-1}(S\cap U)})
\end{align}
%(\ref{lemmaV1}) follows from (\ref{lemmaVprep2}), (\ref{lemmaVprep1}), and the following inequality for $l=0,\ldots,|{\bf L}^{\prime}|-1$:
%\begin{align}
%\nonumber
%&I(X_{A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)})\\
%   \nonumber
%	&\hspace{5mm}+I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})\\
%	\nonumber
%	&\hspace{5mm}= I(X_{A^{\prime}_{l}(S\setminus U)\cup A^{\prime}_{l}(S\cap U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})\\
%	\nonumber
%	&\hspace{5mm}= I(X_{A^{\prime}_{l}(S)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S)}).
%\end{align}
\begin{proof}
We invoke Claim \ref{induction}.2 to justify Claim \ref{induction}.6.  First we verify that the premises of Claim \ref{induction}.2 are satisfied.  Let $S_{1}:=A_{l-1}(S\cap U)$, $S_{2}:=A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)$, and $S_{3}:=\tilde{A}^{\prime}_{l}(S\setminus U)$.  First, we show that $S_{3}\setminus S_{2}=\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)$.  Consider the following sequence of equalities:
\begin{align}
	\nonumber
	&\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)\\
	\label{induction15}
	&\hspace{3mm}=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus(A^{\prime}_{l}(S\cap U)\cup A^{\prime}_{l}(S\setminus U))\\
	\nonumber
	&\hspace{3mm}=(F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\setminus U))\\
	\nonumber
	&\hspace{3mm}\hspace{30mm}\setminus(A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)),\\
	\nonumber
	&\hspace{3mm}=\tilde{A}^{\prime}_{l}(S\setminus U)\setminus(A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U))\\
	\label{induction20}
	&\hspace{3mm}=S_{3}\setminus S_{2}
\end{align}
where (\ref{induction15}) follows from (\ref{induction13}) and (\ref{induction20}) follows from (\ref{induction2}) and standard set-theoretic operations.  
%\begin{align}
%	\nonumber
%	&I(X_{A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)})\geq\\
%	\label{induction21}
%	&\hspace{15mm}I(X_{A_{l-1}(S\cap U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)\setminus A_{l-1}(S\cap U)}). 
%\end{align}
Next we show that $S_{1}\subseteq S_{2}$.  It follows from Lemma \ref{join} that $A_{l-1}(S\cap U)\subseteq A^{\prime}_{l}(S\cap U)$.  Moreover, Lemma \ref{remain} implies $A^{\prime}_{l}(S\setminus U)\subseteq A_{l}(S\setminus U)$.  Now (\ref{A}) implies $A_{l-1}(S\cap U)\subseteq L_{l-1}$ and $A_{l}(S\setminus U)\subseteq L_{l}$.  Moreover, (L2) implies $L_{l-1}\cap L_{l}=\{\}$.  It follows that $A_{l-1}(S\cap U)\cap A^{\prime}_{l}(S\setminus U)=\{\}$.  Therefore $A_{l-1}(S\cap U)\subseteq A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)$, or equivalently $S_{1}\subseteq S_{2}$.  Finally, we show $S_{2}\subseteq S_{3}$.  Since (\ref{Aprime}) implies $A^{\prime}_{l}(S\cap U)\subseteq L^{\prime}_{l}$ it follows that $A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)\subseteq F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\setminus U)$ which implies $S_{2}\subseteq S_{3}$.  Therefore Claim \ref{induction}.2 implies (\ref{induction19}).
%(Lemma \ref{join}), (\ref{induction16}) follows by substituting (\ref{induction14}) into (\ref{induction15}).  Moreover:
%From (\ref{induction13}) we have $\tilde{A}^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus\{A^{\prime}_{l}(S\cap U)\cup A^{\prime}_{l}(S\setminus U)\}=\{\cup^{l}_{q=0}L_{q}\}\setminus\{A^{\prime}_{l}(S\cap U)\cup A^{\prime}_{l}(S\setminus U)\cup A_{l}(U)\}$.
%Since $A_{l-1}(S\cap U)\subseteq A^{\prime}_{l}(S\cap U)$ (Lemma \ref{join}), $A^{\prime}_{l}(S\setminus U)\subseteq A_{l}(S\setminus U)$ (Lemma \ref{remain}), and $A_{l-1}(S\cap U)\cap A_{l}(S\setminus U)=\{\}$, it follows that $A_{l-1}(S\cap U)\subseteq A^{\prime}_{l}(S\cap U)\setminus A^{\prime}_{l}(S\setminus U)$. 
\end{proof} 

 \hspace{-3.5mm}{\bf Claim \ref{induction}.7}   \textit{For any $S\subseteq{\cal S}(d)$ and every $l=0,\ldots,|{\bf L}^{\prime}_{d}|-1$:}
\begin{align}
	\nonumber
	&\hspace{-5mm}I(X_{A_{l-1}(S\cap U)};Y_{d}|X_{\tilde{A}^{\prime}_{l}(S\setminus U)\setminus A_{l-1}(S\cap U)})\geq\\
	&\hspace{25mm}I(X_{A_{l-1}(S\cap U)};Y_{d}|X_{\tilde{A}_{l-1}(S\cap U)}).
\end{align}
\begin{proof}
Consider the following sequence of inequalities:
\begin{align}
	\nonumber
	&\tilde{A}^{\prime}_{l}(S\setminus U)\setminus A_{l-1}(S\cap U)\\
	\label{induction21}
	&=(F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus A^{\prime}_{l}(S\setminus U))\setminus A_{l-1}(S\cap U),\\
	\label{induction22}
	&=F_{I(d)}\cup(\cup^{l}_{q=0}L^{\prime}_{q})\setminus (A^{\prime}_{l}(S\setminus U)\cup A_{l-1}(S\cap U)),\\
	\nonumber
	&=F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\\
	\label{induction23}
	&\hspace{17mm}\setminus(A^{\prime}_{l}(S\setminus U)\cup A_{l-1}(S\cap U)\cup A_{l}(U)),\\
	\nonumber
	&\supseteq F_{I(d)}\cup(\cup^{l}_{q=0}L_{q})\\
	\label{induction24}
	&\hspace{17mm}\setminus(A_{l}(S\setminus U)\cup A_{l-1}(S\cap U)\cup A_{l}(U)),\\
	\label{induction25}
	&\supseteq F_{I(d)}\cup(\cup^{l-1}_{q=0}L_{q})\setminus A_{l-1}(S\cap U),\\
	\label{induction26}
	&=\tilde{A}_{l-1}(S\cap U),
\end{align}
where (\ref{induction21}) follows from (\ref{induction2}), (\ref{induction22}) follows from standard set-theoretic operations, (\ref{induction23}) follows by substituting (\ref{induction14}) into (\ref{induction22}), (\ref{induction24}) follows because Lemma \ref{remain} implies $A^{\prime}_{l}(S\setminus U)\subseteq A_{l}(S\setminus U)$, (\ref{induction25}) follows because (\ref{A}) implies $A_{l}(U)\cup A_{l}(S\setminus U)\subseteq L_{l}$, and (\ref{induction26}) follows from the definition of $\tilde{A}_{l}(\cdot)$ in (\ref{induction7}).  Since removing independent conditional random variables reduces the mutual information, Claim \ref{induction}.7 follows from (\ref{induction26}).
\end{proof}
Combining Claim \ref{induction}.6 and Claim \ref{induction}.7 proves that (\ref{lemmaV2}) follows from (\ref{lemmaV1}).  Moreover, (\ref{lemmaV2}) implies:
\begin{align}
	\label{induction27}
	R_{S\cap U}&>\displaystyle\sum^{|{\bf L}^{\prime}_{d}|-1}_{l=0}I(X_{A_{l-1}(S\cap U)};Y_{d}|X_{\tilde{A}_{l-1}(S\cap U)}).
\end{align}
Observe that (\ref{shift2}) implies $|{\bf L}_{d}|\leq|{\bf L}^{\prime}_{d}|\leq|{\bf L}_{d}|+1$.  Since $ l\leq|{\bf L}_{d}^{\prime}|-1$ it follows that $l-1\leq|{\bf L}^{\prime}_{d}|-2\leq|{\bf L}_{d}|-1$.  Substituting $l^{\prime}=l-1$ into (\ref{induction27}) and relabelling $l^{\prime}=l$ yields (\ref{lemmaV2}) which completes the proof of Lemma \ref{induction}.
\end{proof}


==> flowdecomp 2/introduction.tex <==
\section{Introduction}
  The relay channel consists of three nodes: a source, a relay, and a destination \cite{Meulen1971}.  The source transmits messages to the destination through a “noisy” channel (the output symbols in each use of the channel are statistically related to the input symbols via some probability transition function).  After observing its own channel outputs, the relay attempts to help the destination decode messages sent by the source.  Although the capacity of the relay channel is not fully understood, the channel is still a useful building block for studying general networks from an information-theoretic perspective.  

Two strategies of interest in this channel are decode-forward (DF), where the relay decodes and forwards each message to the destination, and compress-forward (CF), where the relay forwards a compression of the channel observations instead of the message itself \cite{GamalCover}.  Neither strategy is universally better than the other.  %Both strategies capture fundamental issues in general networks involving cooperation, competition, and complexity. 

%The core problem in network information theory is deciding (in finite time) whether or not any desired rate-vector is achievable in some general network.  Since this problem is unsolved for even three-node channels, it may be tempting to dismiss any further study of general channels with arbitrarily many nodes until a solution for three nodes is found.  This would be a mistake.  The difficulty in three-node channels is probabilistic in nature and tied to the optimal way of exploiting correlation between random variables \cite{distributedcoord}.  The problems in networking are of a different flavor, and tend to fall under the scope of graph theory and combinatorics.  Ultimately, all of these problems need to be solved in a single comprehensive framework.  In the meantime, it makes sense to separate the probabilistic issues in network information theory from the combinatorial ones.

The ``complexity'' of an achievable region describes the number of computations required to check whether a desired rate-vector is in the region, with respect to the number of nodes (another aspect of complexity is finding an encoding/decoding scheme that actually achieves this rate-vector).  
%While the capacity region of general channels is unknown, it appears to depend in some way on the number of nodes in the channel and the correlation between inputs.  
We focus on a class of regular DF schemes that generalize index coding.  Regular schemes have the short delays (linear in the channel usage) associated with sliding-window decoding instead of the long (exponential) delays and restrictions on bidirectional communication associated with backward decoding.  A fundamental tension exists in channels with bidirectional communication; nodes can individually benefit by waiting for others to decode first, but some node must always be the first to decode  \cite{Ponniah2016}.  The complexity of the achievable region depends on all the ways of resolving this tension.

Two sets of constraints are necessary for the DF region: first, the mutual-information inequalities derived from the one-relay channel, and second, causality constraints that ensure nodes only forward messages they have already decoded.  We introduce the framework of flow decomposition to prove these two sets of constraints are also sufficient.  Flow decomposition consists of two structures: \textit{flows} and \textit{layerings}.       
%This paper offers a way forward.  It answers whether or not any specified rate-vector is achievable in a general channel with arbitrarily many nodes, using a class of decode-forward schemes similar to network coding.  A major difficulty is the tension in bidirectional communication between the  individual nodes in the network and the network as a whole \cite{Ponniah2016}.  Individual nodes benefit from being the last to forward certain combinations of source messages because they have the flexibility to exploit previous transmissions from other nodes.  However, all nodes cannot be granted this flexibility.  The performance of the network then depends on all the ways of balancing the freedom given to individual nodes with the desired  network performance.  There are infinitely many ways of selecting from these options, which makes the conventional way of expressing achievable regions with mutual-information inequalities inadequate.
%The complexity of an achievable region depends on the “flow” of messages in the decode-forward scheme.  For some flows, namely those with hierarchical or tree-like structure, the achievable region 
%is a polymatroid whose facets correspond to mutual-information inequalities.  Such regions 
%has minimal complexity, per the number of operations needed to verify whether a rate-vector is included.  For all-cast flows, the achievable region can only be defined algorithmically at much higher complexity.  
%This paper proposes the framework of flow decomposition to characterize this achievable region and its complexity for decode-forward schemes in general channels with arbitrarily many nodes.     
Flows define the nodes which forward messages from each source (i.e., the routes), along with the integer-valued encoding delays along each “hop”.  Layerings define the messages decoded by a particular node in each block of channel uses, and correspond to ordered partitions of all the preceding nodes.  %Flow sets define the flows for each source node, and by implication, the messages encoded by all nodes in each block of channel uses.  For any channel with a fixed number of nodes, there are infinitely many flow sets since there are infinitely many possible encoding delays.
%The message-vectors decoded in each block at a particular node correspond to \textit{layerings}, which are ordered partitions of all the preceding nodes in the flow set.  Each disjoint set in the partition is a layer, whose order maps to a previous block of channel uses.  The aforementioned node decodes the information sent by all nodes in this layer in the targeted block.  Deeper layers probe deeper in time.  For any given flow set, there are infinitely many different layerings.
%A \textit{flow decomposition} is a flow set paired with a layering.  It specifies the messages encoded at all nodes and the messages decoded at a fixed node.  
%A distinctive feature of this framework is that messages decoded in the current block of channel uses, are not completely determined by the messages forwarded in the next block.  Decoding schemes have some freedom to operate within the confines of the encoding scheme.  There are constraints, namely, that every scheme be causal; nodes can only forward messages they have already decoded.  However, different “flows” give each node a different level of flexibility in choosing which messages to decode. 
%There is a natural way of extending the decode-forward and compress-forward rates in the one-relay channel to general multi-source multi-relay channels, which gives an outer-bound on the decode-forward region.  This outer-bound depends on the sequence of nodes in the flow set, but not on the encoding delays.  There are no explicit conditions on causality, so the bound could be loose.

Index-coding fits naturally within two types of flow: hierarchical flow, where the routing topology is similar to a tree, and all-cast flow, where the routes cover all nodes.  For any arbitrary flow of either type and any rate-vector satisfying the mutual-information constraints at a specific node, we show  there are ``equivalent'' flows and a layering that achieves the rate-vector and satisfies the causality constraints.  Equivalence, in this context, means the flows are identical up to (but excluding) the encoding delays and thus generate the same mutual-information constraints.  This result implies both sets of constraints are sufficient to define the achievable region; the causality constraints at any fixed node can be ``deactivated'' using equivalent flows.  

Whether or not the causality constraints can be deactivated at \textit{all} nodes simultaneously is a question addressed in separate work.  By way of preview, the answer is yes for hierarchical flow, which implies the achievable region has minimal complexity.  The answer is no for all-cast channels, which raises another question of whether the all-cast region is even computable; there are infinitely many flows and layerings in a channel with a fixed number of nodes.  It turns out the region is computable, but at much higher complexity \cite{Ponniah2018}.
%The main result of this paper is that for any flow set, any rate-vector in the outer-bound \textit{evaluated at a fixed relay}, is achievable.  Moreover, the corresponding flow decomposition is both causal and equivalent to the original flow (causal flow decompositions only encode messages they have already decoded and equivalent flows are identical up to the encoding delays).  Whether this rate-vector is simultaneously achievable at all nodes is a question addressed in future work.  By way of preview, it turns out that the complexity of enforcing causality at all nodes depends on the type of flow.  Hierarchical flow achieves the decode-forward outer-bound, which implies minimal complexity \cite{Ponniah2020}.  All-cast flow, on the other hand, includes bidirectional communication and is subject to the internal tensions mentioned before.  In this complicated setting, flow decomposition provides a computable way of enforcing causality \cite{Ponniah2018}.

The proof of the main result relies on a \textit{shift} operation.  For any fixed  rate-vector satisfying the mutual-information constraints, the shift operation returns a layering with an achievable region  that is ``closer'' to the target rate-vector.  We construct a sequence of shifted layerings and prove the sequence of achievable regions eventually includes the target.  An extra step is required to find equivalent flows and a layering that satisfies the causality constraints.  

The CF setting (not addressed here) requires no notion of flow and no causality constraints, since relays do not forward source  messages.  A simplified version of this proof works for CF schemes \cite{PonniahCompressForward2019}.

%In the compress-forward setting, the notion of “flow” is meaningless because relays decode compressions not the messages themselves.  However, “layerings” retain their meaning.  The proof technique outlined here thus carries over in simpler form, without the tensions and complications from causality that arise in the decode-forward setting.

%The class of decode-forward schemes considered in this paper encodes multiple messages into a single index.  The index rate must exceed the sum rate of all the encoded source messages.  Any desired set of messages can only be decoded if all other messages represented in the index are already known as “side information” \cite{FundamentalsofIndexCoding2018}.  For this reason, hierarchical and all-cast flow fit naturally within the index-coding framework. 

%The decode-forward schemes in this paper inherit the independent input distributions from index-coding and network coding.
%The original decode-forward scheme used superposition coding to induce correlated input distributions.  Although index-coding requires independent input distributions, it is not a special case of super-position coding and the former is sometimes better than the latter \cite{Ponniah2008}.  Flow decomposition, with further development, can also support superposition coding.

Section \ref{background} provides a survey of some previous work.  Section \ref{OutlineAndPreliminaries} provides a high-level overview of the main results and an outline of the proof.  The flow decomposition framework is introduced in Section \ref{FlowDecomposition}, and the main result is presented in Section \ref{mainresult}.  Section \ref{prooftheoremone} includes the proof and Section \ref{conclusion} concludes the paper.%The three-node relay channel, first proposed by Van der Meulen, consists of a source node that communicates to a destination node with the help of a relay node.  By assumption, the symbols transmitted and received by all nodes are discrete, the received symbols depend only the symbols transmitted in the same channel use, and symbols transmitted by the relay may only depend on symbols received in previous channel uses.
%new paragraph
%%The three node relay consists of a source node that communicates to a destination node with the help of a relay node.  Two different schemes are of interest in this channel: decode-forward (DF), in which the relay decodes and forwards source messages to the destination, and compress-forward (CF), in which the relay compresses its channel observations without decoding any messages, and forwards these compressions to the destination.  Neither scheme is universally better than the other.
%%Efforts to extend DF and CF to multi-source, multi-relay channels have been ongoing for several decades.  The most notable results for both schemes involve a key strategy known as ``backward-decoding'', in which information is transmitted over ``blocks'' of channel uses and the destinations wait until all blocks of transmitted symbols are received before decoding in reverse-order.
%%Backward-decoding excludes bidirectional/two-way communication in the DF setting.  For channels where joint CF/DF schemes achieve higher rates than the individual schemes, any restrictions on the latter also apply to the former.  Moreover, individual CF or DF schemes using backward decoding can only participate in joint CF/DF schemes that also use backward-decoding.  These limitations prevent a full extension of CF and DF to general networks.
  %%Regular-coding differs from backward-decoding in that the decoding occurs during each block of channel uses (not after the end of all blocks) which permits unrestricted information flow.  Another important advantage is that the encoding delays scale linearly in the number of channel uses per block, regardless of the number of nodes, whereas the delays in backward decoding scale exponentially (or worse) in the channel usage.  Unfortunately, the achievable region of any given regular-coding scheme is difficult to evaluate, because dependencies within the scheme uniquely affect the geometry of the region.  These dependencies include the order in which nodes forward information and the ways that nodes exploit this order to process information.  
%%For any channel with a fixed number of nodes, there are infinitely many different regular coding schemes, each of which achieve different rate regions.  The conventional approach of defining a single polymatroid that contains all achievable rate-vectors is not viable.  Whether or not a given rate-vector is achievable by any regular-coding scheme, requires an algorithmic solution.
%%Capacity regions in the literature are usually expressed in polymatroid form.  There is an aesthetic appeal to these results that can be measured in terms of complexity.  To check whether or not a rate-vector lies within a polymatroid, it suffices to check that the rate-vector satisfies all of the constraints defining the boundaries of the polymatroid.  The number of operations required is at least equal to the number of boundary facets, which in turn is given by the cut-set outer-bound, since each cut defines a facet of the region.  Polymatroid capacity regions when they exist, are thus algorithmic solutions of minimal complexity.  
%%Applying this insight, any analysis of general networks should first confine itself in scope to polymatroid solutions, before addressing more complicated issues.  In that spirit, we propose the framework of flow decomposition to extend DF schemes to general networks with arbitrary information flow.
%%Flow decompositions are ``objects'' in a mathematical space that correspond to specific regular-coding DF schemes.  The objects are related to each other through a $\text{\sc shift}$ operator, and define the messages encoded at all nodes and the messages decoded at particular nodes.  Each flow decomposition object consists of a ``flow'' and a ``layering''.  The main contribution of this paper is a method of finding flow decompositions that support desired rate-vectors, using the $\text{\sc shift}$ operator.  The key ideas are expanded below.
%%1) \textit{Flows} define the sequences of nodes that forward messages from a given source node and the corresponding block-level integer-valued encoding delays along each ``hop''.  Flow sets consist of flows for each source node, and completely define the source messages encoded by all nodes in each block of channel uses.  For any channel with a fixed number of nodes, there are infinitely many flow sets since there are infinitely many possible encoding delays.  
%%A polymatroid outer-bound on the achievable region of any DF scheme (regular or otherwise) in terms of the flow set, can be derived from cut-set type arguments.  This bound is independent of the encoding delays.  Cut-set arguments are not tight in general, because they do not properly account for causality in DF schemes; the requirement that nodes can only forward messages they have already decoded.  Flows are unique to the DF setting since CF schemes do not forward source messages. 
%%2) \textit{Layerings} are ordered partitions of the nodes preceding some fixed destination.  For any given flow set, there are infinitely many different layerings, each of which define different decoding schemes.  Each layering consists of multiple layers; disjoint sets of nodes that map to previous blocks of channel uses.  The destination only decodes information sent by nodes in the blocks corresponding to their layers.  ``Deeper'' layers convey information from blocks deeper in time.  A flow set paired with a layering, completely defines a regular decoding scheme at a particular node, namely, the messages decoded by the node during each block of channel uses.  This pairing is called a \textit{flow decomposition}.
%%CF schemes generate compressions instead of source messages.  Each node uses compressions forwarded by other nodes to generate its own.  These chains of dependencies also correspond to layerings.  Hence, the concepts and theorems presented in this paper apply in simplified form to CF schemes, without the extra complexity of flows and flow decompositions.
%%3) \textit{Causal} flow decompositions at a given node, specify regular DF schemes in which the node only forwards messages it has already decoded.  A rate-vector is achievable in the DF setting if it can be simultaneously supported by all nodes in the channel.  The key result of this paper is that any rate-vector in the DF cut-set outer-bound is achievable by some causal flow decomposition at a fixed node.  
%%Whether or not a given rate-vector is simultaneously achievable by causal schemes at all nodes in the channel, is a question addressed in future work.  By way of preview, the complexity of enforcing causality at all nodes depends on the type of flow pattern.  Hierarchical flow achieves the cut-set minimal complexity, because it turns out that the achievable region coincides with the DF outer-bound.  By contrast, the solution for all-cast flow, has much higher complexity.  
%%4) \textit{The \text{\sc shift} operation} returns a flow decomposition that is ``closer'' to the target rate-vector than the operand.  Shifting the nodes that encode selected messages down down one layer, improves the decoding rates of those messages.  
%%The process of finding a causal flow decomposition that achieves a desired rate-vector occurs over two steps.  For any rate-vector in the DF outer-bound, a sequence of shifted flow decompositions is first constructed that achieves the target after some finite number of shift operations.  Redundant partition layers are then removed to create a causal flow decomposition from the outcome of the previous step.
%%5) DF \textit{Index Coding} (DFIC) is a type of DF scheme in which nodes encode multiple messages into a single index.  Like conventional index coding, the rate of the index code must exceed the sum rate of all the encoded source messages, and any desired set of messages can only be decoded if all other messages represented in the index are already known as ``side information''.  Characterizing the flow patterns that satisfy this  condition remains an open problem.  Hierarchical and all-cast flow, two flow types considered here, satisfy this condition by inspection.  
%%The input distributions in DFIC are independent, but other flavors of DF based on superposition coding are not always better, even though they enable correlated input distributions.  DFIC is the simplest non-trivial DF scheme that captures the notion of side-information in general networks. 

\section{Literature Review}
\label{background}
The relay channel was first proposed in \cite{Meulen1971}.  The CF and DF schemes for the one-relay channel appear in \cite{GamalCover}.  In its original form, the DF scheme combined super-position coding, random binning, and list-decoding.  This scheme was simplified and streamlined for multi-relay channels in \cite{KramerGastpar} and \cite{XieMultiLevel}.  The binning and list decoding strategy was replaced by a joint typicality decoding scheme called sliding-window decoding, that first appeared for the “multiple-access channel with generalized feedback” in \cite{Carleial1982}.  Sliding-window (or regular) decoding, was a precursor for the DF schemes we consider.  A different scheme from regular decoding called “backward-decoding” was proposed for the “multiple-access channel with cribbing encoders” \cite{willems}.  

While backward-decoding and regular decoding achieve the same rates in the one-source multi-relay channel in \cite{XieMultiLevel}, backward-decoding achieves higher rates in general multi-source multi-relay channels \cite{XieKumar}.  However, backward-decoding requires much longer encoding delays.  To circumvent this delay problem a variation of regular coding called “offset encoding” was proposed for the multiple-access relay channel (MARC) in \cite{Sankar}.  Three different regular decoding schemes collectively achieve the backward-decoding region in \cite{Sankar} thus solving the delay problem in the MARC.  %One of implication of this paper: we solve the delay problem for general multi-source multi-relay channels as well.

Backward-decoding cannot support bidirectional communication in the DF  setting \cite{XieKumar}.  Inspired by \cite{Sankar} offset-encoding was applied in the two-way two-relay channel, where it was first discovered that the causality constraints can not always be simultaneously deactivated at all nodes \cite{Ponniah2008}. 

A parallel effort applying offset-encoding to CF schemes for multi-relay channels was proposed in \cite{Yassaee}, which recognized that regular decoding schemes correspond to layerings.  This work was studied in \cite{PonniahCompressForward2019} to show the mutual-information constraints are sufficient using the proof techniques here. 

Another independent line of inquiry revealed a relationship between CF and network coding \cite{AhlswedeCai2000}.  Noisy Network Coding (NNC) \cite{noisynetworkcoding} is a CF scheme that generalizes the network coding scheme in \cite{Avestimehr2011}.  It turns out that backward-decoding generalizes NNC \cite{Wu2013}\cite{HouKramer}.  The CF schemes in \cite{Yassaee}\cite{PonniahCompressForward2019} rely on regular coding; the long encoding delays and restrictions on bidirectional communication in joint backward-decoding DF-CF schemes \cite{Wu2014}\cite{Hou2016} can be avoided. 

The index-coding DF scheme we use was originally proposed in \cite{Xie2007} and simplified by Xiugang Wu in private correspondence with the authors. 

\section{Outline and Preliminaries}
\label{OutlineAndPreliminaries}
  We give a rough overview of the main results and proof, preparing for the rigor in Sections \ref{FlowDecomposition}, \ref{mainresult} and \ref{prooftheoremone}.  Let ${\cal N}=\{1,\ldots,|{\cal N}|\}$ denote the set of all nodes in the channel.  Assume all nodes are sources and each node is a destination for some subset of sources.  Let ${\bf y}_{\cal N}:=(y_{1},\ldots,y_{|{\cal N}|})$ and ${\bf x}_{\cal N}:=(x_{1},\ldots,x_{|{\cal N}|})$.  The input-output dynamics conform to the discrete memoryless channel:
\begin{align}
	\label{discretememorylesschannel}
	%\nonumber
	(\displaystyle\prod_{i\in {\cal N}}{\cal X}_{i},\hspace{1mm}p({\bf y}_{\cal N}|{\bf x}_{\cal N}),\displaystyle\prod_{i\in{\cal N}}{\cal Y}_{i}).
\end{align}

Let ${\bf f}(s)$ define the flow for each $s\in{\cal N}$ and let ${\bf F}:=\{{\bf f}(s):s\in{\cal N}\}$ be the flows for all nodes in the channel.  Fix some destination node $d\in{\cal N}$ rate-vector ${\bf R}=(R_{1},\ldots,R_{|{\cal N}|})$.  For any subset $S\subseteq{\cal N}$, let $R_{S}:=\sum_{s\in S}R_{s}$.  The mutual-information constraints implied by the one-relay channel are given by: 
\begin{align}
	\label{outline1}
	R_{S}<I(X_{F_{d}(S)};Y_{d}|X_{\tilde{F}_{d}(S)}),
\end{align}   
where $F_{d}(S)$ includes all the nodes upstream of node $d$, that encode the sources $S$, and $\tilde{F}_{d}(S)$ roughly speaking, includes all the nodes downstream of node $d$.  The constraint in (\ref{outline1}) applies for each $S\subseteq{\cal N}$.

 Let ${\bf L}_{d}$ be the layering at node $d$.  We show in Section \ref{FlowDecomposition}, that $({\bf F},{\bf L}_{d})$ corresponds to a well-defined encoding/decoding scheme (see Lemma \ref{splitting}); the messages decoded in each block of channel are encoded in the received sequences and the side information assumed in every typicality check is known or already decoded.  These consistency conditions are best expressed using so-called  ``virtual'' flows $\{{\bf v}(s):s\in{\cal N}\}$ ``seen'' by node $d$, from the actual flows in ${\bf F}$.  Virtual flows have some useful properties (see Lemma \ref{vssuffices}).  
 
A rate-vector is only achievable if the corresponding encoding/decoding scheme is causal (i.e., relays only forward messages they have already decoded).  These causality constraints correspond to the following set of inequalities for every source $s\in{\cal N}$ decoded by node $d$:
\begin{align}
	\label{outline2}
	\text{\sc layer}(v(s))<k_{v(s),d},
\end{align}
where $\text{\sc layer}(v(s))$ is the layer assigned to the virtual source $v(s)$ by ${\bf L}_{d}$ and $k_{v(s),d}$ is the encoding delay; the number of blocks that elapse between the virtual source $v(s)$ encoding a message from the actual source $s$, and node $d$ encoding the same message.  The constraint in (\ref{outline2}) applies to every source $s$ decoded by node $d$.   Both sets of constraints (\ref{outline1}) and (\ref{outline2}) are necessary for DF schemes.

We focus on two types of flow consistent with index-coding: hierarchical flow, where the routes are tree-structured, and all-cast flow, where each route covers all nodes.  The main result in Theorem \ref{theoremone} is that for an arbitrary ${\bf F}$ of either type, and any rate-vector ${\bf R}$ satisfying (\ref{outline1}), there exists an equivalent ${\bf F}^{\prime}$ and a layering ${\bf L}_{d}$ such that the encoding/decoding scheme $({\bf F}^{\prime}, {\bf L}_{d})$ achieves ${\bf R}$ and satisfies (\ref{outline2}).  Equivalent flows generate the same mutual information constraints in (\ref{outline1}).  Theorem \ref{theoremone}  shows that (\ref{outline1}) and (\ref{outline2}) are sufficient conditions for any rate-vector in the DF region.  However, there are infinitely many flows and layerings in a channel of fixed size, which creates ambiguity as to whether   (\ref{outline2}) is computable.

To prove Theorem \ref{theoremone} we pick an arbitrary rate-vector ${\bf R}$ that satisfies (\ref{outline1}) and an arbitrary ${\bf L}_{d}$.  If $({\bf F}, {\bf L}_{d})$ does not achieve ${\bf R}$, we define the following ``shift'' operation: 
\begin{align}
{\bf L}^{\prime}_{d}&=\text{\sc shift}({\bf L}_{d},S),
\end{align}
where $S$ is a selected subset of sources decoded by node $d$.  Lemma \ref{induction} shows that the achievable region generated by $({\bf F}, {\bf L}^{\prime}_{d})$ is closer to ${\bf R}$ than $({\bf F}, {\bf L}_{d})$.  The proof of Lemma \ref{induction} relies on Lemmas \ref{disjoint}, \ref{remain} and \ref{join}.

Next, we create a sequence of layerings $\{{\bf L}_{d,n}:n\in\mathbb{N}\}$, where ${\bf L}_{d,n+1}=\text{\sc shift}({\bf L}_{d,n}, S_{n})$ and $\{S_{n}:n\in\mathbb{N}\}$ is a selected sequence of subsets of ${\cal N}$.  Lemma \ref{grandefinale} proves there is some $n^{*}\in\mathbb{N}$, such that $({\bf F},{\bf L}_{d,n^{*}})$ achieves ${\bf R}$.  The proof of Lemma \ref{grandefinale} uses Lemma \ref{induction}.  

Finally, we construct an equivalent flow ${\bf F}^{\prime}$ and layering ${\bf L}_{d}$ that achieves ${\bf R}$ and satisfies (\ref{outline2}).  Lemmas \ref{fine} and \ref{normalize} show that $({\bf F}^{\prime},{\bf L}_{d})$ exists which completes the proof.

The proofs of each lemma are organized into claims and sub-claims, but   occasionally, the proof of one lemma references the claims of another.  Examples in Appendices \ref{Example}, \ref{appendix2}, and \ref{appendix3} explore the shift operation.

The following definition of typicality is used in the paper.  Let $X_{{\cal N}}:=\{X_{i}:i\in{\cal N}\}$ denote a finite collection of discrete random variables  with a fixed joint distribution $p(x_{{\cal N}})$ for some $x_{{\cal N}}:=\{x_{i}\in{\cal X}_{i}:i\in{\cal N}\}$.  Similarly, let ${\bf x}_{i}:=\{x^{(m)}_{i}\in{\cal X}_{i}:1\leq m\leq n\}$ denote an $n$-length vector of ${\cal X}_{i}$ and let ${\bf x}_{{\cal N}}:=\{{\bf x}_{i}:i\in{\cal N}\}$.  The set of typical $n$-sequences is given by: 
\begin{align}
	\nonumber
	&\hspace{-1mm}T^{(n)}_{\epsilon}(X_{{\cal N}}):=\\
	\nonumber
	&\hspace{7mm}\bigg\{{\bf x}_{{\cal N}}:\left|-\frac{1}{n}\log\text{Prob}({\bf x}_{S})-H(X_{S})\right|<\epsilon, \forall S\subseteq{\cal N}\bigg\},
\end{align}
where $\text{Prob}({\bf x}_{S}):=\prod^{n}_{m=1}p(x^{(m)}_{S})$.

%Let ${\bf x}_{i}:=(x_{1,i},x_{2,i},\ldots,x_{n,i})$ denote an $n$-length vector where $x^{m}_{i}\in{\cal X}_{i}$ for all $1\leq m\leq n$, 

%For any subset $S\subset{\cal N}$  

%Let $(Z_{1},Z_{2},\ldots,Z_{|{\cal N}|})$ denote a finite collection of discrete random variables with some fixed joint distribution $p(z_{1},z_{2},\ldots,z_{|{\cal N}|})$ for $(z_{1},z_{2},\ldots,z_{|{\cal N}|})\in{\cal Z}_{1}\times{\cal Z}_{2}\times\cdots\times{\cal Z}_{|{\cal N}|}$.  The set of typical $n$-sequences is given by:
%\begin{align}
%	\nonumber
%	&T^{(n)}_{\epsilon}(Z_{1},Z_{2},\ldots,Z_{|{\cal N}|})\\
%	\nonumber
%	&\hspace{2mm}:=\bigg\{({\bf z}_{1},{\bf z}_{2},\ldots,{\bf z}_{|{\cal N}|}):\left|-\frac{1}{n}\log\text{Prob}({\bf s})-H(S)\right|<\epsilon,\\
%	\nonumber
%	&\hspace{43mm}\forall S\subseteq\{Z_{1},Z_{2},\ldots,Z_{|{\cal N}|}\}\bigg\},
%\end{align}
%where each ${\bf z}_{i}=(z_{i,1},z_{i,2},\ldots,z_{i,n})$ is an $n$-vector and  $i=1,\ldots,|{\cal N}|$.  Define ${\bf s}=({\bf z}_{i_{1}},{\bf z}_{i_{2}},\ldots,{\bf z}_{i_{l}})$ if $S=(Z_{i_{1}},Z_{i_{2}},\ldots,Z_{i_{l}})$, where $\text{Prob}({\bf s})=\text{Prob}({\bf z}_{i_{1}},{\bf z}_{i_{2}},\ldots,{\bf z}_{i_{l}})=\prod^{n}_{k=1}p(z_{i_{1},k},z_{i_{2},k},\ldots,z_{i_{l},k})$.

 

%The following definition of weak typicality will suffice.  Let $(Z_{1},Z_{2},\ldots,Z_{|{\cal N}|})$ denote a finite collection of discrete random variables with some fixed joint distribution $p(z_{1},z_{2},\ldots,z_{|{\cal N}|})$ for $(z_{1},z_{2},\ldots,z_{|{\cal N}|})\in{\cal Z}_{1}\times{\cal Z}_{2}\times\cdots\times{\cal Z}_{|{\cal N}|}$.  The set of typical $n$-sequences $T^{(n)}_{\epsilon}$ is given by:
%\begin{align}
%	\nonumber
%	&T^{(n)}_{\epsilon}(Z_{1},Z_{2},\ldots,Z_{|{\cal N}|})\\
%	\nonumber
%	&\hspace{6mm}:=\bigg\{({\bf z}_{1},{\bf z}_{2},\ldots,{\bf z}_{|{\cal N}|}):\left|-\frac{1}{n}\log\text{Prob}({\bf s})-H(S)\right|<\epsilon,\\
%	\nonumber
%	&\hspace{47mm}\forall S\subseteq\{Z_{1},Z_{2},\ldots,Z_{|{\cal N}|}\}\bigg\},
%\end{align}
%where each ${\bf z}_{i}=(z_{i,1},z_{i,2},\ldots,z_{i,n})$ is an $n$-vector and  $i=1,\ldots,|{\cal N}|$.  The parameter ${\bf s}$ is defined as follows.  If $S=(Z_{i_{1}},Z_{i_{2}},\ldots,Z_{i_{l}})$, then ${\bf s}=({\bf z}_{i_{1}},{\bf z}_{i_{2}},\ldots,{\bf z}_{i_{l}})$ and 
%\begin{align}
%	\nonumber
%	\text{Prob}({\bf s})&=\text{Prob}({\bf z}_{i_{1}},{\bf z}_{i_{2}},\ldots,{\bf z}_{i_{l}})\\
%	\nonumber
%	&=\prod^{n}_{k=1}p(z_{i_{1},k},z_{i_{2},k},\ldots,z_{i_{l},k}).	
%\end{align}




%%The one-relay channel was proposed in [CITE].  CF and DF schemes for the one-relay channel first appear in [CITE].  In its original form, the DF scheme combines super-position coding with binning and list decoding, and allows the auxiliary and input random variables to have different cardinalities.  The original DF scheme is simplified and streamlined for multi-relay channels in [CITE] and [CITE].   In [CITE], the original binning and list decoding DF strategy is replaced with a simpler joint typicality decoding scheme, first proposed for the Multiple-Access Channel with Generalized Feedback (MAC-GF) in [CITE].  This scheme, called ``sliding-window decoding'' is a precursor of regular decoding.  A different scheme from sliding-window decoding called ``backward-decoding'', first proposed for the Multiple-Access Channel with Cribbing Encoders (MAC-CE) in [CITE], is shown to achieve the same rate as sliding-window decoding for the multi-relay channel in [CITE].  The authors in [CITE] and [CITE] did not apply sliding-window decoding and backward decoding respectively to relay channels.          

%%Backward-decoding is the more powerful scheme in general multi-source multi-relay channels [CITE], but requires much longer encoding delays.  To circumvent this delay problem, ``offset encoding'' is proposed for the multiple-access relay channel (MARC) in [CITE].  A family of offset encoding schemes is shown to collectively achieve the same rate region as backward decoding in the MARC, while preserving the short delays that are desirable in sliding-window decoding.  

%%DF schemes based on backward-decoding exclude channels with  bidirectional communication, the two-way two-relay channel (TWTRC) being the simplest such channel [CITE].  Inspired by [CITE], offset-encoding is applied to the (TWTRC), with the intent of achieving the same  hypothetical rate region as backward-decoding without actually using backward-decoding.  The attempt fails because one particular combination of offset encoding schemes is impossible to make causal at both relays simultaneously.  The discoveries in [CITE] and [CITE], also motivate a framework for extending CF schemes to multi-relay channels in [CITE], which introduces the concept of layering to describe different offset-decoding schemes.  This framework is expanded in [CITE] to include the \text{\sc shift} operator.

%%Another line of inquiry is based on network coding [CITE], which is a capacity achieving scheme in single-source multi-cast graphical networks [CITE].  For  Gaussian relay channels of fixed size, there is a corresponding graph network and network coding scheme that lies within a bounded gap of the Gaussian channel capacity with respect to all channel gains [CITE].  An expanded CF version of this scheme called ``Noisy Network Coding'' is developed for general multi-relay channels in [CITE].  The rates achieved in [CITE] and [CITE] are the same even though the underlying schemes are completely different.  The approach in [CITE] uses regular coding and is thus more general with shorter delays than [CITE].  However, some  important concepts appearing here and in [CITE] are required for the proof in [CITE] to be rigorous.  Noisy Network Coding (NNC) is a variation of backward decoding in the CF setting [CITE].  The backward decoding CF scheme in [CITE] is further refined in [CITE].  Joint CF/DF schemes based on backward decoding appear in [CITE and [CITE].  The restrictions on backward-decoding apply to these schemes.

%%A third line of inquiry arises out of the insight that random binning is a form of network coding, in which source messages are randomly binned, and nodes forward the bin indices that contain the relevant messages [CITE].  Nodes use their prior history of decoded messages as side information to decode other messages in the index.  In each block, relays decode the messages in the indices and re-encode bundles of previously decoded messages into new indices, features indicative of DF regular coding.  DFIC simplifies this scheme by replacing random binning with deterministic binning, a contribution made by Xiugang Wu in private correspondence with the authors.

%%These lines of inquiry converge in flow decomposition, which characterizes DFIC schemes at individual nodes and harmonizes the achievability proofs for both DF and CF regular-coding schemes.  Flow decomposition generalizes offset encoding by introducing flows and layerings, two separate and independent structures to deal with encoding and decoding respectively, and to enforce causality simultaneously at all nodes in the channel.
%Although the capacity of this channel remains unknown, two different schemes are of interest: decode-forward (DF), in which the relay decodes and forwards source messages to the destination and compress-forward (CF), in which the relay compresses its channel observations without decoding any messages, and forwards these compressions to the destination \cite{GamalCover}.  Neither scheme is universally better than the other.

%The focus of this paper is on decode-forward index-coding (DFIC), a variant of decode-forward that has some appealing qualities in multi-source, multi-relay, multi-destination channels.  It is the simplest non-trivial DF scheme that captures the notion of side-information in general networks.  Initially proposed and studied in a series of papers by Xie, DFIC was subsequently refined by Xiugang Wu and privately explained to the authors. 
 
%Relays contribute to the achievable rate vector by forwarding messages over successive blocks of channel uses.  Simultaneously, each relay  decodes messages using any available side information; sequences it receives during previous blocks of channel uses in which other relays transmit relevant messages.  Since the relays can only forward messages they have already decoded, this causal requirement creates a certain tension in which each relay has an ``incentive'' to acquire more side information and improve their contributions.  For instance, each relay in the two-way two-relay channel benefits if the other relay decodes and forwards their messages first.  The rate region depends on all the ways of resolving this tension.  A simple characterization of the rate region that extends to general networks of arbitrary size remains elusive.

%The difficulty of characterizing rate regions is related to a fundamental problem in network information theory, that capacity regions are not always unambiguously computable.  A region is computable, by definition, if a Turing machine can determine whether the region contains a specified rate vector in finite time.  Some necessary conditions for computability have already been studied in the literature: auxiliary time-sharing random variables must have bounded cardinality and the number of letters in any multi-letter description must be bounded.  

%There are infinitely many ways of resolving the tensions described above in the DF setting, even with a bounded number of nodes, because there are infinitely many ways that relays can encode and decode information.  Not all of these ways are advantageous but identifying the ones that are, from a sea of possibilities, is difficult.  This paper proposes the framework of flow decomposition to make the problem more manageable.

%DF and CF schemes either use regular-coding, in which relays decode messages in every block of channel uses, or backward-decoding, in which relays decode the messages sent over many blocks of channel uses after the end of the last block, and in reverse order.  In any given channel, there could be many different regular coding schemes that achieve different rate regions, but each of these rate regions is strictly smaller than that achieved by backward-decoding.  It has been suspected that regular coding schemes collectively achieve the same region as backward-decoding, a suspicion that will be partially confirmed in this paper.  Backward-decoding suffers from much longer encoding delays than regular-coding, and in the DF setting, backward-decoding is confined to channels with ``hierarchical'' information flow.  Regular-coding, on the other hand, has no such restrictions.

%DFIC is a class of regular-coding coding schemes, so each scheme in the class achieves a possibly unique rate region.  Flow decomposition defines a DFIC scheme at a particular relay using two structures: a \textit{flow} set, which determines the node sequences (or paths) that forward source messages to destination nodes and the corresponding encoding delays along each hop, and \textit{layerings}, which determine the source messages decoded by the given relay.

%The framework of flow decomposition addresses the question of whether a desired rate-vector can be achieved by some causal DFIC scheme.  The solution appears in two stages, the first here, and the second in following work.  The first stage fixes a particular relay in the general multi-source, multi-relay, multi-destination channel.  An outer-bound on the DFIC rate region is shown to be tight at this relay.  The proof involves a novel shifting technique.  The second stage explores whether or not the DFIC outer-bound is tight at all relays simultaneously.  Two cases are considered: multi-cast channels with hierarchical flow and all-cast channels with arbitrary flow.  The DFIC outer-bound remains tight in the first case, and the solution is not only computable but also ``order'' optimal in terms of its computational complexity.  The solution in the second case has higher complexity, in part because the DFIC outer-bound is not tight.

%The situation in the CF setting is simpler because the relays do not decode messages and are thus not subject to the same causal restrictions as DF schemes.  Nevertheless, the idea of layering retains the same interpretation if source messages are replaced with ``compression code-words''.  The shifting technique in this paper also extends to the CF setting.  A variation of layering for CF schemes was originally discovered by Yassaee and Aref.


 



%\begin{figure*}[!t]
%       \center{\includegraphics[width=\textwidth]
%        {./taxonomy}}
%       \caption{A taxonomic classification (left) for existing coding schemes in the literature.  Regular-order schemes subsume reverse-order schemes  (right).  This paper focuses on the class of single-letter decode-forward index-coding schemes (red).  Compress-forward, decode-forward, index coding, and super-position coding schemes are labeled CF, DF, IX, and SP respectively.  Basic sub-classes have dual variations.}
%        \label{polytope}
% \end{figure*}

%The next taxonomic level introduces two sub-classes: reverse-order schemes, in which the destination decodes each message after the entire message sequence is sent, and regular-order schemes, in which the destination decodes each message without waiting for the full message sequence.  The first examples of reverse-order and regular-order schemes, called \textit{backward decoding} and \textit{sliding-window decoding} respectively, were proposed for cooperative multiple-access channels and relay channels.  Encoding/decoding delays, which define the number of channel uses to encode/decode each message, scale differently in each sub-class.  Reverse-order schemes have \textit{long} decoding delays; the scaling factor increases in the number of channel uses.  Regular-order schemes have \textit{short} decoding delays; the factor is constant in the channel usage.  Encoding and decoding delays are related through causality; nodes can only encode messages they have already decoded.  

%The dynamics of relay channels include the dynamics of cooperative multiple-access channels, which include the dynamics of multiple-access channels, thus recursively inducing a taxonomy of schemes.  Decode-forward schemes further split into two sub-classes: index-coding schemes with independent input distributions, and superposition coding schemes with correlated input distributions.  The schemes in the second class augment those in the first with auxiliary random variables.  

%The capacity regions of general discrete-memoryless channel (DMC) networks  depend on solutions to several class-specific sub-problems.  One problem, identified by Shannon, is a computable description of multi-letter-deterministic-coding schemes.  Another, identified by Cover, is the channel-induced boundary between the decode-forward and compress-forward classes.  A third, identified by Slepian, is a computable description of correlated-input schemes.  There has been progress on this front.  Classical results establish fundamental limits on the kind of coordination that can occur between distributed inputs; common messages require common parts and each part requires only bounded cardinality.

%This paper explores the complexity of regular-order decode-forward schemes for general DMC networks.  The core problem is that reverse-order decode-forward schemes are intrinsically confined to hierarchical patterns of information flow, which prevents bidirectional communication.  Although reverse-order compress-forward schemes avoid this limitation, combined compress-forward/decode-forward schemes must share the same parent class and jointly inherit any restrictions on a child-class.  Regular-order schemes avoid these artificial constraints, but have no known computable description.  

%We propose the framework of flow decomposition to describe regular-order decode-forward index-coding schemes.  The framework consists of two components: \textit{flows}, which describe encoding schemes at all nodes simultaneously and \textit{layered partitions}, which describe decoding schemes at particular nodes.  Flows define the sequence of hops made by each message and the encoding delays along each hop.  Every flow generates a class-specific cut-set outer-bound on the achievable region, independent of the encoding delays.  The outer-bound is computable with complexity $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$ where ${\cal S}\subseteq{\cal N}$ is the set of source nodes and ${\cal N}$ is the set of all nodes; each source subset $S\subseteq{\cal S}$ generates a different cut at a given node.

%The class-specific cut-set outer-bounds for decode-forward schemes do not include the causal requirement that nodes only encode messages they have already decoded; encoding delays at each node must exceed the decoding delays.  For a network of fixed size, there are infinitely many combinations of encoding delays and layered partitions (decoding schemes), so the actual achievable region is not obviously computable.  

%This problem is resolved in two stages.  The first, addressed here, partially relaxes the assumption of causality.  For an arbitrary flow with arbitrary encoding delays, we fix any rate vector in the class-specific cut-set outer-bound and use a \textit{shift operator} to generate a sequence of layered partitions, converging in $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$ time, to a layered partition that achieves the desired rate vector.

%The second stage fully assumes causality and splits into two extremal cases: multi-cast channels with hierarchical flow and all-cast channels with arbitrary flow.  Reverse-order decode-forward schemes match the class-specific outer-bounds under hierarchical flow constraints.  Regular-order decode-forward schemes, though free of any flow constraints, are \textit{individually} worse than reverse-order schemes.  It has been suspected that the former are \textit{collectively} equivalent to the latter.  This hypothesis is confirmed in the second stage; given any desired rate-vector in the class-specific outer-bounds for channels with hierarchical flow, a corresponding causal regular-order decode-forward scheme in the class is found in $\text{P}(|{\cal N}|)\text{EXP}(|{\cal S}|)$ time.  The outer-bounds are loose for all-cast channels with arbitrary flow, but the achievable region is still computable; it is possible to decide in $\text{NEXP}(|{\cal N}|)$ time if a desired rate-vector is achievable by any scheme in the class.  These results extend directly to the class of super-position-coding schemes, which differ only in the existence of auxiliary random variables.  Arbitrary flow in multi-cast channels is a combination of these two extremes.  

%The preceding discussion applies to compress-forward schemes without any special cases.  As before, regular-order compress-forward schemes are individually worse than their reverse-order counterparts, which match the class-specific cut-set outer-bounds.  A companion paper shows that regular-order compress-forward schemes are collectively equivalent to reverse-order schemes using concepts developed in this paper and independently by Yassaee and Aref.  In particular, compress-forward schemes correspond to layered partitions equipped with a shift operator.  Decode-forward and compress-forward schemes thus share an underlying structure that unifies their individual descriptions.  

%By making reverse-order schemes redundant, these results simplify the taxonomy of coding schemes and eliminate the need for long encoding delays.  While the dual class and the class of correlated-input schemes depend on ``physical layer'' properties like the channel statistics and the source distributions, the class of compress-forward and decode-forward schemes depend on ``network  layer'' properties like the number of nodes, the number of sources, the network flow, and causally induced tensions in the flow structure.  



       


    

  

%The capacity of this channel is not fully understood, but two fundamentally different schemes are of interest: decode-forward, in which the relay decodes the source message then forwards the decoded message to the destination, and compress-forward, in which the relay compresses its observations of the channel without decoding the message, then forwards its compressions to the destination \cite{GamalCover}.  Neither scheme is universally better than the other.  The focus of this paper is on decode-forward schemes and a companion paper addresses compress-forward schemes \cite{compdecomp}.

%Despite the ambiguity surrounding the relay channel, there has been some progress, starting with \cite{KramerGastpar}, in developing cut-set extensions of the compress-forward and decode-forward rates in the one-relay channel to general multi-source, multi-relay, multi-cast channels.  Cut-set extensions imply a ``converse-of-sorts" in that the regions they define cannot be enlarged with compress-forward and decode-forward schemes; their optimality is contingent on the optimality of decode-forward and compress-forward in the one-relay channel.  Other works in this endeavor include \cite{Yassaee}, \cite{noisynetworkcoding}, \cite{WuXie}, and \cite{HouKramer} on the compress-forward side and \cite{XieMultiLevel} and \cite{XieKumar} on the decode-forward side.
  
%Most of these works (with the notable exception of \cite{Yassaee}) rely on ``backward decoding'', a technique originally proposed for cooperative multiple-access channels \cite{willems}.  Backward-decoding requires exponentially-increasing encoding delays in the network size.  Decode-forward schemes based on backward-decoding only support hierarchical patterns of information flow, which excludes bidirectional communication \cite{XieKumar}.

%\textit{Regular} decoding schemes impose no such restrictions but fail to \textit{individually} achieve rate regions with cut-set interpretations.  It has long been suspected that regular decoding schemes \textit{collectively} achieve regional cut-set extensions of the one-relay decode-forward and compress-forward rates.  The first result of this nature was proved in the decode-forward setting for the multiple-access relay channel \cite{Sankar}, by geometrically piecing together achievable regions from three different ``offset-encoding'' schemes.  A second result \cite{Yassaee} in the compress-forward setting for multi-relay channels, includes the key insight that regular decoding schemes correspond to ordered partitions of relay nodes.  

%This paper shows that regular decoding schemes collectively achieve the regional cut-set extension of the one-relay decode-forward rate to multi-source, multi-cast channels, where messages spread through the channel until source-specific subsets of nodes are covered.  The result is based on the framework of flow decomposition, which describes encoding schemes with \textit{flows} and regular decoding schemes with \textit{layered partitions} of the relay nodes.  Layered partitions are similar to ordered partitions and share the same compress-forward interpretation \cite{compdecomp}.

%Flow decomposition reveals a fundamental duality between regular compress-forward and decode-forward schemes with broader implications for combinatorial optimization.  The proof, which mirrors \cite{compdecomp} with the addition of \textit{flow}, constructs a shifted sequence of layered partitions that converges to a target rate vector.  The number of shifts required to reach the target is at most linear in the network size.  As a side benefit, this result also provides closed-form solutions to general variations of the index coding problem \cite{indexcoding}.  The advantages of regular decoding, which include linear encoding delays and unrestricted patterns of flow, carry over without the drawbacks of backward decoding.





%\cite{PonniahArxiv}
%\cite{noisynetworkcoding}
%\cite{Yassaee}
%\cite{KramerGastpar}
%\cite{GamalCover}
%\cite{HouKramer}
%\cite{Sankar}
%\cite{XieKumar}
%\cite{WuXie}
%\cite{indexcoding}

%\restoregeometry 


==> flowdecomp 2/join.tex <==
\begin{lemma}
\label{join}
	For every $S\subseteq{\cal S}(d)$ and $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$, $A_{l-1}(S\cap U)\subseteq A^{\prime}_{l}(S\cap U)$
\end{lemma}
\begin{proof}
First, we introduce some preliminary claims.

\hspace{-3.5mm}{\bf Claim \ref{join}.1} \textit{Suppose $i\in{\bf v}(s)$ for some $s\in U$. If $v^{\prime}(s)=v(s)$ then $i\in{\bf v}^{\prime}(s)$.}

\begin{proof}
Fix $i\in{\bf v}(s)$ and consider the following inequalities:
\begin{align}
\nonumber
	&\hspace{-2mm}\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)\\
	\label{shiftedcomplete1}
	&\hspace{15mm}=\text{\sc layer}^{\prime}(v(s))-\text{\sc layer}^{\prime}(i),\\
	\label{shiftedcomplete2}
	&\hspace{15mm}=(\text{\sc layer}(v(s))+1)-(\text{\sc layer}(i)+1),\\
	\nonumber
	&\hspace{15mm}=\text{\sc layer}(v(s))-\text{\sc layer}(i),\\
	\label{shiftedcomplete4}
	&\hspace{15mm}=k_{v(s),i},\\
	\label{shiftedcomplete5}
	&\hspace{15mm}=k_{v^{\prime}(s),i},
\end{align}
where (\ref{shiftedcomplete1}) follows because $v^{\prime}(s)=v(s)$ is the premise of Claim \ref{join}.1, (\ref{shiftedcomplete2}) follows from (\ref{shift2}) and because $s\in U$ and $i\in{\bf v}(s)$, (\ref{shiftedcomplete4}) follows from (V5) and because $i\in{\bf v}(s)$, and (\ref{shiftedcomplete5}) follows because $v^{\prime}(s)=v(s)$ is the premise of Claim \ref{join}.1.  It follows from (V5) and (\ref{shiftedcomplete5}) that $i\in{\bf v}^{\prime}(s)$.	
\end{proof} 

\hspace{-3.5mm}{\bf Claim \ref{join}.2} \textit{Suppose $i\in{\bf v}(s)$ for some $s\in U$. If $v^{\prime}(s)\neq v(s)$ then $i\in{\bf v}^{\prime}(s)$.}

\begin{proof}
First we prove some preliminary sub-claims.

\hspace{-3.5mm}{\bf Claim \ref{join}.2.a} \textit{If $s\in U$ and $v^{\prime}(s)\neq v(s)$ then $v^{\prime}(s)\in{\bf f}(s,v(s))$.}
\begin{proof}
The proof is by contradiction.  Suppose $v^{\prime}(s)\in{\bf f}(v(s),d)$.  It is convenient to consider $\text{\sc layer}^{\prime}(v^{\prime}(s))>\text{\sc layer}(v^{\prime}(s))$ and $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$ separately.  Suppose $\text{\sc layer}^{\prime}(v^{\prime}(s))>\text{\sc layer}(v^{\prime}(s))$:
\begin{align}
	\nonumber
	&\hspace{-2mm}k_{v(s),v^{\prime}(s)}\\
	\label{shiftedcomplete6}	
	&\hspace{5mm}\geq\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s)),\\
	\label{shiftedcomplete7}
	&\hspace{5mm}=(\text{\sc layer}^{\prime}(v(s))-1)-(\text{\sc layer}^{\prime}(v^{\prime}(s))-1),\\
	\label{shiftedcomplete8}
	&\hspace{5mm}=\text{\sc layer}^{\prime}(v(s))-\text{\sc layer}^{\prime}(v^{\prime}(s)),
\end{align}
where (\ref{shiftedcomplete6}) follows from (\ref{firstIndexCodingShiftedComplete2}) and because $v^{\prime}(s)\in{\bf f}(v(s),d)$, (\ref{shiftedcomplete7}) follows from (\ref{shift2}), $s\in U$, and the assumption $\text{\sc layer}^{\prime}(v^{\prime}(s))>\text{\sc layer}(v^{\prime}(s))$.  Since $v(s)\in{\bf f}(s,v^{\prime}(s))$, (\ref{shiftedcomplete8}) contradicts (\ref{secondIndexShiftedComplete}).  Now suppose $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$: 
\begin{align}
	\label{shiftedcomplete9}
	k_{v(s),v^{\prime}(s)}&\geq\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s)),\\
	\label{shiftedcomplete10}
	&>\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s)),\\
	\label{shiftedcomplete11}
	&=(\text{\sc layer}^{\prime}(v(s))-1)-\text{\sc layer}^{\prime}(v^{\prime}(s)),
\end{align}
where (\ref{shiftedcomplete9}) follows from (\ref{firstIndexCodingShiftedComplete2}). Since $\text{\sc layer}(v^{\prime}(s))=\text{\sc layer}^{\prime}(v^{\prime}(s))$, it follows from (\ref{shift2}) that $v^{\prime}(s)\notin{\bf v}(j)$ for any $j\in U$.  Therefore $v^{\prime}(s)\notin{\bf v}(s)$ since $s\in U$ is the premise of Claim \ref{join}.2.a.  From (V5), equality in (\ref{shiftedcomplete9}) occurs only if $v^{\prime}(s)\in{\bf v}(s)$.  Since $v^{\prime}(s)\notin{\bf v}(s)$, (\ref{shiftedcomplete10}) follows from (\ref{shiftedcomplete9}).  Finally, (\ref{shiftedcomplete11}) follows because (\ref{shift2}) implies $\text{\sc layer}^{\prime}(v(s))=\text{\sc layer}(v(s))+1$ since $s\in U$.  Consider the following inequalities:  
\begin{align}
	\label{shiftedcomplete12}
	\text{\sc layer}^{\prime}(v(s))-\text{\sc layer}^{\prime}(v^{\prime}(s))&<k_{v(s),v^{\prime}(s)}+1,\\
	\label{shiftedcomplete13}
	&\leq k_{v(s),v^{\prime}(s)},
\end{align}
where (\ref{shiftedcomplete12}) follows from (\ref{shiftedcomplete11}), and (\ref{shiftedcomplete13}) follows because the encoding delays are integer-valued.  Since $v(s)\in{\bf f}(s,v^{\prime}(s))$, (\ref{shiftedcomplete13}) contradicts (\ref{secondIndexShiftedComplete}).  It follows from (\ref{secondIndexShiftedComplete}), (\ref{shiftedcomplete8}), and (\ref{shiftedcomplete13}) that $v^{\prime}(s)\in{\bf f}(s,v(s))$.
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{join}.2.b}. \textit{If $s\in U$ and $v^{\prime}(s)\neq v(s)$ then $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$.} 

\begin{proof}
	The proof is by contradiction.  Suppose $\text{\sc layer}^{\prime}(v^{\prime}(s))\neq\text{\sc layer}(v^{\prime}(s))$.  Since (\ref{shift2}) implies $\text{\sc layer}(v^{\prime}(s))\leq\text{\sc layer}^{\prime}(v^{\prime}(s))\leq\text{\sc layer}(v^{\prime}(s))+1$, it follows that:
	\begin{align}
		\label{claim2b1}
		\text{\sc layer}^{\prime}(v^{\prime}(s))&=\text{\sc layer}(v^{\prime}(s))+1.
	\end{align}
	Consider the following inequalities:
	\begin{align}
	\label{claim2b2}
	k_{v^{\prime}(s),v(s)}&<\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(v(s)),\\
	\label{claim2b3}
	&=(\text{\sc layer}^{\prime}(v^{\prime}(s))-1)-\text{\sc layer}(v(s)),\\
	\nonumber
	&=(\text{\sc layer}^{\prime}(v^{\prime}(s))-1)\\
	\label{claim2b4}
	&\hspace{27mm}-(\text{\sc layer}^{\prime}(v(s))-1),\\
	\label{claim2b5}
	&=\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s)),
\end{align}
where (\ref{claim2b2}) follows from (\ref{secondIndexShiftedComplete2}) and because $v^{\prime}(s)\in{\bf f}(s,v(s))$, (\ref{claim2b3}) follows from (\ref{claim2b1}), and (\ref{claim2b4}) follows from (\ref{shift2}) and because $s\in U$ is the premise of Claim \ref{join}.2.  Since Claim \ref{join}.1 implies $v^{\prime}(s)\in{\bf f}(s,v(s))$, it follows that $v(s)\in{\bf f}(v^{\prime}(s),d)$.  Therefore (\ref{claim2b5}) contradicts (\ref{firstIndexCodingShiftedComplete}).
\end{proof}

\hspace{-3.5mm}{\bf Claim \ref{join}.2.c}. \textit{If $s\in U$ and $v^{\prime}(s)\neq v(s)$ then $\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s))=k_{v^{\prime}(s),v(s)}$.}   

\begin{proof}
Consider the following inequalities:
\begin{align}
	\label{shiftedcomplete14}
	k_{v^{\prime}(s),v(s)}&<\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(v(s)),\\
	\label{preshiftedcomplete15}
	&=\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}(v(s)),\\
	\label{shiftedcomplete15}
	&=\text{\sc layer}^{\prime}(v^{\prime}(s))-(\text{\sc layer}^{\prime}(v(s))-1),
\end{align}
where (\ref{shiftedcomplete14}) follows from (\ref{secondIndexShiftedComplete2}) and because $v^{\prime}(s)\in{\bf f}(s,v(s))$, (\ref{preshiftedcomplete15}) follows from Claim \ref{join}.2.b, and (\ref{shiftedcomplete15}) follows from (\ref{shift2}) since $s\in U$.  Consider the following inequalities:
\begin{align}
\label{shiftedcomplete16}
\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s))&>k_{v^{\prime}(s),v(s)}-1,\\
\label{shiftedcomplete17}
&\geq k_{v^{\prime}(s),v(s)},
\end{align}
where (\ref{shiftedcomplete16}) follows from (\ref{shiftedcomplete15}), (\ref{shiftedcomplete17}) follows from (\ref{shiftedcomplete16}) and because the encoding delays are integer-valued.  Since Claim \ref{join}.2.a implies $v^{\prime}(s)\in{\bf f}(s,v(s))$, it follows that $v(s)\in{\bf f}(v^{\prime}(s),d)$.  Invoking (\ref{firstIndexCodingShiftedComplete}) and (\ref{shiftedcomplete17}) together gives: 
\begin{align}
\label{shiftedcomplete18}
\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s))=k_{v^{\prime}(s),v(s)},
\end{align}
which completes the proof of Claim \ref{join}.2.c.
\end{proof}
To complete the proof of Claim \ref{join}.2, fix $i\in{\bf v}(s)$ for some $s\in U$ and  consider the following inequalities:
\begin{align}
	\nonumber
	&\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)\\
	\nonumber
	&=\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s))\\
	\label{preshiftedcomplete20}
	&\hspace{30mm}+\text{\sc layer}^{\prime}(v(s))-\text{\sc layer}^{\prime}(i),\\
	\nonumber
	&=\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s))\\
	\label{shiftedcomplete20}
	&\hspace{14mm}+(\text{\sc layer}(v(s))-1)-(\text{\sc layer}(i)-1),\\
	\nonumber
	&=(\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(v(s)))\\
	\label{shiftedcomplete21}
	&\hspace{29mm}+(\text{\sc layer}(v(s))-\text{\sc layer}(i)),\\
	\label{shiftedjoin1}
	&=k_{v^{\prime}(s),v(s)}+(\text{\sc layer}(v(s))-\text{\sc layer}(i))\\
	\label{shiftedjoin2}
	&=k_{v^{\prime}(s),v(s)}+k_{v(s),i},\\
	\label{shiftedcomplete23}
	&=k_{v^{\prime}(s),i},
\end{align}
where (\ref{preshiftedcomplete20}) follows by adding and subtracting $\text{\sc layer}^{\prime}(v(^{\prime}(s))$ from the left-hand side of the equation, (\ref{shiftedcomplete20}) follows from (\ref{shift2}) since $s\in U$ and $i\in{\bf v}(s)$, (\ref{shiftedcomplete21}) follows from rearranging (\ref{shiftedcomplete20}), (\ref{shiftedjoin1}) follows from Claim \ref{join}.2.c, and (\ref{shiftedjoin2}) follows from (V5) since $i\in{\bf v}(s)$.  It follows from (\ref{shiftedcomplete23}) and (V5) that $i\in{\bf v}^{\prime}(s)$.
\end{proof}

To complete the proof of Lemma \ref{join}, fix $i\in A_{l-1}(S\cap U)$.  It follows from (\ref{A}) that $i\in{\bf v}(s)$ for some $s\in S\cap U$ and $\text{\sc layer}(i)=l-1$.  Since $i\in A_{l-1}(U)$, it follows from (\ref{shift2}) that $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)+1=l$.  There are two cases to consider: $v^{\prime}(s)=v(s)$ and $v^{\prime}(s)\neq v(s)$.  In both cases Claim \ref{join}.1 and Claim \ref{join}.2 respectively show that $i\in{\bf v}^{\prime}(s)$.  Since $i\in{\bf v}^{\prime}(s)$ for some some $s\in S\cap U$ and $\text{\sc layer}(i)=l$, it follows from (\ref{Aprime}) that $i\in A^{\prime}_{l}(S\cap U)$.
\end{proof}


==> flowdecomp 2/remain.tex <==
\begin{lemma}
\label{remain}
For every $S\subseteq{\cal S}(d)$ and $l\in\{0,\ldots,|{\bf L}_{d}|-1\}$, $A^{\prime}_{l}(S\setminus U)	\subseteq A_{l}(S\setminus U)$
\end{lemma}
\begin{proof}
First we prove some preliminary claims.

\hspace{-3.5mm}\text{\bf Claim \ref{remain}.1}. \textit{For every $s\notin U$, there exists some $i\in{\bf v}(s)$ such that $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$}.

\begin{proof}
The proof is by contradiction.  Fix some $s\notin U$, $i\in{\bf v}(s)$, and assume without lost of generality, that $\text{\sc layer}(i)=l$.  If the claim is false, then $i\in{\bf v}(s)$ implies $\text{\sc layer}^{\prime}(i)>\text{\sc layer}(i)$.  Hence, (\ref{shift2}) implies $i\in A_{l}(U)$.  This argument applies to every $i\in{\bf v}(s)$.  It follows that for every $l=0,\ldots,|{\bf L}_{d}|-1$:
\begin{align}
	\nonumber
	\hspace{-60mm}&I(X_{A_{l}(U\cup\{s\})};Y_{d}|X_{\tilde{A}_{l}(U\cup\{s\})})\\
	\label{remain1}
	&\hspace{38mm}=I(X_{A_{l}(U)};Y_{d}|X_{\tilde{A}_{l}(U)}).
\end{align}
By definition, $U\subseteq{\cal S}(d)$ is the largest subset such that:
\begin{align}
\label{remain2}
	R_{U}&>\displaystyle\sum^{|{\bf L}_{d}|-1}_{l=0}I(X_{A_{l}(U)};Y_{d}|X_{\tilde{A}_{l}(U)}).
\end{align}
Since $R_{U\cup\{s\}}\geq R_{U}$, it follows from (\ref{remain1}) and (\ref{remain2}) that:
\begin{align}
\label{remain3}
	R_{U\cup\{s\}}&>\displaystyle\sum^{|{\bf L}_{d}|-1}_{l=0}I(X_{A_{l}(U\cup\{s\})};Y_{d}|X_{\tilde{A}_{l}(U\cup\{s\})}),
\end{align}
which contradicts the definition of $U$ as the largest subset of ${\cal S}(d)$ that violates (\ref{flowdecomp}).
\end{proof}

%\hspace{-3.5mm}{\bf Claim \ref{remain}.2}. \textit{For every $s\notin U$,}
%\begin{align}
%\label{Case2vprimes}
%	v^{\prime}(s)&:=\left\{j:\arg\displaystyle\min_{\substack{j\in {\bf v}(s),\\ \text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)}} k_{v(s),j}\right\}.
%\end{align}
%\begin{proof}
%It follows from Claim \ref{remain}.1 that $v^{\prime}(s)$ is non-empty.  To prove Claim \ref{remain}.2, it suffices to show that (\ref{Case2vprimes}) satisfies (\ref{firstIndexCodingShiftedComplete}) and (\ref{secondIndexShiftedComplete}). The proof follows from the same sequence of inequalities in (\ref{Case3Stage28}) - (\ref{Case3Stage222}).
%\end{proof}

%\hspace{-3.5mm}\text{\bf Claim \ref{remain}.3}. \textit{Fix $s\notin U$.  If $i\notin{\bf v}(s)$ and $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ then $i\notin{\bf v}^{\prime}(s)$.}
%\begin{proof}
%If $i\notin{\bf v}(s)$, then (V5) implies:
%\begin{align}
%\label{remain4}
%	\text{\sc layer}(v(s))-\text{\sc layer}(i)&\neq k_{v(s),i}.
%\end{align}
%Subtracting $k_{v(s),v^{\prime}(s)}$ from both sides of (\ref{remain4}) gives:
%\begin{align}
%\label{remain5}
%	\text{\sc layer}(v(s))-\text{\sc layer}(i)-k_{v(s),v^{\prime}(s)}&\neq k_{v^{\prime}(s),i},
%\end{align}
%where (\ref{remain5}) follows because $k_{v(s),v^{\prime}(s)}+k_{v^{\prime}(s),i}=k_{v(s),i}$.  It follows from (\ref{Case2vprimes}) that $v^{\prime}(s)\in{\bf v}(s)$.  Since $v^{\prime}(s)\in{\bf v}(s)$, it follows from (V5) that $\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))=k_{v(s),v^{\prime}(s)}$.  Therefore: \begin{align}
%	\label{remain6}
%	\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(i)&\neq k_{v^{\prime}(s),i},
%\end{align}
%where (\ref{remain6}) follows from substituting $\text{\sc layer}(v^{\prime}(s))=\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)}$ into (\ref{remain5}).  Hence,
%\begin{align}
%	\label{remain7}
%	\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)&\neq k_{v^{\prime}(s),i},
%\end{align} 
%where (\ref{remain7}) follows from substituting $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v(s))$ (by construction in (\ref{Case2vprimes})) and $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ (by claim assumption) into (\ref{remain6}).  It follows from (V5) and (\ref{remain7}) that $i\notin{\bf v}^{\prime}(s)$.
%\end{proof}

\hspace{-3.5mm}\text{\bf Claim \ref{remain}.2}. \textit{If $i\in{\bf v}^{\prime}(s)$ for any $s\in S\setminus U$ then $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$.}
\begin{proof}
Fix $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.  We have the following sequence of equalities:
\begin{align}
	\label{remain4}
	k_{v^{\prime}(s),i}&=\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i),\\
	\label{remain5}
	&=\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i),\\
	\label{remain6}
	&=\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)}-\text{\sc layer}^{\prime}(i),
\end{align}
where (\ref{remain4}) follows from (V5) and because $i\in{\bf v}^{\prime}(s)$.  To justify (\ref{remain5}), observe that Claim \ref{disjoint}.3 implies $v^{\prime}(s)$ is defined by (\ref{Case3v2s}) provided there is some $j\in{\bf v}(s)$ such that $\text{\sc layer}^{\prime}(j)=\text{\sc layer}(j)$.  Claim \ref{remain}.1 implies that such a $j\in{\bf v}(s)$ exists.  By construction in (\ref{Case3v2s}), $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$, so (\ref{remain5}) follows from (\ref{remain4}).  Finally, (\ref{remain6}) follows from (V5) and because (\ref{Case3v2s}) implies  $v^{\prime}(s)\in{\bf v}(s)$.  Since $i\in{\bf v}^{\prime}(s)$ and $v^{\prime}(s)\in{\bf v}(s)$ it follows that $k_{v(s),v^{\prime}(s)}+k_{v^{\prime}(s),i}=k_{v(s),i}$.  Therefore:
\begin{align}
	\label{remain7}
	k_{v(s),i}&=\text{\sc layer}(v(s))-\text{\sc layer}^{\prime}(i),
\end{align} 
where (\ref{remain7}) follows from (\ref{remain6}) and because $k_{v(s),v^{\prime}(s)}+k_{v^{\prime}(s),i}=k_{v(s),i}$.  Moreover,
\begin{align}
	\label{remain8}
	\text{\sc layer}^{\prime}(i)\geq\text{\sc layer}(i),
\end{align}
where (\ref{remain8}) follows from (\ref{shift2}).  Therefore:
\begin{align}
	\label{remain9}
	\text{\sc layer}(v(s))-\text{\sc layer}(i)&\geq k_{v(s),i},
\end{align}
where (\ref{remain9}) follows from substituting (\ref{remain8}) into (\ref{remain7}).  Now $i\in{\bf f}(v^{\prime}(s),d)$ since $i\in{\bf v}^{\prime}(s)$ and $v^{\prime}(s)\in{\bf f}(v(s),d)$ since (\ref{Case3v2s}) implies $v^{\prime}(s)\in{\bf v}(s)$.  Therefore $i\in{\bf f}(v(s),d)$.  Invoking (\ref{firstIndexCodingShiftedComplete2}) and (\ref{remain9}) together gives:
\begin{align}
	\label{remain91}
	\text{\sc layer}(v(s))-\text{\sc layer}(i)&=k_{v(s),i}.
\end{align}
Comparing (\ref{remain91}) and (\ref{remain7}) gives $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$.  
%\begin{align}
%	\nonumber
%	&\hspace{-2mm}\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)\\
%	\label{remain4}
%	&\hspace{3mm}=[\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)}]-\text{\sc layer}^{\prime}(i),\\
%		\label{remain5}
%	&\hspace{3mm}=[\text{\sc layer}(v(s))-k_{v(s),v^{\prime}(s)}]-[\text{\sc layer}(i)+1],\\
%	\label{remain6}
%	&\hspace{3mm}=[\text{\sc layer}(v(s))-\text{\sc layer}(i)]-k_{v(s),v^{\prime}(s)}-1,\\
%	\label{remain7}
%	&\hspace{3mm}\leq k_{v(s),i}-k_{v(s),v^{\prime}(s)}-1,\\
%	\label{remain8}
%	&\hspace{3mm}=k_{v^{\prime}(s),i}-1,\\
%	\label{remain9}
%	&\hspace{3mm}<k_{v^{\prime}(s),i},
%\end{align}
%where (\ref{remain4}) follows because $v^{\prime}(s)\in{\bf v}(s)$ (from (\ref{Case2vprimes})) and (V5) implies $\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))=k_{v(s),v^{\prime}(s)}$ if $v^{\prime}(s)\in{\bf v}(s)$, (\ref{remain5}) follows from (\ref{shift2}) and because $\text{\sc layer}^{\prime}(i)>\text{\sc layer}(i)$ (by claim assumption), (\ref{remain6}) follows by rearranging (\ref{remain5}), (\ref{remain7}) follows from (\ref{firstIndexCodingShiftedComplete}) and because $i\in{\bf f}(v(s),d)$, and  (\ref{remain8}) follows because $k_{v(s),v^{\prime}(s)}+k_{v^{\prime}(s),i}=k_{v(s),i}$.  Since $\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)\neq k_{v^{\prime}(s),i}$, it follows from (V5) that $i\notin{\bf v}^{\prime}(s)$.
%Now suppose $i\in{\bf f}(s,v(s))$.  Since $v^{\prime}(s)\in{\bf v}(s)$ (from Claim \ref{remain}.2) it follows from (\ref{firstIndexCodingShiftedComplete2}) that $i\in{\bf f}(s,v^{\prime}(s))$.  Furthermore (\ref{secondIndexShiftedComplete}) implies that $\text{\sc layer}^{\prime}(i)-\text{\sc layer}^{\prime}(v^{\prime}(s))>k_{i,v^{\prime}(s)}$.  It follows from (V5) that $i\notin{\bf v}^{\prime}(s)$.
\end{proof}
To complete the proof of Lemma \ref{remain}, fix some $i\in A^{\prime}_{l}(S\setminus U)$.  It follows from (\ref{Aprime}) that $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.  Since $i\in{\bf v}^{\prime}(s)$, Claim \ref{remain}.2 implies that $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$.  Consider the following inequalities:
\begin{align}
	\nonumber
	&\text{\sc layer}(v(s))-\text{\sc layer}(i)\\
	\nonumber
	&\hspace{3mm}=\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))\\
	\label{remain10}
	&\hspace{32mm}+\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(i),\\
	\label{remain11}
	&\hspace{3mm}=k_{v(s),v^{\prime}(s)}+(\text{\sc layer}(v^{\prime}(s))-\text{\sc layer}(i)),\\
	\label{remain12}
	&\hspace{3mm}=k_{v(s),v^{\prime}(s)}+(\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)),\\
	\label{remain13}
	&\hspace{3mm}=k_{v(s),v^{\prime}(s)}+k_{v^{\prime}(s),i},\\
	\label{remain14}
	&\hspace{3mm}=k_{v(s),i},
\end{align}
where (\ref{remain10}) follows by adding and subtracting $\text{\sc layer}(v^{\prime}(s))$ from the left side, (\ref{remain11}) follows because (V5) implies $\text{\sc layer}(v(s))-\text{\sc layer}(v^{\prime}(s))=k_{v(s),v^{\prime}(s)}$ if $v^{\prime}(s)\in{\bf v}(s)$ and (\ref{Case3v2s}) implies $v^{\prime}(s)\in{\bf v}(s)$, (\ref{remain12}) follows because (\ref{Case3v2s}) implies $\text{\sc layer}^{\prime}(v^{\prime}(s))=\text{\sc layer}(v^{\prime}(s))$ and Claim \ref{remain}.2 implies $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ if $i\in{\bf v}^{\prime}(s))$, and (\ref{remain13}) follows from (V5) which implies that $\text{\sc layer}^{\prime}(v^{\prime}(s))-\text{\sc layer}^{\prime}(i)=k_{v^{\prime}(s),i}$ if $i\in{\bf v}^{\prime}(s)$.  Since (\ref{remain14}) implies that $\text{\sc layer}(v(s))-\text{\sc layer}(i)=k_{v(s),i}$, it follows from (V5) that $i\in{\bf v}(s)$.  

Now $i\in A^{\prime}_{l}(S\setminus U)$, so (\ref{Aprime}) implies that $\text{\sc layer}^{\prime}(i)=l$.  Moreover, $i\in{\bf v}(s)$ for some $s\in S\setminus U$, so Claim \ref{remain}.2 implies $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$.  Therefore $\text{\sc layer}(i)=l$ which implies $i\in L_{l}$.  Since $i\in{\bf v}(s)$ and $s\in S\setminus U$ and $i\in L_{l}$, it follows from (\ref{A}) that $i\in A_{l}(S\setminus U)$.
%Observe that (\ref{shift2}) implies $\text{\sc layer}^{\prime}(i)\geq\text{\sc layer}(i)$.  It is convenient to consider $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$ separately from $\text{\sc layer}^{\prime}(i)>\text{\sc layer}(i)$.  Suppose $\text{\sc layer}^{\prime}(i)=\text{\sc layer}(i)$.  Since $i\in{\bf v}^{\prime}(s)$, it follows from [Lemma \ref{remain}]:(CL3) that $i\in{\bf v}(s)$.  By definition (\ref{A}), $i\in A_{l}(S\setminus U)$.  Now suppose $\text{\sc layer}^{\prime}(i)>\text{\sc layer}(i)$.  We will show that $i\notin{\bf v}(s)$.
	%Fix $i\in A^{\prime}_{l}(S\setminus U)$ and suppose $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.  If node $i$ is a non-shifted node then $i\in{\bf v}(s)$ and $\text{\sc layer}(i)=l$.  If node $i$ is a shifted node then $i\in A_{l-1}(U)$ but $A_{l-1}(U)\cap A_{l}(S\setminus U)=\{\}$.  Therefore it suffices to show that node $i$ cannot be a shifted node that remains within a non-shifted flow ${\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.  
	%Assume the contrary; $\text{\sc layer}(i)=l-1$, $\text{\sc layer}^{\prime}(i)=l$, and $i\in{\bf v}^{\prime}(s)$ for some $s\in S\setminus U$.  There are two cases to consider.
 %First suppose the non-shifted flow ${\bf v}(s)$ is not fully contained in the shifted flows.  That is, $V(\{s\})\not\subseteq V(U)$.  The claim is that none of the shifted nodes in ${\bf v}(s)$ will be in ${\bf v}^{\prime}(s)$.  If $v(s)$ is a shifted node then $v(s)$ does not satisfy (\ref{firstIndexCoding}) with respect to the non-shifted nodes downstream of $v(s)$ in ${\bf v}(s)$; $v^{\prime}(s)$ must be the closest (by-hop-count) non-shifted node (or set of nodes) downstream of $v(s)$ in ${\bf v}(s)$.  Since $v^{\prime}(s)$ is non-shifted, none of the other shifted nodes in ${\bf v}(s)$ satisfy (V4) post-{\sc shift}.  Therefore these shifted nodes will not be in ${\bf v}^{\prime}(s)$.  If $v(s)$ is a \textit{non}-shifted node then $v^{\prime}(s)=v(s)$ still satisfies (\ref{firstIndexCoding}) with respect to the shifted and non-shifted nodes downstream of $v(s)$ in ${\bf v}(s)$.  As before,  $v^{\prime}(s)$ is non-shifted so none of the shifted nodes in ${\bf v}(s)$ satisfy (V4) post-{\sc shift}.  Therefore these shifted nodes will not be in ${\bf v}^{\prime}(s)$.  
%Next suppose the non-shifted flow is fully contained in the shifted flows.  That is, $V(\{s\})\subseteq V(U)$.  Then $A_{k}(U\cup\{s\})=A_{k}(U)$ for all $k=0,\ldots,|{\bf L}|-1$ which contradicts the assumption that $U$ is the largest subset that violates (\ref{flowdecomp}) since $s\in S\setminus U$.
\end{proof}


==> flowdecomp 2/splitting.tex <==
\begin{lemma} 
\label{splitting}
 If (C1) and (C2) are satisfied then (C3), (C4), and (C5) are also satisfied.
\end{lemma}
\begin{proof}
Given the assumptions $i\in{\bf f}(s)$, $i\in A_{l}({\cal N})$, and $i\in{\bf v}(s)$ in (C3), consider the following sequence of inequalities:
\begin{align}
	\label{C2proof1}
	b-l-k_{s,i}&=b-\text{\sc layer}(i)-k_{s,i},\\
	\label{C2proof2}
	&=b-(\text{\sc layer}(v(s))-k_{v(s),i})-k_{s,i},\\
	\nonumber
	&=b-\text{\sc layer}(v(s))-(k_{s,i}-k_{v(s),i}),\\
	\label{C2proof3}
	&=b-\text{\sc layer}(v(s))-k_{s,v(s)},
\end{align}
where (\ref{C2proof1}) follows because (\ref{AN}) implies that $i\in A_{l}({\cal N})$ only if $i\in L_{l}$ which implies $\text{\sc layer}(i)=l$, and (\ref{C2proof2}) follows because (V5) implies $i\in{\bf v}(s)$ only if $\text{\sc layer}(v(s))-\text{\sc layer}(i)=k_{v(s),i}$.  By inspection, (\ref{C2proof3}) satisfies (\ref{C2}) in (C3).

Consider assumptions $i\in{\bf f}(s)$ and $i\in L_{l}$ in (C4).  If (C2) is satisfied, then (\ref{C1}) implies $s\in{\cal S}(d)$ which implies that $v(s)$ and ${\bf v}(s)$ exist at node $d$, as defined by (\ref{vs}) and (V1)-(V5) respectively.  Assume $i\notin{\bf v}(s)$ as stated in (C4).  
% \input{"clocksecurity.tex"}
Suppose $i\in{\bf f}(v(s),d)$ and consider the following inequalities:
\begin{align}
	\label{feasibility1}
	b-l-k_{s,i}&\leq b-(\text{\sc layer}(v(s))-k_{v(s),i})-k_{s,i},\\
	\nonumber
	&=b-(k_{s,i}-k_{v(s),i})-\text{\sc layer}(v(s)),\\
	\label{feasibility12}
	&=b-k_{s,v(s)}-\text{\sc layer}(v(s)),
\end{align} 
where (\ref{feasibility1}) follows from (\ref{firstIndexCoding}) 
and because (L5) implies $\text{\sc layer}(i)=l$ if $i\in L_{l}$.   Equality in (\ref{feasibility12}) only occurs if property (V5) holds which implies $i\in{\bf v}(s)$ as in (\ref{C2proof3}).  Since $i\notin{\bf v}(s)$, it follows from (\ref{C2proof3}) and (\ref{feasibility12}) that:
\begin{align}
\label{feasibility13}
b-l-k_{s,i}<b-k_{s,v(s)}-\text{\sc layer}(v(s))
\end{align}   
Now suppose $i\in{\bf f}(s,v(s))$.  Note that ${\bf f}(s,v(s))$ precedes $v(s)$ so $i\notin{\bf v}(s)$.  Consider the following inequalities: 
\begin{align}
	\label{feasibility2}
	b-l-k_{s,i}&<b-(k_{i,v(s)}+\text{\sc layer}(v(s)))-k_{s,i},\\
	\nonumber
	&=b-(k_{s,i}+k_{i,v(s)})-\text{\sc layer}(v(s)),\\
	\label{feasibility22}
	&=b-k_{s,v(s)}-\text{\sc layer}(v(s)),
\end{align} 
where (\ref{feasibility2}) follows from (\ref{secondIndexCoding}) and because (L5) implies $\text{\sc layer}(i)=l$ if $i\in L_{l}$ (L5).  Since $i\notin{\bf v}(s)$, it follows from (\ref{feasibility13}) and (\ref{feasibility22}) that: 
\begin{align}
\label{C3proof1}
b-l-k_{s,i}<b-k_{s,v(s)}-\text{\sc layer}(v(s)),  	
\end{align}
which satisfies (\ref{C3}) in (C4).

Consider assumptions $i\in{\bf f}(s)$ and $i\in\tilde{A}_{l}({\cal N})$ in (C5).  It follows from (\ref{AtildeN}) that $\tilde{A}_{l}({\cal N})=((\cup_{j\in I(d)}F_{j}({\cal N}))\setminus F_{d}({\cal N}))\cup(F_{d}({\cal N})\setminus(\cup^{|{\bf L}_{d}|-1}_{q=l+1}L_{q}\cup A_{l}({\cal N})))$.  First, suppose $i\in(F_{d}({\cal N})\setminus(\cup^{|{\bf L}_{d}|-1}_{q=l+1}L_{q}\cup A_{l}({\cal N})))$.  It follows from property (L3) and (\ref{AN}) that $(F_{d}({\cal N})\setminus(\cup^{|{\bf L}_{d}|-1}_{q=l+1}L_{q}\cup A_{l}({\cal N})))=(L_{l}\setminus A_{l}({\cal N}))\cup(\cup^{l-1}_{q=0}L_{q})$.  If $i\in L_{l}\setminus A_{l}({\cal N})$ then (\ref{AN}) implies $i\notin{\bf v}(s)$ for every  $s\in{\cal S}(d)$.  It follows from (\ref{C3proof1}) that (C5) is satisfied.  If $i\in\cup^{l-1}_{q=0}L_{q}$ then $b-q-k_{s,i}\leq b-k_{s,v(s)}-\text{\sc layer}(v(s))$ for some $0\leq q\leq l-1$ and $\text{sc layer}(i)=q$, as implied by (\ref{feasibility12}) when $i\in{\bf f}(v(s),d)$ and (\ref{feasibility22}) when $i\in{\bf f}(s,v(s))$.  Therefore $b-l-k_{s,i}<b-k_{s,v(s)}-\text{\sc layer}(v(s))$ which satisfies (C5).  Second, suppose $i\in(\cup_{j\in I(d)}F_{j}({\cal N}))\setminus F_{d}({\cal N})$ and consider the following inequalities:
\begin{align}
	\label{C5proof1}
	b-k_{s,v(s)}-\text{\sc layer}(v(s))&>b-k_{s,d},\\
	\label{C5proof2}
	&>b-k_{s,i},
\end{align}
where (\ref{C5proof1}) follows from (C1).  By definition in (\ref{id}), $I(d):=\{j:{\cal S}(j)\subseteq{\cal S}(d)\}$, so (\ref{sd}) implies node $i$ only encodes sources decoded by node $d$.  Since $i\notin F_{d}({\cal N})$, node $i$ is ``downstream'' of node $d$ so that $k_{s,i}>k_{s,d}$ which implies (\ref{C5proof2}).  It follows from (\ref{C5proof2}) that $b-k_{s,v(s)}-\text{\sc layer}(v(s))>b-l-k_{s,i}$ which satisfies (C5).
\end{proof} 

